Some New Results on the Maximum Growth Factor in Gaussian Elimination

This paper combines modern numerical computation with theoretical results to improve our understanding of the growth factor problem for Gaussian elimination. On the computational side we obtain lower bounds for the maximum growth for complete pivoting for $n=1:75$ and $n=100$ using the Julia JuMP optimization package. At $n=100$ we obtain a growth factor bigger than $3n$. The numerical evidence suggests that the maximum growth factor is bigger than $n$ if and only if $n \ge 11$. We also present a number of theoretical results. We show that the maximum growth factor over matrices with entries restricted to a subset of the reals is nearly equal to the maximum growth factor over all real matrices. We also show that the growth factors under floating point arithmetic and exact arithmetic are nearly identical. Finally, through numerical search, and stability and extrapolation results, we provide improved lower bounds for the maximum growth factor. Specifically, we find that the largest growth factor is bigger than $1.0045n$ for $n>10$, and the lim sup of the ratio with $n$ is greater than or equal to $3.317$. In contrast to the old conjecture that growth might never be bigger than $n$, it seems likely that the maximum growth divided by $n$ goes to infinity as $n \rightarrow \infty$.

==> julia_font.tex <==
\newfontfamily\JuliaMono{JuliaMono}[
    UprightFont = *-Regular,
    BoldFont = *-Bold,
    Path = ./,
    Extension = .ttf]
\newfontface\JuliaMonoRegular{JuliaMono-Regular}
\newfontface\JuliaMonoBold{JuliaMono-Bold}
\setmonofont{JuliaMono-Medium}[Contextuals=Alternate]



==> julia_listings.tex <==
\input{julia_listings_unicode} % full unicode support


% This is the primary language defn for Julia.
\lstdefinelanguage{Julia}{
    % keywords
    keywords=[1]{begin,end,let,using,import,export,in,if,else,elseif,for,while,do,try,type,catch,finally,return,break,continue},
    % functions
    keywords=[2]{abs,abs2,abspath,accept,accumulate,accumulate!,acos,acos_fast,acosd,acosh,acosh_fast,acot,acotd,acoth,acsc,acscd,acsch,adjoint,adjoint!,all,all!,allunique,angle,angle_fast,any,any!,append!,apropos,ascii,asec,asecd,asech,asin,asin_fast,asind,asinh,asinh_fast,assert,asyncmap,asyncmap!,atan,atan2,atan2_fast,atan_fast,atand,atanh,atanh_fast,atexit,atreplinit,axes,backtrace,base,basename,beta,big,bin,bind,binomial,bitbroadcast,bitrand,bits,bitstring,bkfact,bkfact!,blkdiag,broadcast,broadcast!,broadcast_getindex,broadcast_setindex!,bswap,bytes2hex,cat,catch_backtrace,catch_stacktrace,cbrt,cbrt_fast,cd,ceil,cfunction,cglobal,charwidth,checkbounds,checkindex,chmod,chol,cholfact,cholfact!,chomp,chop,chown,chr2ind,circcopy!,circshift,circshift!,cis,cis_fast,clamp,clamp!,cld,clipboard,close,cmp,coalesce,code_llvm,code_lowered,code_native,code_typed,code_warntype,codeunit,codeunits,collect,colon,complex,cond,condskeel,conj,conj!,connect,consume,contains,convert,copy,copy!,copysign,copyto!,cor,cos,cos_fast,cosc,cosd,cosh,cosh_fast,cospi,cot,cotd,coth,count,count_ones,count_zeros,countlines,countnz,cov,cp,cross,csc,cscd,csch,ctime,ctranspose,ctranspose!,cummax,cummin,cumprod,cumprod!,cumsum,cumsum!,current_module,current_task,dec,deepcopy,deg2rad,delete!,deleteat!,den,denominator,deserialize,det,detach,diag,diagind,diagm,diff,digits,digits!,dirname,disable_sigint,display,displayable,displaysize,div,divrem,done,dot,download,dropzeros,dropzeros!,dump,eachcol,eachindex,eachline,eachmatch,edit,eig,eigfact,eigfact!,eigmax,eigmin,eigvals,eigvals!,eigvecs,eltype,empty,empty!,endof,endswith,enumerate,eof,eps,equalto,error,esc,escape_string,evalfile,exit,exp,exp10,exp10_fast,exp2,exp2_fast,exp_fast,expanduser,expm,expm!,expm1,expm1_fast,exponent,extrema,eye,factorial,factorize,falses,fd,fdio,fetch,fieldcount,fieldname,fieldnames,fieldoffset,filemode,filesize,fill,fill!,filter,filter!,finalize,finalizer,find,findfirst,findin,findlast,findmax,findmax!,findmin,findmin!,findn,findnext,findnz,findprev,first,fld,fld1,fldmod,fldmod1,flipbits!,flipdim,flipsign,float,floor,flush,fma,foldl,foldr,foreach,frexp,full,fullname,functionloc,gamma,gc,gc_enable,gcd,gcdx,gensym,get,get!,get_zero_subnormals,getaddrinfo,getalladdrinfo,gethostname,getindex,getipaddr,getkey,getnameinfo,getpeername,getpid,getsockname,givens,gperm,gradient,hash,haskey,hcat,hessfact,hessfact!,hex,hex2bytes,hex2bytes!,hex2num,homedir,htol,hton,hvcat,hypot,hypot_fast,identity,ifelse,ignorestatus,im,imag,in,include_dependency,include_string,ind2chr,ind2sub,indexin,indices,indmax,indmin,info,insert!,instances,intersect,intersect!,inv,invmod,invperm,invpermute!,ipermute!,ipermutedims,is,is_apple,is_bsd,is_linux,is_unix,is_windows,isabspath,isapprox,isascii,isassigned,isbits,isblockdev,ischardev,isconcrete,isconst,isdiag,isdir,isdirpath,isempty,isequal,iseven,isfifo,isfile,isfinite,ishermitian,isimag,isimmutable,isinf,isinteger,isinteractive,isleaftype,isless,isletter,islink,islocked,ismarked,ismatch,ismissing,ismount,isnan,isodd,isone,isopen,ispath,isperm,isposdef,isposdef!,ispow2,isqrt,isreadable,isreadonly,isready,isreal,issetgid,issetuid,issocket,issorted,issparse,issticky,issubnormal,issubset,issubtype,issymmetric,istaskdone,istaskstarted,istextmime,istril,istriu,isvalid,iswritable,iszero,join,joinpath,keys,keytype,kill,kron,last,lbeta,lcm,ldexp,ldltfact,ldltfact!,leading_ones,leading_zeros,length,less,lexcmp,lexless,lfact,lgamma,lgamma_fast,linearindices,linreg,linspace,listen,listenany,lock,log,log10,log10_fast,log1p,log1p_fast,log2,log2_fast,log_fast,logabsdet,logdet,logging,logm,logspace,lpad,lq,lqfact,lqfact!,lstat,lstrip,ltoh,lu,lufact,lufact!,lyap,macroexpand,map,map!,mapfoldl,mapfoldr,mapreduce,mapreducedim,mapslices,mark,match,matchall,max,max_fast,maxabs,maximum,maximum!,maxintfloat,mean,mean!,median,median!,merge,merge!,method_exists,methods,methodswith,middle,midpoints,mimewritable,min,min_fast,minabs,minimum,minimum!,minmax,minmax_fast,missing,mkdir,mkpath,mktemp,mktempdir,mod,mod1,mod2pi,modf,module_name,module_parent,mtime,muladd,mv,names,nb_available,ncodeunits,ndigits,ndims,next,nextfloat,nextind,nextpow,nextpow2,nextprod,nnz,nonzeros,norm,normalize,normalize!,normpath,notify,ntoh,ntuple,nullspace,num,num2hex,numerator,nzrange,object_id,occursin,oct,oftype,one,ones,oneunit,open,operm,ordschur,ordschur!,pairs,parent,parentindexes,parentindices,parse,partialsort,partialsort!,partialsortperm,partialsortperm!,peakflops,permute,permute!,permutedims,permutedims!,pi,pinv,pipeline,pointer,pointer_from_objref,pop!,popdisplay,popfirst!,position,pow_fast,powermod,precision,precompile,prepend!,prevfloat,prevind,prevpow,prevpow2,print,print_shortest,print_with_color,println,process_exited,process_running,prod,prod!,produce,promote,promote_rule,promote_shape,promote_type,push!,pushdisplay,pushfirst!,put!,pwd,qr,qrfact,qrfact!,quantile,quantile!,quit,rad2deg,rand,rand!,randcycle,randcycle!,randexp,randexp!,randjump,randn,randn!,randperm,randperm!,randstring,randsubseq,randsubseq!,range,rank,rationalize,read,read!,readandwrite,readavailable,readbytes!,readchomp,readdir,readline,readlines,readlink,readstring,readuntil,real,realmax,realmin,realpath,recv,recvfrom,redirect_stderr,redirect_stdin,redirect_stdout,redisplay,reduce,reducedim,reenable_sigint,reim,reinterpret,reload,relpath,rem,rem2pi,repeat,replace,replace!,repmat,repr,reprmime,reset,reshape,resize!,rethrow,retry,reverse,reverse!,reverseind,rm,rol,rol!,ror,ror!,rot180,rotl90,rotr90,round,rounding,rowvals,rpad,rsearch,rsearchindex,rsplit,rstrip,run,scale!,schedule,schur,schurfact,schurfact!,search,searchindex,searchsorted,searchsortedfirst,searchsortedlast,sec,secd,sech,seek,seekend,seekstart,select,select!,selectperm,selectperm!,send,serialize,set_zero_subnormals,setdiff,setdiff!,setenv,setindex!,setprecision,setrounding,shift!,show,showall,showcompact,showerror,shuffle,shuffle!,sign,signbit,signed,signif,significand,similar,sin,sin_fast,sinc,sincos,sind,sinh,sinh_fast,sinpi,size,sizehint!,sizeof,skip,skipchars,skipmissing,sleep,slicedim,sort,sort!,sortcols,sortperm,sortperm!,sortrows,sparse,sparsevec,spawn,spdiagm,speye,splice!,split,splitdir,splitdrive,splitext,spones,sprand,sprandn,sprint,spzeros,sqrt,sqrt_fast,sqrtm,squeeze,srand,stacktrace,start,startswith,stat,std,stdm,step,stride,strides,string,stringmime,strip,strwidth,sub2ind,subtypes,success,sum,sum!,sumabs,sumabs2,summary,supertype,svd,svdfact,svdfact!,svdvals,svdvals!,sylvester,symdiff,symdiff!,symlink,systemerror,take!,takebuf_array,takebuf_string,tan,tan_fast,tand,tanh,tanh_fast,task_local_storage,tempdir,tempname,thisind,tic,time,time_ns,timedwait,to_indices,toc,toq,touch,trace,trailing_ones,trailing_zeros,transcode,transpose,transpose!,tril,tril!,triu,triu!,trues,trunc,truncate,trylock,tryparse,typeintersect,typejoin,typemax,typemin,unescape_string,union,union!,unique,unique!,unlock,unmark,unsafe_copy!,unsafe_copyto!,unsafe_load,unsafe_pointer_to_objref,unsafe_read,unsafe_store!,unsafe_string,unsafe_trunc,unsafe_wrap,unsafe_write,unshift!,unsigned,uperm,valtype,values,var,varinfo,varm,vcat,vec,vecdot,vecnorm,versioninfo,view,wait,walkdir,warn,which,whos,widemul,widen,withenv,workspace,write,xor,yield,yieldto,zero,zeros,zip,applicable,eval,fieldtype,getfield,invoke,isa,isdefined,nfields,nothing,setfield!,throw,tuple,typeassert,typeof,uninitialized,undef,
    asum,axpby!,axpy!,blascopy!,dot,dotc,dotu,gbmv,gbmv!,gemm,gemm!,gemv,gemv!,ger!,hemm,hemm!,hemv,hemv!,her!,her2k,her2k!,herk,herk!,iamax,nrm2,sbmv,sbmv!,scal,scal!,symm,symm!,symv,symv!,syr!,syr2k,syr2k!,syrk,syrk!,trmm,trmm!,trmv,trmv!,trsm,trsm!,trsv,trsv!),abs,abs2,abspath,accept,accumulate,accumulate!,acos,acos_fast,acosd,acosh,acosh_fast,acot,acotd,acoth,acsc,acscd,acsch,adjoint,adjoint!,all,all!,allunique,angle,angle_fast,any,any!,append!,apropos,argmax,argmin,ascii,asec,asecd,asech,asin,asin_fast,asind,asinh,asinh_fast,assert,asyncmap,asyncmap!,atan,atan2,atan2_fast,atan_fast,atand,atanh,atanh_fast,atexit,atreplinit,axes,backtrace,base,basename,beta,bfft,bfft!,big,bin,bind,binomial,bitbroadcast,bitrand,bits,bitstring,bkfact,bkfact!,blkdiag,brfft,broadcast,broadcast!,broadcast_getindex,broadcast_setindex!,bswap,bytes2hex,cat,catch_backtrace,catch_stacktrace,cbrt,cbrt_fast,cd,ceil,cfunction,cglobal,charwidth,checkbounds,checkindex,chmod,chol,cholfact,cholfact!,chomp,chop,chown,chr2ind,circcopy!,circshift,circshift!,cis,cis_fast,clamp,clamp!,cld,clipboard,close,cmp,coalesce,code_llvm,code_lowered,code_native,code_typed,code_warntype,codeunit,codeunits,collect,colon,complex,cond,condskeel,conj,conj!,connect,consume,contains,conv,conv2,convert,copy,copy!,copysign,copyto!,cor,cos,cos_fast,cosc,cosd,cosh,cosh_fast,cospi,cot,cotd,coth,count,count_ones,count_zeros,countlines,countnz,cov,cp,cross,csc,cscd,csch,ctime,ctranspose,ctranspose!,cummax,cummin,cumprod,cumprod!,cumsum,cumsum!,current_module,current_task,dct,dct!,dec,deconv,deepcopy,deg2rad,delete!,deleteat!,den,denominator,deserialize,det,detach,diag,diagind,diagm,diff,digits,digits!,dirname,disable_sigint,display,displayable,displaysize,div,divrem,done,dot,download,dropzeros,dropzeros!,dump,eachcol,eachindex,eachline,eachmatch,edit,eig,eigfact,eigfact!,eigmax,eigmin,eigvals,eigvals!,eigvecs,eltype,empty,empty!,endof,endswith,enumerate,eof,eps,equalto,error,esc,escape_string,evalfile,exit,exp,exp10,exp10_fast,exp2,exp2_fast,exp_fast,expand,expanduser,expm,expm!,expm1,expm1_fast,exponent,extrema,eye,factorial,factorize,falses,fd,fdio,fetch,fft,fft!,fftshift,fieldcount,fieldname,fieldnames,fieldoffset,filemode,filesize,fill,fill!,filt,filt!,filter,filter!,finalize,finalizer,find,findfirst,findin,findlast,findmax,findmax!,findmin,findmin!,findn,findnext,findnz,findprev,first,fld,fld1,fldmod,fldmod1,flipbits!,flipdim,flipsign,float,floor,flush,fma,foldl,foldr,foreach,frexp,full,fullname,functionloc,gamma,gc,gc_enable,gcd,gcdx,gensym,get,get!,get_zero_subnormals,getaddrinfo,getalladdrinfo,gethostname,getindex,getipaddr,getkey,getnameinfo,getpeername,getpid,getsockname,givens,gperm,gradient,hash,haskey,hcat,hessfact,hessfact!,hex,hex2bytes,hex2bytes!,hex2num,homedir,htol,hton,hvcat,hypot,hypot_fast,idct,idct!,identity,ifelse,ifft,ifft!,ifftshift,ignorestatus,im,imag,in,include_dependency,include_string,ind2chr,ind2sub,indexin,indices,indmax,indmin,info,insert!,instances,intersect,intersect!,inv,invmod,invperm,invpermute!,ipermute!,ipermutedims,irfft,is,is_apple,is_bsd,is_linux,is_unix,is_windows,isabspath,isapprox,isascii,isassigned,isbits,isblockdev,ischardev,isconcrete,isconst,isdiag,isdir,isdirpath,isempty,isequal,iseven,isfifo,isfile,isfinite,ishermitian,isimag,isimmutable,isinf,isinteger,isinteractive,isleaftype,isless,isletter,islink,islocked,ismarked,ismatch,ismissing,ismount,isnan,isodd,isone,isopen,ispath,isperm,isposdef,isposdef!,ispow2,isqrt,isreadable,isreadonly,isready,isreal,issetgid,issetuid,issocket,issorted,issparse,issticky,issubnormal,issubset,issubtype,issymmetric,istaskdone,istaskstarted,istextmime,istril,istriu,isvalid,iswritable,iszero,join,joinpath,keys,keytype,kill,kron,last,lbeta,lcm,ldexp,ldltfact,ldltfact!,leading_ones,leading_zeros,length,less,lexcmp,lexless,lfact,lgamma,lgamma_fast,linearindices,linreg,linspace,listen,listenany,lock,log,log10,log10_fast,log1p,log1p_fast,log2,log2_fast,log_fast,logabsdet,logdet,logging,logm,logspace,lpad,lq,lqfact,lqfact!,lstat,lstrip,ltoh,lu,lufact,lufact!,lyap,macroexpand,map,map!,mapfoldl,mapfoldr,mapreduce,mapreducedim,mapslices,mark,match,matchall,max,max_fast,maxabs,maximum,maximum!,maxintfloat,mean,mean!,median,median!,merge,merge!,method_exists,methods,methodswith,middle,midpoints,mimewritable,min,min_fast,minabs,minimum,minimum!,minmax,minmax_fast,missing,mkdir,mkpath,mktemp,mktempdir,mod,mod1,mod2pi,modf,module_name,module_parent,mtime,muladd,mv,names,nb_available,ncodeunits,ndigits,ndims,next,nextfloat,nextind,nextpow,nextpow2,nextprod,nnz,nonzeros,norm,normalize,normalize!,normpath,notify,ntoh,ntuple,nullspace,num,num2hex,numerator,nzrange,object_id,occursin,oct,oftype,one,ones,oneunit,open,operm,ordschur,ordschur!,pairs,parent,parentindexes,parentindices,parse,partialsort,partialsort!,partialsortperm,partialsortperm!,peakflops,permute,permute!,permutedims,permutedims!,pi,pinv,pipeline,plan_bfft,plan_bfft!,plan_brfft,plan_dct,plan_dct!,plan_fft,plan_fft!,plan_idct,plan_idct!,plan_ifft,plan_ifft!,plan_irfft,plan_rfft,pointer,pointer_from_objref,pop!,popdisplay,popfirst!,position,pow_fast,powermod,precision,precompile,prepend!,prevfloat,prevind,prevpow,prevpow2,print,print_shortest,print_with_color,println,process_exited,process_running,prod,prod!,produce,promote,promote_rule,promote_shape,promote_type,push!,pushdisplay,pushfirst!,put!,pwd,qr,qrfact,qrfact!,quantile,quantile!,quit,rad2deg,rand,rand!,randcycle,randcycle!,randexp,randexp!,randjump,randperm,randperm!,randstring,randsubseq,randsubseq!,range,rank,rationalize,read,read!,readandwrite,readavailable,readbytes!,readchomp,readdir,readline,readlines,readlink,readstring,readuntil,real,realmax,realmin,realpath,recv,recvfrom,redirect_stderr,redirect_stdin,redirect_stdout,redisplay,reduce,reducedim,reenable_sigint,reim,reinterpret,reload,relpath,rem,rem2pi,repeat,replace,replace!,repmat,repr,reprmime,reset,reshape,resize!,rethrow,retry,reverse,reverse!,reverseind,rfft,rm,rol,rol!,ror,ror!,rot180,rotl90,rotr90,round,rounding,rowvals,rpad,rsearch,rsearchindex,rsplit,rstrip,run,scale!,schedule,schur,schurfact,schurfact!,search,searchindex,searchsorted,searchsortedfirst,searchsortedlast,sec,secd,sech,seek,seekend,seekstart,select,select!,selectperm,selectperm!,send,serialize,set_zero_subnormals,setdiff,setdiff!,setenv,setindex!,setprecision,setrounding,shift!,show,showall,showcompact,showerror,shuffle,shuffle!,sign,signbit,signed,signif,significand,similar,sin,sin_fast,sinc,sincos,sind,sinh,sinh_fast,sinpi,size,sizehint!,sizeof,skip,skipchars,skipmissing,sleep,slicedim,sort,sort!,sortcols,sortperm,sortperm!,sortrows,sparse,sparsevec,spawn,spdiagm,speye,splice!,split,splitdir,splitdrive,splitext,spones,sprand,sprandn,sprint,spzeros,sqrt,sqrt_fast,sqrtm,squeeze,srand,stacktrace,start,startswith,stat,std,stdm,step,stride,strides,string,stringmime,strip,strwidth,sub2ind,subtypes,success,sum,sum!,sumabs,sumabs2,summary,super,supertype,svd,svdfact,svdfact!,svdvals,svdvals!,sylvester,symdiff,symdiff!,symlink,systemerror,take!,takebuf_array,takebuf_string,tan,tan_fast,tand,tanh,tanh_fast,task_local_storage,tempdir,tempname,thisind,tic,time,time_ns,timedwait,to_indices,toc,toq,touch,trace,trailing_ones,trailing_zeros,transcode,transpose,transpose!,tril,tril!,triu,triu!,trues,trunc,truncate,trylock,tryparse,typeintersect,typejoin,typemax,typemin,unescape_string,union,union!,unique,unique!,unlock,unmark,unsafe_copy!,unsafe_copyto!,unsafe_load,unsafe_pointer_to_objref,unsafe_read,unsafe_store!,unsafe_string,unsafe_trunc,unsafe_wrap,unsafe_write,unshift!,unsigned,uperm,valtype,values,var,varinfo,varm,vcat,vec,vecdot,vecnorm,versioninfo,view,wait,walkdir,warn,which,whos,widemul,widen,withenv,workspace,write,xcorr,xor,yield,yieldto,zero,zeros,zip,broadcast_getindex,broadcast_indices,broadcast_setindex!,broadcast_similar,dotview,apropos,doc,countfrom,cycle,drop,enumerate,flatten,partition,product,repeated,rest,take,zip,get_creds!,with,calloc,errno,flush_cstdio,free,gethostname,getpid,malloc,realloc,strerror,strftime,strptime,systemsleep,time,transcode,dlclose,dlext,dllist,dlopen,dlopen_e,dlpath,dlsym,dlsym_e,find_library,adjoint,adjoint!,axpby!,axpy!,bkfact,bkfact!,chol,cholfact,cholfact!,cond,condskeel,copy_transpose!,copyto!,cross,det,diag,diagind,diagm,diff,dot,eig,eigfact,eigfact!,eigmax,eigmin,eigvals,eigvals!,eigvecs,factorize,getq,givens,gradient,hessfact,hessfact!,isdiag,ishermitian,isposdef,isposdef!,issuccess,issymmetric,istril,istriu,kron,ldltfact,ldltfact!,linreg,logabsdet,logdet,lq,lqfact,lqfact!,lu,lufact,lufact!,lyap,norm,normalize,normalize!,nullspace,ordschur,ordschur!,peakflops,pinv,qr,qrfact,qrfact!,rank,scale!,schur,schurfact,schurfact!,svd,svdfact,svdfact!,svdvals,svdvals!,sylvester,trace,transpose,transpose!,transpose_type,tril,tril!,triu,triu!,vecdot,vecnorm,html,latex,license,readme,isexpr,quot,show_sexpr,add,available,build,checkout,clone,dir,free,init,installed,pin,resolve,rm,setprotocol!,status,test,update,deserialize,serialize,blkdiag,droptol!,dropzeros,dropzeros!,issparse,nnz,nonzeros,nzrange,permute,rowvals,sparse,sparsevec,spdiagm,spones,sprand,sprandn,spzeros,catch_stacktrace,stacktrace,cpu_info,cpu_summary,free_memory,isapple,isbsd,islinux,isunix,iswindows,loadavg,total_memory,uptime,atomic_add!,atomic_and!,atomic_cas!,atomic_fence,atomic_max!,atomic_min!,atomic_nand!,atomic_or!,atomic_sub!,atomic_xchg!,atomic_xor!,nthreads,threadid,applicable,eval,fieldtype,getfield,invoke,isa,isdefined,nfields,nothing,setfield!,throw,tuple,typeassert,typeof,uninitialized,undef,
    AbstractArray,AbstractChannel,AbstractDict,AbstractDisplay,AbstractFloat,AbstractIrrational,AbstractMatrix,AbstractRNG,AbstractRange,AbstractSerializer,AbstractSet,AbstractSparseArray,AbstractSparseMatrix,AbstractSparseVector,AbstractString,AbstractUnitRange,AbstractVecOrMat,AbstractVector,Adjoint,Any,ArgumentError,Array,AssertionError,Bidiagonal,BigFloat,BigInt,BitArray,BitMatrix,BitSet,BitVector,Bool,BoundsError,BufferStream,CapturedException,CartesianIndex,CartesianIndices,Cchar,Cdouble,Cfloat,Channel,Char,Cint,Cintmax_t,Clong,Clonglong,Cmd,CodeInfo,Colon,Complex,ComplexF16,ComplexF32,ComplexF64,CompositeException,Condition,ConjArray,ConjMatrix,ConjVector,Cptrdiff_t,Cshort,Csize_t,Cssize_t,Cstring,Cuchar,Cuint,Cuintmax_t,Culong,Culonglong,Cushort,Cvoid,Cwchar_t,Cwstring,DataType,DenseArray,DenseMatrix,DenseVecOrMat,DenseVector,Diagonal,Dict,DimensionMismatch,Dims,DivideError,DomainError,EOFError,EachLine,Enum,Enumerate,ErrorException,Exception,ExponentialBackOff,Expr,Factorization,Float16,Float32,Float64,Function,GlobalRef,GotoNode,HTML,Hermitian,IO,IOBuffer,IOContext,IOStream,IPAddr,IPv4,IPv6,IndexCartesian,IndexLinear,IndexStyle,InexactError,InitError,Int,Int128,Int16,Int32,Int64,Int8,Integer,InterruptException,InvalidStateException,Irrational,KeyError,LabelNode,LinSpace,LineNumberNode,LinearIndices,LoadError,LowerTriangular,MIME,Matrix,MersenneTwister,Method,MethodError,MethodTable,Missing,MissingException,Module,NTuple,NamedTuple,NewvarNode,Nothing,Number,ObjectIdDict,OrdinalRange,OutOfMemoryError,OverflowError,Pair,PartialQuickSort,PermutedDimsArray,Pipe,Ptr,QuoteNode,RandomDevice,Rational,RawFD,ReadOnlyMemoryError,Real,ReentrantLock,Ref,Regex,RegexMatch,RoundingMode,RowVector,SSAValue,SegmentationFault,SerializationState,Set,Signed,SimpleVector,Slot,SlotNumber,Some,SparseMatrixCSC,SparseVector,StackFrame,StackOverflowError,StackTrace,StepRange,StepRangeLen,StridedArray,StridedMatrix,StridedVecOrMat,StridedVector,String,StringIndexError,SubArray,SubString,SymTridiagonal,Symbol,Symmetric,SystemError,TCPSocket,Task,Text,TextDisplay,Timer,Transpose,Tridiagonal,Tuple,Type,TypeError,TypeMapEntry,TypeMapLevel,TypeName,TypeVar,TypedSlot,UDPSocket,UInt,UInt128,UInt16,UInt32,UInt64,UInt8,UndefRefError,UndefVarError,UniformScaling,Uninitialized,Union,UnionAll,UnitRange,Unsigned,UpperTriangular,Val,Vararg,VecElement,VecOrMat,Vector,VersionNumber,WeakKeyDict,WeakRef,BLAS,Base,Broadcast,DFT,Docs,Iterators,LAPACK,LibGit2,Libc,Libdl,LinAlg,Markdown,Meta,Operators,Pkg,Serializer,SparseArrays,StackTraces,Sys,Threads,Core,Main, semicircle, sample, plot!, plot, xlims!, savefig, GOE_eigvals, append!, histogram,
    solve, Tsit5, ODEProblem, tracywidomODE!, airy, TracyWIdomPDF_via_ODE, @parallel, @everywhere, @distributed,
    wireframe, Hist2D, bincenters, bincounts, scatter!, bar, patiencesort, derivative, Polynomial, newton},%
    % Blue keywords
    keywords=[3]{const, abstract, type, mutable, struct, function, true, false, nothing, missing, macro, quote, module, baremodule, local, global},
    % "Numbers"
    keywords=[4]{π, im},
    sensitive=true,
    morecomment=[l]{\#},
    morecomment=[n]{\#=}{=\#},
    morestring=[s]{"}{"},
    morestring=[m]{'}{'},
    literate=*{-}{-}1,
    alsoletter=!?
}

% This defines the styles for the code blocks
\lstdefinestyle{julia}{
    backgroundcolor  = \color[HTML]{1E1E1E},
    basicstyle       = \JuliaMonoRegular\notsotiny\color[HTML]{D4D4D4},
    keywordstyle     = [1]{\JuliaMonoRegular\color[HTML]{C586C0}},
    keywordstyle     = [2]{\JuliaMonoRegular\color[HTML]{DCDCAA}},
    keywordstyle     = [3]{\JuliaMonoRegular\color[HTML]{0F6FA3}},
    keywordstyle     = [4]{\JuliaMonoRegular\color[HTML]{569CD6}},
    keywordstyle     = [5]{\JuliaMonoRegular\color[HTML]{B5CEA8}},
    stringstyle      = \JuliaMonoRegular\color[HTML]{CE9178},
    commentstyle     = \color[HTML]{6A9955},
    rulecolor        = \color[HTML]{000000},
    tabsize=4,
    captionpos=b,
    breaklines=true,
    breakatwhitespace=false,
    showstringspaces=false,
    showspaces=false,
    showtabs=false,
    columns=fullflexible,
    keepspaces=true,
    numbers=none % this removes the line numbers
}

% this defines the inline style
\lstdefinestyle{juliainline}{
    backgroundcolor  = \color[HTML]{1E1E1E},
    basicstyle       = \JuliaMonoRegular\scriptsize\color[HTML]{000000},
    tabsize=4,
    captionpos=b,
    breaklines=true,
    breakatwhitespace=false,
    showstringspaces=false,
    showspaces=false,
    showtabs=false,
    columns=fullflexible,
    keepspaces=true,
    numbers=left
}

==> julia_listings_unicode.tex <==
% set lstlisting to accept full Julia unicode support
\makeatletter
\lst@InputCatcodes
\def\lst@DefEC{%
 \lst@CCECUse \lst@ProcessLetter
  % 2-digit hex
  ^^a1% ¡   \exclamdown Inverted Exclamation Mark
  ^^a3% £   \sterling   Pound Sign
  ^^a5% ¥   \yen    Yen Sign
  ^^a6% ¦   \brokenbar  Broken Bar / Broken Vertical Bar
  ^^a7% §   \S  Section Sign
  ^^a9% ©   \copyright, \:copyright:    Copyright Sign
  ^^aa% ª   \ordfeminine    Feminine Ordinal Indicator
  ^^ac% ¬   \neg    Not Sign
  ^^ae% ®   \circledR, \:registered:    Registered Sign / Registered Trade Mark Sign
  ^^af% ¯   \highminus  Macron / Spacing Macron
  ^^b0% °   \degree Degree Sign
  ^^b1% ±   \pm Plus-Minus Sign / Plus-Or-Minus Sign
  ^^b2% ²   \^2 Superscript Two / Superscript Digit Two
  ^^b3% ³   \^3 Superscript Three / Superscript Digit Three
  ^^b6% ¶   \P  Pilcrow Sign / Paragraph Sign
  ^^b7% ·   \cdotp  Middle Dot
  ^^b9% ¹   \^1 Superscript One / Superscript Digit One
  ^^ba% º   \ordmasculine   Masculine Ordinal Indicator
  ^^bc% ¼   \1/4    Vulgar Fraction One Quarter / Fraction One Quarter
  ^^bd% ½   \1/2    Vulgar Fraction One Half / Fraction One Half
  ^^be% ¾   \3/4    Vulgar Fraction Three Quarters / Fraction Three Quarters
  ^^bf% ¿   \questiondown   Inverted Question Mark
  ^^c5% Å   \AA Latin Capital Letter A With Ring Above / Latin Capital Letter A Ring
  ^^c6% Æ   \AE Latin Capital Letter Ae / Latin Capital Letter A E
  ^^d0% Ð   \DH Latin Capital Letter Eth
  ^^d7% ×   \times  Multiplication Sign
  ^^d8% Ø   \O  Latin Capital Letter O With Stroke / Latin Capital Letter O Slash
  ^^de% Þ   \TH Latin Capital Letter Thorn
  ^^df% ß   \ss Latin Small Letter Sharp S
  ^^e5% å   \aa Latin Small Letter A With Ring Above / Latin Small Letter A Ring
  ^^e6% æ   \ae Latin Small Letter Ae / Latin Small Letter A E
  ^^f0% ð   \eth, \dh   Latin Small Letter Eth
  ^^f7% ÷   \div    Division Sign
  ^^f8% ø   \o  Latin Small Letter O With Stroke / Latin Small Letter O Slash
  ^^fe% þ   \th Latin Small Letter Thorn
  % zero-padded 4-digit hex
  ^^^^0110% Đ   \DJ Latin Capital Letter D With Stroke / Latin Capital Letter D Bar
  ^^^^0111% đ   \dj Latin Small Letter D With Stroke / Latin Small Letter D Bar
  ^^^^0127% ħ   \hbar   Latin Small Letter H With Stroke / Latin Small Letter H Bar
  ^^^^0131% ı   \imath  Latin Small Letter Dotless I
  ^^^^0141% Ł   \L  Latin Capital Letter L With Stroke / Latin Capital Letter L Slash
  ^^^^0142% ł   \l  Latin Small Letter L With Stroke / Latin Small Letter L Slash
  ^^^^014a% Ŋ   \NG Latin Capital Letter Eng
  ^^^^014b% ŋ   \ng Latin Small Letter Eng
  ^^^^0152% Œ   \OE Latin Capital Ligature Oe / Latin Capital Letter O E
  ^^^^0153% œ   \oe Latin Small Ligature Oe / Latin Small Letter O E
  ^^^^0195% ƕ   \hvlig  Latin Small Letter Hv / Latin Small Letter H V
  ^^^^019e% ƞ   \nrleg  Latin Small Letter N With Long Right Leg
  ^^^^01b5% Ƶ   \Zbar   Latin Capital Letter Z With Stroke / Latin Capital Letter Z Bar
  ^^^^01c2% ǂ   \doublepipe Latin Letter Alveolar Click / Latin Letter Pipe Double Bar
  ^^^^0237% ȷ   \jmath  Latin Small Letter Dotless J
  ^^^^0250% ɐ   \trna   Latin Small Letter Turned A
  ^^^^0252% ɒ   \trnsa  Latin Small Letter Turned Alpha / Latin Small Letter Turned Script A
  ^^^^0254% ɔ   \openo  Latin Small Letter Open O
  ^^^^0256% ɖ   \rtld   Latin Small Letter D With Tail / Latin Small Letter D Retroflex Hook
  ^^^^0259% ə   \schwa  Latin Small Letter Schwa
  ^^^^0263% ɣ   \pgamma Latin Small Letter Gamma
  ^^^^0264% ɤ   \pbgam  Latin Small Letter Rams Horn / Latin Small Letter Baby Gamma
  ^^^^0265% ɥ   \trnh   Latin Small Letter Turned H
  ^^^^026c% ɬ   \btdl   Latin Small Letter L With Belt / Latin Small Letter L Belt
  ^^^^026d% ɭ   \rtll   Latin Small Letter L With Retroflex Hook / Latin Small Letter L Retroflex Hook
  ^^^^026f% ɯ   \trnm   Latin Small Letter Turned M
  ^^^^0270% ɰ   \trnmlr Latin Small Letter Turned M With Long Leg
  ^^^^0271% ɱ   \ltlmr  Latin Small Letter M With Hook / Latin Small Letter M Hook
  ^^^^0272% ɲ   \ltln   Latin Small Letter N With Left Hook / Latin Small Letter N Hook
  ^^^^0273% ɳ   \rtln   Latin Small Letter N With Retroflex Hook / Latin Small Letter N Retroflex Hook
  ^^^^0277% ɷ   \clomeg Latin Small Letter Closed Omega
  ^^^^0278% ɸ   \ltphi  Latin Small Letter Phi
  ^^^^0279% ɹ   \trnr   Latin Small Letter Turned R
  ^^^^027a% ɺ   \trnrl  Latin Small Letter Turned R With Long Leg
  ^^^^027b% ɻ   \rttrnr Latin Small Letter Turned R With Hook / Latin Small Letter Turned R Hook
  ^^^^027c% ɼ   \rl Latin Small Letter R With Long Leg
  ^^^^027d% ɽ   \rtlr   Latin Small Letter R With Tail / Latin Small Letter R Hook
  ^^^^027e% ɾ   \fhr    Latin Small Letter R With Fishhook / Latin Small Letter Fishhook R
  ^^^^0282% ʂ   \rtls   Latin Small Letter S With Hook / Latin Small Letter S Hook
  ^^^^0283% ʃ   \esh    Latin Small Letter Esh
  ^^^^0287% ʇ   \trnt   Latin Small Letter Turned T
  ^^^^0288% ʈ   \rtlt   Latin Small Letter T With Retroflex Hook / Latin Small Letter T Retroflex Hook
  ^^^^028a% ʊ   \pupsil Latin Small Letter Upsilon
  ^^^^028b% ʋ   \pscrv  Latin Small Letter V With Hook / Latin Small Letter Script V
  ^^^^028c% ʌ   \invv   Latin Small Letter Turned V
  ^^^^028d% ʍ   \invw   Latin Small Letter Turned W
  ^^^^028e% ʎ   \trny   Latin Small Letter Turned Y
  ^^^^0290% ʐ   \rtlz   Latin Small Letter Z With Retroflex Hook / Latin Small Letter Z Retroflex Hook
  ^^^^0292% ʒ   \yogh   Latin Small Letter Ezh / Latin Small Letter Yogh
  ^^^^0294% ʔ   \glst   Latin Letter Glottal Stop
  ^^^^0295% ʕ   \reglst Latin Letter Pharyngeal Voiced Fricative / Latin Letter Reversed Glottal Stop
  ^^^^0296% ʖ   \inglst Latin Letter Inverted Glottal Stop
  ^^^^029e% ʞ   \turnk  Latin Small Letter Turned K
  ^^^^02a4% ʤ   \dyogh  Latin Small Letter Dezh Digraph / Latin Small Letter D Yogh
  ^^^^02a7% ʧ   \tesh   Latin Small Letter Tesh Digraph / Latin Small Letter T Esh
  ^^^^02b0% ʰ   \^h Modifier Letter Small H
  ^^^^02b2% ʲ   \^j Modifier Letter Small J
  ^^^^02b3% ʳ   \^r Modifier Letter Small R
  ^^^^02b7% ʷ   \^w Modifier Letter Small W
  ^^^^02b8% ʸ   \^y Modifier Letter Small Y
  ^^^^02bc% ʼ   \rasp   Modifier Letter Apostrophe
  ^^^^02c8% ˈ   \verts  Modifier Letter Vertical Line
  ^^^^02cc% ˌ   \verti  Modifier Letter Low Vertical Line
  ^^^^02d0% ː   \lmrk   Modifier Letter Triangular Colon
  ^^^^02d1% ˑ   \hlmrk  Modifier Letter Half Triangular Colon
  ^^^^02d2% ˒   \sbrhr  Modifier Letter Centred Right Half Ring / Modifier Letter Centered Right Half Ring
  ^^^^02d3% ˓   \sblhr  Modifier Letter Centred Left Half Ring / Modifier Letter Centered Left Half Ring
  ^^^^02d4% ˔   \rais   Modifier Letter Up Tack
  ^^^^02d5% ˕   \low    Modifier Letter Down Tack
  ^^^^02d8% ˘   \u  Breve / Spacing Breve
  ^^^^02dc% ˜   \tildelow   Small Tilde / Spacing Tilde
  ^^^^02e1% ˡ   \^l Modifier Letter Small L
  ^^^^02e2% ˢ   \^s Modifier Letter Small S
  ^^^^02e3% ˣ   \^x Modifier Letter Small X
  ^^^^0300%  ̀  \grave  Combining Grave Accent / Non-Spacing Grave
  ^^^^0301%  ́  \acute  Combining Acute Accent / Non-Spacing Acute
  ^^^^0302%  ̂  \hat    Combining Circumflex Accent / Non-Spacing Circumflex
  ^^^^0303%  ̃  \tilde  Combining Tilde / Non-Spacing Tilde
  ^^^^0304%  ̄  \bar    Combining Macron / Non-Spacing Macron
  ^^^^0305%  ̅  \overbar    Combining Overline / Non-Spacing Overscore
  ^^^^0306%  ̆  \breve  Combining Breve / Non-Spacing Breve
  ^^^^0307%  ̇  \dot    Combining Dot Above / Non-Spacing Dot Above
  ^^^^0308%  ̈  \ddot   Combining Diaeresis / Non-Spacing Diaeresis
  ^^^^0309%  ̉  \ovhook Combining Hook Above / Non-Spacing Hook Above
  ^^^^030a%  ̊  \ocirc  Combining Ring Above / Non-Spacing Ring Above
  ^^^^030b%  ̋  \H  Combining Double Acute Accent / Non-Spacing Double Acute
  ^^^^030c%  ̌  \check  Combining Caron / Non-Spacing Hacek
  ^^^^0310%  ̐  \candra Combining Candrabindu / Non-Spacing Candrabindu
  ^^^^0312%  ̒  \oturnedcomma   Combining Turned Comma Above / Non-Spacing Turned Comma Above
  ^^^^0315%  ̕  \ocommatopright Combining Comma Above Right / Non-Spacing Comma Above Right
  ^^^^031a%  ̚  \droang Combining Left Angle Above / Non-Spacing Left Angle Above
  ^^^^0321%  ̡  \palh   Combining Palatalized Hook Below / Non-Spacing Palatalized Hook Below
  ^^^^0322%  ̢  \rh Combining Retroflex Hook Below / Non-Spacing Retroflex Hook Below
  ^^^^0327%  ̧  \c  Combining Cedilla / Non-Spacing Cedilla
  ^^^^0328%  ̨  \k  Combining Ogonek / Non-Spacing Ogonek
  ^^^^032a%  ̪  \sbbrg  Combining Bridge Below / Non-Spacing Bridge Below
  ^^^^0330%  ̰  \wideutilde Combining Tilde Below / Non-Spacing Tilde Below
  ^^^^0332%  ̲  \underbar   Combining Low Line / Non-Spacing Underscore
  ^^^^0336%  ̶  \strike, \sout  Combining Long Stroke Overlay / Non-Spacing Long Bar Overlay
  ^^^^0338%  ̸  \not    Combining Long Solidus Overlay / Non-Spacing Long Slash Overlay
  ^^^^034d%  ͍  \underleftrightarrow    Combining Left Right Arrow Below
  ^^^^0391% Α   \Alpha  Greek Capital Letter Alpha
  ^^^^0392% Β   \Beta   Greek Capital Letter Beta
  ^^^^0393% Γ   \Gamma  Greek Capital Letter Gamma
  ^^^^0394% Δ   \Delta  Greek Capital Letter Delta
  ^^^^0395% Ε   \Epsilon    Greek Capital Letter Epsilon
  ^^^^0396% Ζ   \Zeta   Greek Capital Letter Zeta
  ^^^^0397% Η   \Eta    Greek Capital Letter Eta
  ^^^^0398% Θ   \Theta  Greek Capital Letter Theta
  ^^^^0399% Ι   \Iota   Greek Capital Letter Iota
  ^^^^039a% Κ   \Kappa  Greek Capital Letter Kappa
  ^^^^039b% Λ   \Lambda Greek Capital Letter Lamda / Greek Capital Letter Lambda
  ^^^^039c% Μ   \upMu   Greek Capital Letter Mu
  ^^^^039d% Ν   \upNu   Greek Capital Letter Nu
  ^^^^039e% Ξ   \Xi Greek Capital Letter Xi
  ^^^^039f% Ο   \upOmicron  Greek Capital Letter Omicron
  ^^^^03a0% Π   \Pi Greek Capital Letter Pi
  ^^^^03a1% Ρ   \Rho    Greek Capital Letter Rho
  ^^^^03a3% Σ   \Sigma  Greek Capital Letter Sigma
  ^^^^03a4% Τ   \Tau    Greek Capital Letter Tau
  ^^^^03a5% Υ   \Upsilon    Greek Capital Letter Upsilon
  ^^^^03a6% Φ   \Phi    Greek Capital Letter Phi
  ^^^^03a7% Χ   \Chi    Greek Capital Letter Chi
  ^^^^03a8% Ψ   \Psi    Greek Capital Letter Psi
  ^^^^03a9% Ω   \Omega  Greek Capital Letter Omega
  ^^^^03b1% α   \alpha  Greek Small Letter Alpha
  ^^^^03b2% β   \beta   Greek Small Letter Beta
  ^^^^03b3% γ   \gamma  Greek Small Letter Gamma
  ^^^^03b4% δ   \delta  Greek Small Letter Delta
  ^^^^03b5% ε   \upepsilon, \varepsilon Greek Small Letter Epsilon
  ^^^^03b6% ζ   \zeta   Greek Small Letter Zeta
  ^^^^03b7% η   \eta    Greek Small Letter Eta
  ^^^^03b8% θ   \theta  Greek Small Letter Theta
  ^^^^03b9% ι   \iota   Greek Small Letter Iota
  ^^^^03ba% κ   \kappa  Greek Small Letter Kappa
  ^^^^03bb% λ   \lambda Greek Small Letter Lamda / Greek Small Letter Lambda
  ^^^^03bc% μ   \mu Greek Small Letter Mu
  ^^^^03bd% ν   \nu Greek Small Letter Nu
  ^^^^03be% ξ   \xi Greek Small Letter Xi
  ^^^^03bf% ο   \upomicron  Greek Small Letter Omicron
  ^^^^03c0% π   \pi Greek Small Letter Pi
  ^^^^03c1% ρ   \rho    Greek Small Letter Rho
  ^^^^03c2% ς   \varsigma   Greek Small Letter Final Sigma
  ^^^^03c3% σ   \sigma  Greek Small Letter Sigma
  ^^^^03c4% τ   \tau    Greek Small Letter Tau
  ^^^^03c5% υ   \upsilon    Greek Small Letter Upsilon
  ^^^^03c6% φ   \varphi Greek Small Letter Phi
  ^^^^03c7% χ   \chi    Greek Small Letter Chi
  ^^^^03c8% ψ   \psi    Greek Small Letter Psi
  ^^^^03c9% ω   \omega  Greek Small Letter Omega
  ^^^^03d0% ϐ   \upvarbeta  Greek Beta Symbol / Greek Small Letter Curled Beta
  ^^^^03d1% ϑ   \vartheta   Greek Theta Symbol / Greek Small Letter Script Theta
  ^^^^03d5% ϕ   \phi    Greek Phi Symbol / Greek Small Letter Script Phi
  ^^^^03d6% ϖ   \varpi  Greek Pi Symbol / Greek Small Letter Omega Pi
  ^^^^03d8% Ϙ   \upoldKoppa Greek Letter Archaic Koppa
  ^^^^03d9% ϙ   \upoldkoppa Greek Small Letter Archaic Koppa
  ^^^^03da% Ϛ   \Stigma Greek Letter Stigma / Greek Capital Letter Stigma
  ^^^^03db% ϛ   \upstigma   Greek Small Letter Stigma
  ^^^^03dc% Ϝ   \Digamma    Greek Letter Digamma / Greek Capital Letter Digamma
  ^^^^03dd% ϝ   \digamma    Greek Small Letter Digamma
  ^^^^03de% Ϟ   \Koppa  Greek Letter Koppa / Greek Capital Letter Koppa
  ^^^^03df% ϟ   \upkoppa    Greek Small Letter Koppa
  ^^^^03e0% Ϡ   \Sampi  Greek Letter Sampi / Greek Capital Letter Sampi
  ^^^^03e1% ϡ   \upsampi    Greek Small Letter Sampi
  ^^^^03f0% ϰ   \varkappa   Greek Kappa Symbol / Greek Small Letter Script Kappa
  ^^^^03f1% ϱ   \varrho Greek Rho Symbol / Greek Small Letter Tailed Rho
  ^^^^03f4% ϴ   \varTheta   Greek Capital Theta Symbol
  ^^^^03f5% ϵ   \epsilon    Greek Lunate Epsilon Symbol
  ^^^^03f6% ϶   \backepsilon    Greek Reversed Lunate Epsilon Symbol
  % 4-digit hex
  ^^^^1d2c% ᴬ   \^A Modifier Letter Capital A
  ^^^^1d2e% ᴮ   \^B Modifier Letter Capital B
  ^^^^1d30% ᴰ   \^D Modifier Letter Capital D
  ^^^^1d31% ᴱ   \^E Modifier Letter Capital E
  ^^^^1d33% ᴳ   \^G Modifier Letter Capital G
  ^^^^1d34% ᴴ   \^H Modifier Letter Capital H
  ^^^^1d35% ᴵ   \^I Modifier Letter Capital I
  ^^^^1d36% ᴶ   \^J Modifier Letter Capital J
  ^^^^1d37% ᴷ   \^K Modifier Letter Capital K
  ^^^^1d38% ᴸ   \^L Modifier Letter Capital L
  ^^^^1d39% ᴹ   \^M Modifier Letter Capital M
  ^^^^1d3a% ᴺ   \^N Modifier Letter Capital N
  ^^^^1d3c% ᴼ   \^O Modifier Letter Capital O
  ^^^^1d3e% ᴾ   \^P Modifier Letter Capital P
  ^^^^1d3f% ᴿ   \^R Modifier Letter Capital R
  ^^^^1d40% ᵀ   \^T Modifier Letter Capital T
  ^^^^1d41% ᵁ   \^U Modifier Letter Capital U
  ^^^^1d42% ᵂ   \^W Modifier Letter Capital W
  ^^^^1d43% ᵃ   \^a Modifier Letter Small A
  ^^^^1d45% ᵅ   \^alpha Modifier Letter Small Alpha
  ^^^^1d47% ᵇ   \^b Modifier Letter Small B
  ^^^^1d48% ᵈ   \^d Modifier Letter Small D
  ^^^^1d49% ᵉ   \^e Modifier Letter Small E
  ^^^^1d4b% ᵋ   \^epsilon   Modifier Letter Small Open E
  ^^^^1d4d% ᵍ   \^g Modifier Letter Small G
  ^^^^1d4f% ᵏ   \^k Modifier Letter Small K
  ^^^^1d50% ᵐ   \^m Modifier Letter Small M
  ^^^^1d52% ᵒ   \^o Modifier Letter Small O
  ^^^^1d56% ᵖ   \^p Modifier Letter Small P
  ^^^^1d57% ᵗ   \^t Modifier Letter Small T
  ^^^^1d58% ᵘ   \^u Modifier Letter Small U
  ^^^^1d5b% ᵛ   \^v Modifier Letter Small V
  ^^^^1d5d% ᵝ   \^beta  Modifier Letter Small Beta
  ^^^^1d5e% ᵞ   \^gamma Modifier Letter Small Greek Gamma
  ^^^^1d5f% ᵟ   \^delta Modifier Letter Small Delta
  ^^^^1d60% ᵠ   \^phi   Modifier Letter Small Greek Phi
  ^^^^1d61% ᵡ   \^chi   Modifier Letter Small Chi
  ^^^^1d62% ᵢ   \_i Latin Subscript Small Letter I
  ^^^^1d63% ᵣ   \_r Latin Subscript Small Letter R
  ^^^^1d64% ᵤ   \_u Latin Subscript Small Letter U
  ^^^^1d65% ᵥ   \_v Latin Subscript Small Letter V
  ^^^^1d66% ᵦ   \_beta  Greek Subscript Small Letter Beta
  ^^^^1d67% ᵧ   \_gamma Greek Subscript Small Letter Gamma
  ^^^^1d68% ᵨ   \_rho   Greek Subscript Small Letter Rho
  ^^^^1d69% ᵩ   \_phi   Greek Subscript Small Letter Phi
  ^^^^1d6a% ᵪ   \_chi   Greek Subscript Small Letter Chi
  ^^^^1d9c% ᶜ   \^c Modifier Letter Small C
  ^^^^1da0% ᶠ   \^f Modifier Letter Small F
  ^^^^1da5% ᶥ   \^iota  Modifier Letter Small Iota
  ^^^^1db2% ᶲ   \^Phi   Modifier Letter Small Phi
  ^^^^1dbb% ᶻ   \^z Modifier Letter Small Z
  ^^^^1dbf% ᶿ   \^theta Modifier Letter Small Theta
  ^^^^2002%     \enspace    En Space
  ^^^^2003%     \quad   Em Space
  ^^^^2005%     \thickspace Four-Per-Em Space
  ^^^^2009%     \thinspace  Thin Space
  ^^^^200a%     \hspace Hair Space
  ^^^^2013% –   \endash En Dash
  ^^^^2014% —   \emdash Em Dash
  ^^^^2016% ‖   \Vert   Double Vertical Line / Double Vertical Bar
  ^^^^2018% ‘   \lq Left Single Quotation Mark / Single Turned Comma Quotation Mark
  ^^^^2019% ’   \rq Right Single Quotation Mark / Single Comma Quotation Mark
  ^^^^201b% ‛   \reapos Single High-Reversed-9 Quotation Mark / Single Reversed Comma Quotation Mark
  ^^^^201c% “   \quotedblleft   Left Double Quotation Mark / Double Turned Comma Quotation Mark
  ^^^^201d% ”   \quotedblright  Right Double Quotation Mark / Double Comma Quotation Mark
  ^^^^2020% †   \dagger Dagger
  ^^^^2021% ‡   \ddagger    Double Dagger
  ^^^^2022% •   \bullet Bullet
  ^^^^2026% …   \dots, \ldots   Horizontal Ellipsis
  ^^^^2030% ‰   \perthousand    Per Mille Sign
  ^^^^2031% ‱   \pertenthousand Per Ten Thousand Sign
  ^^^^2032% ′   \prime  Prime
  ^^^^2033% ″   \pprime Double Prime
  ^^^^2034% ‴   \ppprime    Triple Prime
  ^^^^2035% ‵   \backprime  Reversed Prime
  ^^^^2036% ‶   \backpprime Reversed Double Prime
  ^^^^2037% ‷   \backppprime    Reversed Triple Prime
  ^^^^2039% ‹   \guilsinglleft  Single Left-Pointing Angle Quotation Mark / Left Pointing Single Guillemet
  ^^^^203a% ›   \guilsinglright Single Right-Pointing Angle Quotation Mark / Right Pointing Single Guillemet
  ^^^^203c% ‼   \:bangbang: Double Exclamation Mark
  ^^^^2040% ⁀   \tieconcat  Character Tie
  ^^^^2049% ⁉   \:interrobang:  Exclamation Question Mark
  ^^^^2057% ⁗   \pppprime   Quadruple Prime
  ^^^^205d% ⁝   \tricolon   Tricolon
  ^^^^2060% ⁠   \nolinebreak    Word Joiner
  ^^^^2070% ⁰   \^0 Superscript Zero / Superscript Digit Zero
  ^^^^2071% ⁱ   \^i Superscript Latin Small Letter I
  ^^^^2074% ⁴   \^4 Superscript Four / Superscript Digit Four
  ^^^^2075% ⁵   \^5 Superscript Five / Superscript Digit Five
  ^^^^2076% ⁶   \^6 Superscript Six / Superscript Digit Six
  ^^^^2077% ⁷   \^7 Superscript Seven / Superscript Digit Seven
  ^^^^2078% ⁸   \^8 Superscript Eight / Superscript Digit Eight
  ^^^^2079% ⁹   \^9 Superscript Nine / Superscript Digit Nine
  ^^^^207a% ⁺   \^+ Superscript Plus Sign
  ^^^^207b% ⁻   \^- Superscript Minus / Superscript Hyphen-Minus
  ^^^^207c% ⁼   \^= Superscript Equals Sign
  ^^^^207d% ⁽   \^( Superscript Left Parenthesis / Superscript Opening Parenthesis
  ^^^^207e% ⁾   \^) Superscript Right Parenthesis / Superscript Closing Parenthesis
  ^^^^207f% ⁿ   \^n Superscript Latin Small Letter N
  ^^^^2080% ₀   \_0 Subscript Zero / Subscript Digit Zero
  ^^^^2081% ₁   \_1 Subscript One / Subscript Digit One
  ^^^^2082% ₂   \_2 Subscript Two / Subscript Digit Two
  ^^^^2083% ₃   \_3 Subscript Three / Subscript Digit Three
  ^^^^2084% ₄   \_4 Subscript Four / Subscript Digit Four
  ^^^^2085% ₅   \_5 Subscript Five / Subscript Digit Five
  ^^^^2086% ₆   \_6 Subscript Six / Subscript Digit Six
  ^^^^2087% ₇   \_7 Subscript Seven / Subscript Digit Seven
  ^^^^2088% ₈   \_8 Subscript Eight / Subscript Digit Eight
  ^^^^2089% ₉   \_9 Subscript Nine / Subscript Digit Nine
  ^^^^208a% ₊   \_+ Subscript Plus Sign
  ^^^^208b% ₋   \_- Subscript Minus / Subscript Hyphen-Minus
  ^^^^208c% ₌   \_= Subscript Equals Sign
  ^^^^208d% ₍   \_( Subscript Left Parenthesis / Subscript Opening Parenthesis
  ^^^^208e% ₎   \_) Subscript Right Parenthesis / Subscript Closing Parenthesis
  ^^^^2090% ₐ   \_a Latin Subscript Small Letter A
  ^^^^2091% ₑ   \_e Latin Subscript Small Letter E
  ^^^^2092% ₒ   \_o Latin Subscript Small Letter O
  ^^^^2093% ₓ   \_x Latin Subscript Small Letter X
  ^^^^2094% ₔ   \_schwa Latin Subscript Small Letter Schwa
  ^^^^2095% ₕ   \_h Latin Subscript Small Letter H
  ^^^^2096% ₖ   \_k Latin Subscript Small Letter K
  ^^^^2097% ₗ   \_l Latin Subscript Small Letter L
  ^^^^2098% ₘ   \_m Latin Subscript Small Letter M
  ^^^^2099% ₙ   \_n Latin Subscript Small Letter N
  ^^^^209a% ₚ   \_p Latin Subscript Small Letter P
  ^^^^209b% ₛ   \_s Latin Subscript Small Letter S
  ^^^^209c% ₜ   \_t Latin Subscript Small Letter T
  ^^^^20a7% ₧   \pes    Peseta Sign
  ^^^^20ac% €   \euro   Euro Sign
  ^^^^20d0%  ⃐  \leftharpoonaccent  Combining Left Harpoon Above / Non-Spacing Left Harpoon Above
  ^^^^20d1%  ⃑  \rightharpoonaccent Combining Right Harpoon Above / Non-Spacing Right Harpoon Above
  ^^^^20d2%  ⃒  \vertoverlay    Combining Long Vertical Line Overlay / Non-Spacing Long Vertical Bar Overlay
  ^^^^20d6%  ⃖  \overleftarrow  Combining Left Arrow Above / Non-Spacing Left Arrow Above
  ^^^^20d7%  ⃗  \vec    Combining Right Arrow Above / Non-Spacing Right Arrow Above
  ^^^^20db%  ⃛  \dddot  Combining Three Dots Above / Non-Spacing Three Dots Above
  ^^^^20dc%  ⃜  \ddddot Combining Four Dots Above / Non-Spacing Four Dots Above
  ^^^^20dd%  ⃝  \enclosecircle  Combining Enclosing Circle / Enclosing Circle
  ^^^^20de%  ⃞  \enclosesquare  Combining Enclosing Square / Enclosing Square
  ^^^^20df%  ⃟  \enclosediamond Combining Enclosing Diamond / Enclosing Diamond
  ^^^^20e1%  ⃡  \overleftrightarrow Combining Left Right Arrow Above / Non-Spacing Left Right Arrow Above
  ^^^^20e4%  ⃤  \enclosetriangle    Combining Enclosing Upward Pointing Triangle
  ^^^^20e7%  ⃧  \annuity    Combining Annuity Symbol
  ^^^^20e8%  ⃨  \threeunderdot  Combining Triple Underdot
  ^^^^20e9%  ⃩  \widebridgeabove    Combining Wide Bridge Above
  ^^^^20ec%  ⃬  \underrightharpoondown  Combining Rightwards Harpoon With Barb Downwards
  ^^^^20ed%  ⃭  \underleftharpoondown   Combining Leftwards Harpoon With Barb Downwards
  ^^^^20ee%  ⃮  \underleftarrow Combining Left Arrow Below
  ^^^^20ef%  ⃯  \underrightarrow    Combining Right Arrow Below
  ^^^^20f0%  ⃰  \asteraccent    Combining Asterisk Above
  ^^^^2102% ℂ   \bbC    Double-Struck Capital C / Double-Struck C
  ^^^^2107% ℇ   \eulermascheroni    Euler Constant / Eulers
  ^^^^210a% ℊ   \scrg   Script Small G
  ^^^^210b% ℋ   \scrH   Script Capital H / Script H
  ^^^^210c% ℌ   \frakH  Black-Letter Capital H / Black-Letter H
  ^^^^210d% ℍ   \bbH    Double-Struck Capital H / Double-Struck H
  ^^^^210e% ℎ   \planck Planck Constant
  ^^^^210f% ℏ   \hslash Planck Constant Over Two Pi / Planck Constant Over 2 Pi
  ^^^^2110% ℐ   \scrI   Script Capital I / Script I
  ^^^^2111% ℑ   \Im Black-Letter Capital I / Black-Letter I
  ^^^^2112% ℒ   \scrL   Script Capital L / Script L
  ^^^^2113% ℓ   \ell    Script Small L
  ^^^^2115% ℕ   \bbN    Double-Struck Capital N / Double-Struck N
  ^^^^2116% №   \numero Numero Sign / Numero
  ^^^^2118% ℘   \wp Script Capital P / Script P
  ^^^^2119% ℙ   \bbP    Double-Struck Capital P / Double-Struck P
  ^^^^211a% ℚ   \bbQ    Double-Struck Capital Q / Double-Struck Q
  ^^^^211b% ℛ   \scrR   Script Capital R / Script R
  ^^^^211c% ℜ   \Re Black-Letter Capital R / Black-Letter R
  ^^^^211d% ℝ   \bbR    Double-Struck Capital R / Double-Struck R
  ^^^^211e% ℞   \xrat   Prescription Take
  ^^^^2122% ™   \trademark, \:tm:   Trade Mark Sign / Trademark
  ^^^^2124% ℤ   \bbZ    Double-Struck Capital Z / Double-Struck Z
  ^^^^2126% Ω   \ohm    Ohm Sign / Ohm
  ^^^^2127% ℧   \mho    Inverted Ohm Sign / Mho
  ^^^^2128% ℨ   \frakZ  Black-Letter Capital Z / Black-Letter Z
  ^^^^2129% ℩   \turnediota Turned Greek Small Letter Iota
  ^^^^212b% Å   \Angstrom   Angstrom Sign / Angstrom Unit
  ^^^^212c% ℬ   \scrB   Script Capital B / Script B
  ^^^^212d% ℭ   \frakC  Black-Letter Capital C / Black-Letter C
  ^^^^212f% ℯ   \scre, \euler   Script Small E
  ^^^^2130% ℰ   \scrE   Script Capital E / Script E
  ^^^^2131% ℱ   \scrF   Script Capital F / Script F
  ^^^^2132% Ⅎ   \Finv   Turned Capital F / Turned F
  ^^^^2133% ℳ   \scrM   Script Capital M / Script M
  ^^^^2134% ℴ   \scro   Script Small O
  ^^^^2135% ℵ   \aleph  Alef Symbol / First Transfinite Cardinal
  ^^^^2136% ℶ   \beth   Bet Symbol / Second Transfinite Cardinal
  ^^^^2137% ℷ   \gimel  Gimel Symbol / Third Transfinite Cardinal
  ^^^^2138% ℸ   \daleth Dalet Symbol / Fourth Transfinite Cardinal
  ^^^^2139% ℹ   \:information_source:   Information Source
  ^^^^213c% ℼ   \bbpi   Double-Struck Small Pi
  ^^^^213d% ℽ   \bbgamma    Double-Struck Small Gamma
  ^^^^213e% ℾ   \bbGamma    Double-Struck Capital Gamma
  ^^^^213f% ℿ   \bbPi   Double-Struck Capital Pi
  ^^^^2140% ⅀   \bbsum  Double-Struck N-Ary Summation
  ^^^^2141% ⅁   \Game   Turned Sans-Serif Capital G
  ^^^^2142% ⅂   \sansLturned    Turned Sans-Serif Capital L
  ^^^^2143% ⅃   \sansLmirrored  Reversed Sans-Serif Capital L
  ^^^^2144% ⅄   \Yup    Turned Sans-Serif Capital Y
  ^^^^2145% ⅅ   \bbiD   Double-Struck Italic Capital D
  ^^^^2146% ⅆ   \bbid   Double-Struck Italic Small D
  ^^^^2147% ⅇ   \bbie   Double-Struck Italic Small E
  ^^^^2148% ⅈ   \bbii   Double-Struck Italic Small I
  ^^^^2149% ⅉ   \bbij   Double-Struck Italic Small J
  ^^^^214a% ⅊   \PropertyLine   Property Line
  ^^^^214b% ⅋   \upand  Turned Ampersand
  ^^^^2150% ⅐   \1/7    Vulgar Fraction One Seventh
  ^^^^2151% ⅑   \1/9    Vulgar Fraction One Ninth
  ^^^^2152% ⅒   \1/10   Vulgar Fraction One Tenth
  ^^^^2153% ⅓   \1/3    Vulgar Fraction One Third / Fraction One Third
  ^^^^2154% ⅔   \2/3    Vulgar Fraction Two Thirds / Fraction Two Thirds
  ^^^^2155% ⅕   \1/5    Vulgar Fraction One Fifth / Fraction One Fifth
  ^^^^2156% ⅖   \2/5    Vulgar Fraction Two Fifths / Fraction Two Fifths
  ^^^^2157% ⅗   \3/5    Vulgar Fraction Three Fifths / Fraction Three Fifths
  ^^^^2158% ⅘   \4/5    Vulgar Fraction Four Fifths / Fraction Four Fifths
  ^^^^2159% ⅙   \1/6    Vulgar Fraction One Sixth / Fraction One Sixth
  ^^^^215a% ⅚   \5/6    Vulgar Fraction Five Sixths / Fraction Five Sixths
  ^^^^215b% ⅛   \1/8    Vulgar Fraction One Eighth / Fraction One Eighth
  ^^^^215c% ⅜   \3/8    Vulgar Fraction Three Eighths / Fraction Three Eighths
  ^^^^215d% ⅝   \5/8    Vulgar Fraction Five Eighths / Fraction Five Eighths
  ^^^^215e% ⅞   \7/8    Vulgar Fraction Seven Eighths / Fraction Seven Eighths
  ^^^^215f% ⅟   \1/ Fraction Numerator One
  ^^^^2189% ↉   \0/3    Vulgar Fraction Zero Thirds
  ^^^^2190% ←   \leftarrow  Leftwards Arrow / Left Arrow
  ^^^^2191% ↑   \uparrow    Upwards Arrow / Up Arrow
  ^^^^2192% →   \to, \rightarrow    Rightwards Arrow / Right Arrow
  ^^^^2193% ↓   \downarrow  Downwards Arrow / Down Arrow
  ^^^^2194% ↔   \leftrightarrow, \:left_right_arrow:    Left Right Arrow
  ^^^^2195% ↕   \updownarrow, \:arrow_up_down:  Up Down Arrow
  ^^^^2196% ↖   \nwarrow, \:arrow_upper_left:   North West Arrow / Upper Left Arrow
  ^^^^2197% ↗   \nearrow, \:arrow_upper_right:  North East Arrow / Upper Right Arrow
  ^^^^2198% ↘   \searrow, \:arrow_lower_right:  South East Arrow / Lower Right Arrow
  ^^^^2199% ↙   \swarrow, \:arrow_lower_left:   South West Arrow / Lower Left Arrow
  ^^^^219a% ↚   \nleftarrow Leftwards Arrow With Stroke / Left Arrow With Stroke
  ^^^^219b% ↛   \nrightarrow    Rightwards Arrow With Stroke / Right Arrow With Stroke
  ^^^^219c% ↜   \leftwavearrow  Leftwards Wave Arrow / Left Wave Arrow
  ^^^^219d% ↝   \rightwavearrow Rightwards Wave Arrow / Right Wave Arrow
  ^^^^219e% ↞   \twoheadleftarrow   Leftwards Two Headed Arrow / Left Two Headed Arrow
  ^^^^219f% ↟   \twoheaduparrow Upwards Two Headed Arrow / Up Two Headed Arrow
  ^^^^21a0% ↠   \twoheadrightarrow  Rightwards Two Headed Arrow / Right Two Headed Arrow
  ^^^^21a1% ↡   \twoheaddownarrow   Downwards Two Headed Arrow / Down Two Headed Arrow
  ^^^^21a2% ↢   \leftarrowtail  Leftwards Arrow With Tail / Left Arrow With Tail
  ^^^^21a3% ↣   \rightarrowtail Rightwards Arrow With Tail / Right Arrow With Tail
  ^^^^21a4% ↤   \mapsfrom   Leftwards Arrow From Bar / Left Arrow From Bar
  ^^^^21a5% ↥   \mapsup Upwards Arrow From Bar / Up Arrow From Bar
  ^^^^21a6% ↦   \mapsto Rightwards Arrow From Bar / Right Arrow From Bar
  ^^^^21a7% ↧   \mapsdown   Downwards Arrow From Bar / Down Arrow From Bar
  ^^^^21a8% ↨   \updownarrowbar Up Down Arrow With Base
  ^^^^21a9% ↩   \hookleftarrow, \:leftwards_arrow_with_hook:    Leftwards Arrow With Hook / Left Arrow With Hook
  ^^^^21aa% ↪   \hookrightarrow, \:arrow_right_hook:    Rightwards Arrow With Hook / Right Arrow With Hook
  ^^^^21ab% ↫   \looparrowleft  Leftwards Arrow With Loop / Left Arrow With Loop
  ^^^^21ac% ↬   \looparrowright Rightwards Arrow With Loop / Right Arrow With Loop
  ^^^^21ad% ↭   \leftrightsquigarrow    Left Right Wave Arrow
  ^^^^21ae% ↮   \nleftrightarrow    Left Right Arrow With Stroke
  ^^^^21af% ↯   \downzigzagarrow    Downwards Zigzag Arrow / Down Zigzag Arrow
  ^^^^21b0% ↰   \Lsh    Upwards Arrow With Tip Leftwards / Up Arrow With Tip Left
  ^^^^21b1% ↱   \Rsh    Upwards Arrow With Tip Rightwards / Up Arrow With Tip Right
  ^^^^21b2% ↲   \Ldsh   Downwards Arrow With Tip Leftwards / Down Arrow With Tip Left
  ^^^^21b3% ↳   \Rdsh   Downwards Arrow With Tip Rightwards / Down Arrow With Tip Right
  ^^^^21b4% ↴   \linefeed   Rightwards Arrow With Corner Downwards / Right Arrow With Corner Down
  ^^^^21b5% ↵   \carriagereturn Downwards Arrow With Corner Leftwards / Down Arrow With Corner Left
  ^^^^21b6% ↶   \curvearrowleft Anticlockwise Top Semicircle Arrow
  ^^^^21b7% ↷   \curvearrowright    Clockwise Top Semicircle Arrow
  ^^^^21b8% ↸   \barovernorthwestarrow  North West Arrow To Long Bar / Upper Left Arrow To Long Bar
  ^^^^21b9% ↹   \barleftarrowrightarrowbar  Leftwards Arrow To Bar Over Rightwards Arrow To Bar / Left Arrow To Bar Over Right Arrow To Bar
  ^^^^21ba% ↺   \circlearrowleft    Anticlockwise Open Circle Arrow
  ^^^^21bb% ↻   \circlearrowright   Clockwise Open Circle Arrow
  ^^^^21bc% ↼   \leftharpoonup  Leftwards Harpoon With Barb Upwards / Left Harpoon With Barb Up
  ^^^^21bd% ↽   \leftharpoondown    Leftwards Harpoon With Barb Downwards / Left Harpoon With Barb Down
  ^^^^21be% ↾   \upharpoonright Upwards Harpoon With Barb Rightwards / Up Harpoon With Barb Right
  ^^^^21bf% ↿   \upharpoonleft  Upwards Harpoon With Barb Leftwards / Up Harpoon With Barb Left
  ^^^^21c0% ⇀   \rightharpoonup Rightwards Harpoon With Barb Upwards / Right Harpoon With Barb Up
  ^^^^21c1% ⇁   \rightharpoondown   Rightwards Harpoon With Barb Downwards / Right Harpoon With Barb Down
  ^^^^21c2% ⇂   \downharpoonright   Downwards Harpoon With Barb Rightwards / Down Harpoon With Barb Right
  ^^^^21c3% ⇃   \downharpoonleft    Downwards Harpoon With Barb Leftwards / Down Harpoon With Barb Left
  ^^^^21c4% ⇄   \rightleftarrows    Rightwards Arrow Over Leftwards Arrow / Right Arrow Over Left Arrow
  ^^^^21c5% ⇅   \dblarrowupdown Upwards Arrow Leftwards Of Downwards Arrow / Up Arrow Left Of Down Arrow
  ^^^^21c6% ⇆   \leftrightarrows    Leftwards Arrow Over Rightwards Arrow / Left Arrow Over Right Arrow
  ^^^^21c7% ⇇   \leftleftarrows Leftwards Paired Arrows / Left Paired Arrows
  ^^^^21c8% ⇈   \upuparrows Upwards Paired Arrows / Up Paired Arrows
  ^^^^21c9% ⇉   \rightrightarrows   Rightwards Paired Arrows / Right Paired Arrows
  ^^^^21ca% ⇊   \downdownarrows Downwards Paired Arrows / Down Paired Arrows
  ^^^^21cb% ⇋   \leftrightharpoons  Leftwards Harpoon Over Rightwards Harpoon / Left Harpoon Over Right Harpoon
  ^^^^21cc% ⇌   \rightleftharpoons  Rightwards Harpoon Over Leftwards Harpoon / Right Harpoon Over Left Harpoon
  ^^^^21cd% ⇍   \nLeftarrow Leftwards Double Arrow With Stroke / Left Double Arrow With Stroke
  ^^^^21ce% ⇎   \nLeftrightarrow    Left Right Double Arrow With Stroke
  ^^^^21cf% ⇏   \nRightarrow    Rightwards Double Arrow With Stroke / Right Double Arrow With Stroke
  ^^^^21d0% ⇐   \Leftarrow  Leftwards Double Arrow / Left Double Arrow
  ^^^^21d1% ⇑   \Uparrow    Upwards Double Arrow / Up Double Arrow
  ^^^^21d2% ⇒   \Rightarrow Rightwards Double Arrow / Right Double Arrow
  ^^^^21d3% ⇓   \Downarrow  Downwards Double Arrow / Down Double Arrow
  ^^^^21d4% ⇔   \Leftrightarrow Left Right Double Arrow
  ^^^^21d5% ⇕   \Updownarrow    Up Down Double Arrow
  ^^^^21d6% ⇖   \Nwarrow    North West Double Arrow / Upper Left Double Arrow
  ^^^^21d7% ⇗   \Nearrow    North East Double Arrow / Upper Right Double Arrow
  ^^^^21d8% ⇘   \Searrow    South East Double Arrow / Lower Right Double Arrow
  ^^^^21d9% ⇙   \Swarrow    South West Double Arrow / Lower Left Double Arrow
  ^^^^21da% ⇚   \Lleftarrow Leftwards Triple Arrow / Left Triple Arrow
  ^^^^21db% ⇛   \Rrightarrow    Rightwards Triple Arrow / Right Triple Arrow
  ^^^^21dc% ⇜   \leftsquigarrow Leftwards Squiggle Arrow / Left Squiggle Arrow
  ^^^^21dd% ⇝   \rightsquigarrow    Rightwards Squiggle Arrow / Right Squiggle Arrow
  ^^^^21de% ⇞   \nHuparrow  Upwards Arrow With Double Stroke / Up Arrow With Double Stroke
  ^^^^21df% ⇟   \nHdownarrow    Downwards Arrow With Double Stroke / Down Arrow With Double Stroke
  ^^^^21e0% ⇠   \leftdasharrow  Leftwards Dashed Arrow / Left Dashed Arrow
  ^^^^21e1% ⇡   \updasharrow    Upwards Dashed Arrow / Up Dashed Arrow
  ^^^^21e2% ⇢   \rightdasharrow Rightwards Dashed Arrow / Right Dashed Arrow
  ^^^^21e3% ⇣   \downdasharrow  Downwards Dashed Arrow / Down Dashed Arrow
  ^^^^21e4% ⇤   \barleftarrow   Leftwards Arrow To Bar / Left Arrow To Bar
  ^^^^21e5% ⇥   \rightarrowbar  Rightwards Arrow To Bar / Right Arrow To Bar
  ^^^^21e6% ⇦   \leftwhitearrow Leftwards White Arrow / White Left Arrow
  ^^^^21e7% ⇧   \upwhitearrow   Upwards White Arrow / White Up Arrow
  ^^^^21e8% ⇨   \rightwhitearrow    Rightwards White Arrow / White Right Arrow
  ^^^^21e9% ⇩   \downwhitearrow Downwards White Arrow / White Down Arrow
  ^^^^21ea% ⇪   \whitearrowupfrombar    Upwards White Arrow From Bar / White Up Arrow From Bar
  ^^^^21f4% ⇴   \circleonrightarrow Right Arrow With Small Circle
  ^^^^21f5% ⇵   \DownArrowUpArrow   Downwards Arrow Leftwards Of Upwards Arrow
  ^^^^21f6% ⇶   \rightthreearrows   Three Rightwards Arrows
  ^^^^21f7% ⇷   \nvleftarrow    Leftwards Arrow With Vertical Stroke
  ^^^^21f8% ⇸   \nvrightarrow   Rightwards Arrow With Vertical Stroke
  ^^^^21f9% ⇹   \nvleftrightarrow   Left Right Arrow With Vertical Stroke
  ^^^^21fa% ⇺   \nVleftarrow    Leftwards Arrow With Double Vertical Stroke
  ^^^^21fb% ⇻   \nVrightarrow   Rightwards Arrow With Double Vertical Stroke
  ^^^^21fc% ⇼   \nVleftrightarrow   Left Right Arrow With Double Vertical Stroke
  ^^^^21fd% ⇽   \leftarrowtriangle  Leftwards Open-Headed Arrow
  ^^^^21fe% ⇾   \rightarrowtriangle Rightwards Open-Headed Arrow
  ^^^^21ff% ⇿   \leftrightarrowtriangle Left Right Open-Headed Arrow
  ^^^^2200% ∀   \forall For All
  ^^^^2201% ∁   \complement Complement
  ^^^^2202% ∂   \partial    Partial Differential
  ^^^^2203% ∃   \exists There Exists
  ^^^^2204% ∄   \nexists    There Does Not Exist
  ^^^^2205% ∅   \varnothing, \emptyset  Empty Set
  ^^^^2206% ∆   \increment  Increment
  ^^^^2207% ∇   \del, \nabla    Nabla
  ^^^^2208% ∈   \in Element Of
  ^^^^2209% ∉   \notin  Not An Element Of
  ^^^^220a% ∊   \smallin    Small Element Of
  ^^^^220b% ∋   \ni Contains As Member
  ^^^^220c% ∌   \nni    Does Not Contain As Member
  ^^^^220d% ∍   \smallni    Small Contains As Member
  ^^^^220e% ∎   \QED    End Of Proof
  ^^^^220f% ∏   \prod   N-Ary Product
  ^^^^2210% ∐   \coprod N-Ary Coproduct
  ^^^^2211% ∑   \sum    N-Ary Summation
  ^^^^2212% −   \minus  Minus Sign
  ^^^^2213% ∓   \mp Minus-Or-Plus Sign
  ^^^^2214% ∔   \dotplus    Dot Plus
  ^^^^2216% ∖   \setminus   Set Minus
  ^^^^2217% ∗   \ast    Asterisk Operator
  ^^^^2218% ∘   \circ   Ring Operator
  ^^^^2219% ∙   \vysmblkcircle  Bullet Operator
  ^^^^221a% √   \surd, \sqrt    Square Root
  ^^^^221b% ∛   \cbrt   Cube Root
  ^^^^221c% ∜   \fourthroot Fourth Root
  ^^^^221d% ∝   \propto Proportional To
  ^^^^221e% ∞   \infty  Infinity
  ^^^^221f% ∟   \rightangle Right Angle
  ^^^^2220% ∠   \angle  Angle
  ^^^^2221% ∡   \measuredangle  Measured Angle
  ^^^^2222% ∢   \sphericalangle Spherical Angle
  ^^^^2223% ∣   \mid    Divides
  ^^^^2224% ∤   \nmid   Does Not Divide
  ^^^^2225% ∥   \parallel   Parallel To
  ^^^^2226% ∦   \nparallel  Not Parallel To
  ^^^^2227% ∧   \wedge  Logical And
  ^^^^2228% ∨   \vee    Logical Or
  ^^^^2229% ∩   \cap    Intersection
  ^^^^222a% ∪   \cup    Union
  ^^^^222b% ∫   \int    Integral
  ^^^^222c% ∬   \iint   Double Integral
  ^^^^222d% ∭   \iiint  Triple Integral
  ^^^^222e% ∮   \oint   Contour Integral
  ^^^^222f% ∯   \oiint  Surface Integral
  ^^^^2230% ∰   \oiiint Volume Integral
  ^^^^2231% ∱   \clwintegral    Clockwise Integral
  ^^^^2232% ∲   \varointclockwise   Clockwise Contour Integral
  ^^^^2233% ∳   \ointctrclockwise   Anticlockwise Contour Integral
  ^^^^2234% ∴   \therefore  Therefore
  ^^^^2235% ∵   \because    Because
  ^^^^2237% ∷   \Colon  Proportion
  ^^^^2238% ∸   \dotminus   Dot Minus
  ^^^^223a% ∺   \dotsminusdots  Geometric Proportion
  ^^^^223b% ∻   \kernelcontraction  Homothetic
  ^^^^223c% ∼   \sim    Tilde Operator
  ^^^^223d% ∽   \backsim    Reversed Tilde
  ^^^^223e% ∾   \lazysinv   Inverted Lazy S
  ^^^^223f% ∿   \sinewave   Sine Wave
  ^^^^2240% ≀   \wr Wreath Product
  ^^^^2241% ≁   \nsim   Not Tilde
  ^^^^2242% ≂   \eqsim  Minus Tilde
  ^^^^2242% + ^^^^0338%   ≂̸  \neqsim Minus Tilde + Combining Long Solidus Overlay / Non-Spacing Long Slash Overlay
  ^^^^2243% ≃   \simeq  Asymptotically Equal To
  ^^^^2244% ≄   \nsime  Not Asymptotically Equal To
  ^^^^2245% ≅   \cong   Approximately Equal To
  ^^^^2246% ≆   \approxnotequal Approximately But Not Actually Equal To
  ^^^^2247% ≇   \ncong  Neither Approximately Nor Actually Equal To
  ^^^^2248% ≈   \approx Almost Equal To
  ^^^^2249% ≉   \napprox    Not Almost Equal To
  ^^^^224a% ≊   \approxeq   Almost Equal Or Equal To
  ^^^^224b% ≋   \tildetrpl  Triple Tilde
  ^^^^224c% ≌   \allequal   All Equal To
  ^^^^224d% ≍   \asymp  Equivalent To
  ^^^^224e% ≎   \Bumpeq Geometrically Equivalent To
  ^^^^224e% + ^^^^0338%   ≎̸  \nBumpeq    Geometrically Equivalent To + Combining Long Solidus Overlay / Non-Spacing Long Slash Overlay
  ^^^^224f% ≏   \bumpeq Difference Between
  ^^^^224f% + ^^^^0338%   ≏̸  \nbumpeq    Difference Between + Combining Long Solidus Overlay / Non-Spacing Long Slash Overlay
  ^^^^2250% ≐   \doteq  Approaches The Limit
  ^^^^2251% ≑   \Doteq  Geometrically Equal To
  ^^^^2252% ≒   \fallingdotseq  Approximately Equal To Or The Image Of
  ^^^^2253% ≓   \risingdotseq   Image Of Or Approximately Equal To
  ^^^^2254% ≔   \coloneq    Colon Equals / Colon Equal
  ^^^^2255% ≕   \eqcolon    Equals Colon / Equal Colon
  ^^^^2256% ≖   \eqcirc Ring In Equal To
  ^^^^2257% ≗   \circeq Ring Equal To
  ^^^^2258% ≘   \arceq  Corresponds To
  ^^^^2259% ≙   \wedgeq Estimates
  ^^^^225a% ≚   \veeeq  Equiangular To
  ^^^^225b% ≛   \starequal  Star Equals
  ^^^^225c% ≜   \triangleq  Delta Equal To
  ^^^^225d% ≝   \eqdef  Equal To By Definition
  ^^^^225e% ≞   \measeq Measured By
  ^^^^225f% ≟   \questeq    Questioned Equal To
  ^^^^2260% ≠   \ne Not Equal To
  ^^^^2261% ≡   \equiv  Identical To
  ^^^^2262% ≢   \nequiv Not Identical To
  ^^^^2263% ≣   \Equiv  Strictly Equivalent To
  ^^^^2264% ≤   \le, \leq   Less-Than Or Equal To / Less Than Or Equal To
  ^^^^2265% ≥   \ge, \geq   Greater-Than Or Equal To / Greater Than Or Equal To
  ^^^^2266% ≦   \leqq   Less-Than Over Equal To / Less Than Over Equal To
  ^^^^2267% ≧   \geqq   Greater-Than Over Equal To / Greater Than Over Equal To
  ^^^^2268% ≨   \lneqq  Less-Than But Not Equal To / Less Than But Not Equal To
  ^^^^2268% + ^^^^fe00%   ≨︀  \lvertneqq  Less-Than But Not Equal To / Less Than But Not Equal To + Variation Selector-1
  ^^^^2269% ≩   \gneqq  Greater-Than But Not Equal To / Greater Than But Not Equal To
  ^^^^2269% + ^^^^fe00%   ≩︀  \gvertneqq  Greater-Than But Not Equal To / Greater Than But Not Equal To + Variation Selector-1
  ^^^^226a% ≪   \ll Much Less-Than / Much Less Than
  ^^^^226a% + ^^^^0338%   ≪̸  \NotLessLess    Much Less-Than / Much Less Than + Combining Long Solidus Overlay / Non-Spacing Long Slash Overlay
  ^^^^226b% ≫   \gg Much Greater-Than / Much Greater Than
  ^^^^226b% + ^^^^0338%   ≫̸  \NotGreaterGreater  Much Greater-Than / Much Greater Than + Combining Long Solidus Overlay / Non-Spacing Long Slash Overlay
  ^^^^226c% ≬   \between    Between
  ^^^^226d% ≭   \nasymp Not Equivalent To
  ^^^^226e% ≮   \nless  Not Less-Than / Not Less Than
  ^^^^226f% ≯   \ngtr   Not Greater-Than / Not Greater Than
  ^^^^2270% ≰   \nleq   Neither Less-Than Nor Equal To / Neither Less Than Nor Equal To
  ^^^^2271% ≱   \ngeq   Neither Greater-Than Nor Equal To / Neither Greater Than Nor Equal To
  ^^^^2272% ≲   \lesssim    Less-Than Or Equivalent To / Less Than Or Equivalent To
  ^^^^2273% ≳   \gtrsim Greater-Than Or Equivalent To / Greater Than Or Equivalent To
  ^^^^2274% ≴   \nlesssim   Neither Less-Than Nor Equivalent To / Neither Less Than Nor Equivalent To
  ^^^^2275% ≵   \ngtrsim    Neither Greater-Than Nor Equivalent To / Neither Greater Than Nor Equivalent To
  ^^^^2276% ≶   \lessgtr    Less-Than Or Greater-Than / Less Than Or Greater Than
  ^^^^2277% ≷   \gtrless    Greater-Than Or Less-Than / Greater Than Or Less Than
  ^^^^2278% ≸   \notlessgreater Neither Less-Than Nor Greater-Than / Neither Less Than Nor Greater Than
  ^^^^2279% ≹   \notgreaterless Neither Greater-Than Nor Less-Than / Neither Greater Than Nor Less Than
  ^^^^227a% ≺   \prec   Precedes
  ^^^^227b% ≻   \succ   Succeeds
  ^^^^227c% ≼   \preccurlyeq    Precedes Or Equal To
  ^^^^227d% ≽   \succcurlyeq    Succeeds Or Equal To
  ^^^^227e% ≾   \precsim    Precedes Or Equivalent To
  ^^^^227e% + ^^^^0338%   ≾̸  \nprecsim   Precedes Or Equivalent To + Combining Long Solidus Overlay / Non-Spacing Long Slash Overlay
  ^^^^227f% ≿   \succsim    Succeeds Or Equivalent To
  ^^^^227f% + ^^^^0338%   ≿̸  \nsuccsim   Succeeds Or Equivalent To + Combining Long Solidus Overlay / Non-Spacing Long Slash Overlay
  ^^^^2280% ⊀   \nprec  Does Not Precede
  ^^^^2281% ⊁   \nsucc  Does Not Succeed
  ^^^^2282% ⊂   \subset Subset Of
  ^^^^2283% ⊃   \supset Superset Of
  ^^^^2284% ⊄   \nsubset    Not A Subset Of
  ^^^^2285% ⊅   \nsupset    Not A Superset Of
  ^^^^2286% ⊆   \subseteq   Subset Of Or Equal To
  ^^^^2287% ⊇   \supseteq   Superset Of Or Equal To
  ^^^^2288% ⊈   \nsubseteq  Neither A Subset Of Nor Equal To
  ^^^^2289% ⊉   \nsupseteq  Neither A Superset Of Nor Equal To
  ^^^^228a% ⊊   \subsetneq  Subset Of With Not Equal To / Subset Of Or Not Equal To
  ^^^^228a% + ^^^^fe00%   ⊊︀  \varsubsetneqq  Subset Of With Not Equal To / Subset Of Or Not Equal To + Variation Selector-1
  ^^^^228b% ⊋   \supsetneq  Superset Of With Not Equal To / Superset Of Or Not Equal To
  ^^^^228b% + ^^^^fe00%   ⊋︀  \varsupsetneq   Superset Of With Not Equal To / Superset Of Or Not Equal To + Variation Selector-1
  ^^^^228d% ⊍   \cupdot Multiset Multiplication
  ^^^^228e% ⊎   \uplus  Multiset Union
  ^^^^228f% ⊏   \sqsubset   Square Image Of
  ^^^^228f% + ^^^^0338%   ⊏̸  \NotSquareSubset    Square Image Of + Combining Long Solidus Overlay / Non-Spacing Long Slash Overlay
  ^^^^2290% ⊐   \sqsupset   Square Original Of
  ^^^^2290% + ^^^^0338%   ⊐̸  \NotSquareSuperset  Square Original Of + Combining Long Solidus Overlay / Non-Spacing Long Slash Overlay
  ^^^^2291% ⊑   \sqsubseteq Square Image Of Or Equal To
  ^^^^2292% ⊒   \sqsupseteq Square Original Of Or Equal To
  ^^^^2293% ⊓   \sqcap  Square Cap
  ^^^^2294% ⊔   \sqcup  Square Cup
  ^^^^2295% ⊕   \oplus  Circled Plus
  ^^^^2296% ⊖   \ominus Circled Minus
  ^^^^2297% ⊗   \otimes Circled Times
  ^^^^2298% ⊘   \oslash Circled Division Slash
  ^^^^2299% ⊙   \odot   Circled Dot Operator
  ^^^^229a% ⊚   \circledcirc    Circled Ring Operator
  ^^^^229b% ⊛   \circledast Circled Asterisk Operator
  ^^^^229c% ⊜   \circledequal   Circled Equals
  ^^^^229d% ⊝   \circleddash    Circled Dash
  ^^^^229e% ⊞   \boxplus    Squared Plus
  ^^^^229f% ⊟   \boxminus   Squared Minus
  ^^^^22a0% ⊠   \boxtimes   Squared Times
  ^^^^22a1% ⊡   \boxdot Squared Dot Operator
  ^^^^22a2% ⊢   \vdash  Right Tack
  ^^^^22a3% ⊣   \dashv  Left Tack
  ^^^^22a4% ⊤   \top    Down Tack
  ^^^^22a5% ⊥   \bot    Up Tack
  ^^^^22a7% ⊧   \models Models
  ^^^^22a8% ⊨   \vDash  True
  ^^^^22a9% ⊩   \Vdash  Forces
  ^^^^22aa% ⊪   \Vvdash Triple Vertical Bar Right Turnstile
  ^^^^22ab% ⊫   \VDash  Double Vertical Bar Double Right Turnstile
  ^^^^22ac% ⊬   \nvdash Does Not Prove
  ^^^^22ad% ⊭   \nvDash Not True
  ^^^^22ae% ⊮   \nVdash Does Not Force
  ^^^^22af% ⊯   \nVDash Negated Double Vertical Bar Double Right Turnstile
  ^^^^22b0% ⊰   \prurel Precedes Under Relation
  ^^^^22b1% ⊱   \scurel Succeeds Under Relation
  ^^^^22b2% ⊲   \vartriangleleft    Normal Subgroup Of
  ^^^^22b3% ⊳   \vartriangleright   Contains As Normal Subgroup
  ^^^^22b4% ⊴   \trianglelefteq Normal Subgroup Of Or Equal To
  ^^^^22b5% ⊵   \trianglerighteq    Contains As Normal Subgroup Or Equal To
  ^^^^22b6% ⊶   \original   Original Of
  ^^^^22b7% ⊷   \image  Image Of
  ^^^^22b8% ⊸   \multimap   Multimap
  ^^^^22b9% ⊹   \hermitconjmatrix   Hermitian Conjugate Matrix
  ^^^^22ba% ⊺   \intercal   Intercalate
  ^^^^22bb% ⊻   \veebar, \xor   Xor
  ^^^^22bc% ⊼   \barwedge   Nand
  ^^^^22bd% ⊽   \barvee Nor
  ^^^^22be% ⊾   \rightanglearc  Right Angle With Arc
  ^^^^22bf% ⊿   \varlrtriangle  Right Triangle
  ^^^^22c0% ⋀   \bigwedge   N-Ary Logical And
  ^^^^22c1% ⋁   \bigvee N-Ary Logical Or
  ^^^^22c2% ⋂   \bigcap N-Ary Intersection
  ^^^^22c3% ⋃   \bigcup N-Ary Union
  ^^^^22c4% ⋄   \diamond    Diamond Operator
  ^^^^22c5% ⋅   \cdot   Dot Operator
  ^^^^22c6% ⋆   \star   Star Operator
  ^^^^22c7% ⋇   \divideontimes  Division Times
  ^^^^22c8% ⋈   \bowtie Bowtie
  ^^^^22c9% ⋉   \ltimes Left Normal Factor Semidirect Product
  ^^^^22ca% ⋊   \rtimes Right Normal Factor Semidirect Product
  ^^^^22cb% ⋋   \leftthreetimes Left Semidirect Product
  ^^^^22cc% ⋌   \rightthreetimes    Right Semidirect Product
  ^^^^22cd% ⋍   \backsimeq  Reversed Tilde Equals
  ^^^^22ce% ⋎   \curlyvee   Curly Logical Or
  ^^^^22cf% ⋏   \curlywedge Curly Logical And
  ^^^^22d0% ⋐   \Subset Double Subset
  ^^^^22d1% ⋑   \Supset Double Superset
  ^^^^22d2% ⋒   \Cap    Double Intersection
  ^^^^22d3% ⋓   \Cup    Double Union
  ^^^^22d4% ⋔   \pitchfork  Pitchfork
  ^^^^22d5% ⋕   \equalparallel  Equal And Parallel To
  ^^^^22d6% ⋖   \lessdot    Less-Than With Dot / Less Than With Dot
  ^^^^22d7% ⋗   \gtrdot Greater-Than With Dot / Greater Than With Dot
  ^^^^22d8% ⋘   \verymuchless   Very Much Less-Than / Very Much Less Than
  ^^^^22d9% ⋙   \ggg    Very Much Greater-Than / Very Much Greater Than
  ^^^^22da% ⋚   \lesseqgtr  Less-Than Equal To Or Greater-Than / Less Than Equal To Or Greater Than
  ^^^^22db% ⋛   \gtreqless  Greater-Than Equal To Or Less-Than / Greater Than Equal To Or Less Than
  ^^^^22dc% ⋜   \eqless Equal To Or Less-Than / Equal To Or Less Than
  ^^^^22dd% ⋝   \eqgtr  Equal To Or Greater-Than / Equal To Or Greater Than
  ^^^^22de% ⋞   \curlyeqprec    Equal To Or Precedes
  ^^^^22df% ⋟   \curlyeqsucc    Equal To Or Succeeds
  ^^^^22e0% ⋠   \npreccurlyeq   Does Not Precede Or Equal
  ^^^^22e1% ⋡   \nsucccurlyeq   Does Not Succeed Or Equal
  ^^^^22e2% ⋢   \nsqsubseteq    Not Square Image Of Or Equal To
  ^^^^22e3% ⋣   \nsqsupseteq    Not Square Original Of Or Equal To
  ^^^^22e4% ⋤   \sqsubsetneq    Square Image Of Or Not Equal To
  ^^^^22e5% ⋥   \sqspne Square Original Of Or Not Equal To
  ^^^^22e6% ⋦   \lnsim  Less-Than But Not Equivalent To / Less Than But Not Equivalent To
  ^^^^22e7% ⋧   \gnsim  Greater-Than But Not Equivalent To / Greater Than But Not Equivalent To
  ^^^^22e8% ⋨   \precnsim   Precedes But Not Equivalent To
  ^^^^22e9% ⋩   \succnsim   Succeeds But Not Equivalent To
  ^^^^22ea% ⋪   \ntriangleleft  Not Normal Subgroup Of
  ^^^^22eb% ⋫   \ntriangleright Does Not Contain As Normal Subgroup
  ^^^^22ec% ⋬   \ntrianglelefteq    Not Normal Subgroup Of Or Equal To
  ^^^^22ed% ⋭   \ntrianglerighteq   Does Not Contain As Normal Subgroup Or Equal
  ^^^^22ee% ⋮   \vdots  Vertical Ellipsis
  ^^^^22ef% ⋯   \cdots  Midline Horizontal Ellipsis
  ^^^^22f0% ⋰   \adots  Up Right Diagonal Ellipsis
  ^^^^22f1% ⋱   \ddots  Down Right Diagonal Ellipsis
  ^^^^22f2% ⋲   \disin  Element Of With Long Horizontal Stroke
  ^^^^22f3% ⋳   \varisins   Element Of With Vertical Bar At End Of Horizontal Stroke
  ^^^^22f4% ⋴   \isins  Small Element Of With Vertical Bar At End Of Horizontal Stroke
  ^^^^22f5% ⋵   \isindot    Element Of With Dot Above
  ^^^^22f6% ⋶   \varisinobar    Element Of With Overbar
  ^^^^22f7% ⋷   \isinobar   Small Element Of With Overbar
  ^^^^22f8% ⋸   \isinvb Element Of With Underbar
  ^^^^22f9% ⋹   \isinE  Element Of With Two Horizontal Strokes
  ^^^^22fa% ⋺   \nisd   Contains With Long Horizontal Stroke
  ^^^^22fb% ⋻   \varnis Contains With Vertical Bar At End Of Horizontal Stroke
  ^^^^22fc% ⋼   \nis    Small Contains With Vertical Bar At End Of Horizontal Stroke
  ^^^^22fd% ⋽   \varniobar  Contains With Overbar
  ^^^^22fe% ⋾   \niobar Small Contains With Overbar
  ^^^^22ff% ⋿   \bagmember  Z Notation Bag Membership
  ^^^^2300% ⌀   \diameter   Diameter Sign
  ^^^^2302% ⌂   \house  House
  ^^^^2305% ⌅   \varbarwedge    Projective
  ^^^^2306% ⌆   \vardoublebarwedge  Perspective
  ^^^^2308% ⌈   \lceil  Left Ceiling
  ^^^^2309% ⌉   \rceil  Right Ceiling
  ^^^^230a% ⌊   \lfloor Left Floor
  ^^^^230b% ⌋   \rfloor Right Floor
  ^^^^2310% ⌐   \invnot Reversed Not Sign
  ^^^^2311% ⌑   \sqlozenge  Square Lozenge
  ^^^^2312% ⌒   \profline   Arc
  ^^^^2313% ⌓   \profsurf   Segment
  ^^^^2315% ⌕   \recorder   Telephone Recorder
  ^^^^2317% ⌗   \viewdata   Viewdata Square
  ^^^^2319% ⌙   \turnednot  Turned Not Sign
  ^^^^231a% ⌚   \:watch:    Watch
  ^^^^231b% ⌛   \:hourglass:    Hourglass
  ^^^^231c% ⌜   \ulcorner   Top Left Corner
  ^^^^231d% ⌝   \urcorner   Top Right Corner
  ^^^^231e% ⌞   \llcorner   Bottom Left Corner
  ^^^^231f% ⌟   \lrcorner   Bottom Right Corner
  ^^^^2322% ⌢   \frown  Frown
  ^^^^2323% ⌣   \smile  Smile
  ^^^^232c% ⌬   \varhexagonlrbonds  Benzene Ring
  ^^^^2332% ⌲   \conictaper Conical Taper
  ^^^^2336% ⌶   \topbot Apl Functional Symbol I-Beam
  ^^^^233d% ⌽   \obar   Apl Functional Symbol Circle Stile
  ^^^^233f% ⌿   \notslash   Apl Functional Symbol Slash Bar
  ^^^^2340% ⍀   \notbackslash   Apl Functional Symbol Backslash Bar
  ^^^^2353% ⍓   \boxupcaret Apl Functional Symbol Quad Up Caret
  ^^^^2370% ⍰   \boxquestion    Apl Functional Symbol Quad Question
  ^^^^2394% ⎔   \hexagon    Software-Function Symbol
  ^^^^23a3% ⎣   \dlcorn Left Square Bracket Lower Corner
  ^^^^23b0% ⎰   \lmoustache Upper Left Or Lower Right Curly Bracket Section
  ^^^^23b1% ⎱   \rmoustache Upper Right Or Lower Left Curly Bracket Section
  ^^^^23b4% ⎴   \overbracket    Top Square Bracket
  ^^^^23b5% ⎵   \underbracket   Bottom Square Bracket
  ^^^^23b6% ⎶   \bbrktbrk   Bottom Square Bracket Over Top Square Bracket
  ^^^^23b7% ⎷   \sqrtbottom Radical Symbol Bottom
  ^^^^23b8% ⎸   \lvboxline  Left Vertical Box Line
  ^^^^23b9% ⎹   \rvboxline  Right Vertical Box Line
  ^^^^23ce% ⏎   \varcarriagereturn  Return Symbol
  ^^^^23de% ⏞   \overbrace  Top Curly Bracket
  ^^^^23df% ⏟   \underbrace Bottom Curly Bracket
  ^^^^23e2% ⏢   \trapezium  White Trapezium
  ^^^^23e3% ⏣   \benzenr    Benzene Ring With Circle
  ^^^^23e4% ⏤   \strns  Straightness
  ^^^^23e5% ⏥   \fltns  Flatness
  ^^^^23e6% ⏦   \accurrent  Ac Current
  ^^^^23e7% ⏧   \elinters   Electrical Intersection
  ^^^^23e9% ⏩   \:fast_forward: Black Right-Pointing Double Triangle
  ^^^^23ea% ⏪   \:rewind:   Black Left-Pointing Double Triangle
  ^^^^23eb% ⏫   \:arrow_double_up:  Black Up-Pointing Double Triangle
  ^^^^23ec% ⏬   \:arrow_double_down:    Black Down-Pointing Double Triangle
  ^^^^23f0% ⏰   \:alarm_clock:  Alarm Clock
  ^^^^23f3% ⏳   \:hourglass_flowing_sand:   Hourglass With Flowing Sand
  ^^^^2422% ␢   \blanksymbol    Blank Symbol / Blank
  ^^^^2423% ␣   \visiblespace   Open Box
  ^^^^24c2% Ⓜ   \:m:    Circled Latin Capital Letter M
  ^^^^24c8% Ⓢ   \circledS   Circled Latin Capital Letter S
  ^^^^2500% ─       Box Drawings Light Horizontal
  ^^^^2502% │       Box Drawings Light Vertical
  ^^^^253c% ┼       Box Drawings Light Vertical and Horizontal
  ^^^^2506% ┆   \dshfnc Box Drawings Light Triple Dash Vertical / Forms Light Triple Dash Vertical
  ^^^^2519% ┙   \sqfnw  Box Drawings Up Light And Left Heavy / Forms Up Light And Left Heavy
  ^^^^2571% ╱   \diagup Box Drawings Light Diagonal Upper Right To Lower Left / Forms Light Diagonal Upper Right To Lower Left
  ^^^^2572% ╲   \diagdown   Box Drawings Light Diagonal Upper Left To Lower Right / Forms Light Diagonal Upper Left To Lower Right
  ^^^^2580% ▀   \blockuphalf    Upper Half Block
  ^^^^2584% ▄   \blocklowhalf   Lower Half Block
  ^^^^2588% █   \blockfull  Full Block
  ^^^^258c% ▌   \blocklefthalf  Left Half Block
  ^^^^2590% ▐   \blockrighthalf Right Half Block
  ^^^^2591% ░   \blockqtrshaded Light Shade
  ^^^^2592% ▒   \blockhalfshaded    Medium Shade
  ^^^^2593% ▓   \blockthreeqtrshaded    Dark Shade
  ^^^^25a0% ■   \blacksquare    Black Square
  ^^^^25a1% □   \square White Square
  ^^^^25a2% ▢   \squoval    White Square With Rounded Corners
  ^^^^25a3% ▣   \blackinwhitesquare White Square Containing Black Small Square
  ^^^^25a4% ▤   \squarehfill    Square With Horizontal Fill
  ^^^^25a5% ▥   \squarevfill    Square With Vertical Fill
  ^^^^25a6% ▦   \squarehvfill   Square With Orthogonal Crosshatch Fill
  ^^^^25a7% ▧   \squarenwsefill Square With Upper Left To Lower Right Fill
  ^^^^25a8% ▨   \squareneswfill Square With Upper Right To Lower Left Fill
  ^^^^25a9% ▩   \squarecrossfill    Square With Diagonal Crosshatch Fill
  ^^^^25aa% ▪   \smblksquare, \:black_small_square: Black Small Square
  ^^^^25ab% ▫   \smwhtsquare, \:white_small_square: White Small Square
  ^^^^25ac% ▬   \hrectangleblack    Black Rectangle
  ^^^^25ad% ▭   \hrectangle White Rectangle
  ^^^^25ae% ▮   \vrectangleblack    Black Vertical Rectangle
  ^^^^25af% ▯   \vrecto White Vertical Rectangle
  ^^^^25b0% ▰   \parallelogramblack Black Parallelogram
  ^^^^25b1% ▱   \parallelogram  White Parallelogram
  ^^^^25b2% ▲   \bigblacktriangleup Black Up-Pointing Triangle / Black Up Pointing Triangle
  ^^^^25b3% △   \bigtriangleup  White Up-Pointing Triangle / White Up Pointing Triangle
  ^^^^25b4% ▴   \blacktriangle  Black Up-Pointing Small Triangle / Black Up Pointing Small Triangle
  ^^^^25b5% ▵   \vartriangle    White Up-Pointing Small Triangle / White Up Pointing Small Triangle
  ^^^^25b6% ▶   \blacktriangleright, \:arrow_forward:   Black Right-Pointing Triangle / Black Right Pointing Triangle
  ^^^^25b7% ▷   \triangleright  White Right-Pointing Triangle / White Right Pointing Triangle
  ^^^^25b8% ▸   \smallblacktriangleright    Black Right-Pointing Small Triangle / Black Right Pointing Small Triangle
  ^^^^25b9% ▹   \smalltriangleright White Right-Pointing Small Triangle / White Right Pointing Small Triangle
  ^^^^25ba% ►   \blackpointerright  Black Right-Pointing Pointer / Black Right Pointing Pointer
  ^^^^25bb% ▻   \whitepointerright  White Right-Pointing Pointer / White Right Pointing Pointer
  ^^^^25bc% ▼   \bigblacktriangledown   Black Down-Pointing Triangle / Black Down Pointing Triangle
  ^^^^25bd% ▽   \bigtriangledown    White Down-Pointing Triangle / White Down Pointing Triangle
  ^^^^25be% ▾   \blacktriangledown  Black Down-Pointing Small Triangle / Black Down Pointing Small Triangle
  ^^^^25bf% ▿   \triangledown   White Down-Pointing Small Triangle / White Down Pointing Small Triangle
  ^^^^25c0% ◀   \blacktriangleleft, \:arrow_backward:   Black Left-Pointing Triangle / Black Left Pointing Triangle
  ^^^^25c1% ◁   \triangleleft   White Left-Pointing Triangle / White Left Pointing Triangle
  ^^^^25c2% ◂   \smallblacktriangleleft Black Left-Pointing Small Triangle / Black Left Pointing Small Triangle
  ^^^^25c3% ◃   \smalltriangleleft  White Left-Pointing Small Triangle / White Left Pointing Small Triangle
  ^^^^25c4% ◄   \blackpointerleft   Black Left-Pointing Pointer / Black Left Pointing Pointer
  ^^^^25c5% ◅   \whitepointerleft   White Left-Pointing Pointer / White Left Pointing Pointer
  ^^^^25c6% ◆   \mdlgblkdiamond Black Diamond
  ^^^^25c7% ◇   \mdlgwhtdiamond White Diamond
  ^^^^25c8% ◈   \blackinwhitediamond    White Diamond Containing Black Small Diamond
  ^^^^25c9% ◉   \fisheye    Fisheye
  ^^^^25ca% ◊   \lozenge    Lozenge
  ^^^^25cb% ○   \bigcirc    White Circle
  ^^^^25cc% ◌   \dottedcircle   Dotted Circle
  ^^^^25cd% ◍   \circlevertfill Circle With Vertical Fill
  ^^^^25ce% ◎   \bullseye   Bullseye
  ^^^^25cf% ●   \mdlgblkcircle  Black Circle
  ^^^^25d0% ◐   \cirfl  Circle With Left Half Black
  ^^^^25d1% ◑   \cirfr  Circle With Right Half Black
  ^^^^25d2% ◒   \cirfb  Circle With Lower Half Black
  ^^^^25d3% ◓   \circletophalfblack Circle With Upper Half Black
  ^^^^25d4% ◔   \circleurquadblack  Circle With Upper Right Quadrant Black
  ^^^^25d5% ◕   \blackcircleulquadwhite Circle With All But Upper Left Quadrant Black
  ^^^^25d6% ◖   \blacklefthalfcircle    Left Half Black Circle
  ^^^^25d7% ◗   \blackrighthalfcircle   Right Half Black Circle
  ^^^^25d8% ◘   \rvbull Inverse Bullet
  ^^^^25d9% ◙   \inversewhitecircle Inverse White Circle
  ^^^^25da% ◚   \invwhiteupperhalfcircle    Upper Half Inverse White Circle
  ^^^^25db% ◛   \invwhitelowerhalfcircle    Lower Half Inverse White Circle
  ^^^^25dc% ◜   \ularc  Upper Left Quadrant Circular Arc
  ^^^^25dd% ◝   \urarc  Upper Right Quadrant Circular Arc
  ^^^^25de% ◞   \lrarc  Lower Right Quadrant Circular Arc
  ^^^^25df% ◟   \llarc  Lower Left Quadrant Circular Arc
  ^^^^25e0% ◠   \topsemicircle  Upper Half Circle
  ^^^^25e1% ◡   \botsemicircle  Lower Half Circle
  ^^^^25e2% ◢   \lrblacktriangle    Black Lower Right Triangle
  ^^^^25e3% ◣   \llblacktriangle    Black Lower Left Triangle
  ^^^^25e4% ◤   \ulblacktriangle    Black Upper Left Triangle
  ^^^^25e5% ◥   \urblacktriangle    Black Upper Right Triangle
  ^^^^25e6% ◦   \smwhtcircle    White Bullet
  ^^^^25e7% ◧   \sqfl   Square With Left Half Black
  ^^^^25e8% ◨   \sqfr   Square With Right Half Black
  ^^^^25e9% ◩   \squareulblack  Square With Upper Left Diagonal Half Black
  ^^^^25ea% ◪   \sqfse  Square With Lower Right Diagonal Half Black
  ^^^^25eb% ◫   \boxbar White Square With Vertical Bisecting Line
  ^^^^25ec% ◬   \trianglecdot   White Up-Pointing Triangle With Dot / White Up Pointing Triangle With Dot
  ^^^^25ed% ◭   \triangleleftblack  Up-Pointing Triangle With Left Half Black / Up Pointing Triangle With Left Half Black
  ^^^^25ee% ◮   \trianglerightblack Up-Pointing Triangle With Right Half Black / Up Pointing Triangle With Right Half Black
  ^^^^25ef% ◯   \lgwhtcircle    Large Circle
  ^^^^25f0% ◰   \squareulquad   White Square With Upper Left Quadrant
  ^^^^25f1% ◱   \squarellquad   White Square With Lower Left Quadrant
  ^^^^25f2% ◲   \squarelrquad   White Square With Lower Right Quadrant
  ^^^^25f3% ◳   \squareurquad   White Square With Upper Right Quadrant
  ^^^^25f4% ◴   \circleulquad   White Circle With Upper Left Quadrant
  ^^^^25f5% ◵   \circlellquad   White Circle With Lower Left Quadrant
  ^^^^25f6% ◶   \circlelrquad   White Circle With Lower Right Quadrant
  ^^^^25f7% ◷   \circleurquad   White Circle With Upper Right Quadrant
  ^^^^25f8% ◸   \ultriangle Upper Left Triangle
  ^^^^25f9% ◹   \urtriangle Upper Right Triangle
  ^^^^25fa% ◺   \lltriangle Lower Left Triangle
  ^^^^25fb% ◻   \mdwhtsquare, \:white_medium_square:    White Medium Square
  ^^^^25fc% ◼   \mdblksquare, \:black_medium_square:    Black Medium Square
  ^^^^25fd% ◽   \mdsmwhtsquare, \:white_medium_small_square:    White Medium Small Square
  ^^^^25fe% ◾   \mdsmblksquare, \:black_medium_small_square:    Black Medium Small Square
  ^^^^25ff% ◿   \lrtriangle Lower Right Triangle
  ^^^^2600% ☀   \:sunny:    Black Sun With Rays
  ^^^^2601% ☁   \:cloud:    Cloud
  ^^^^2605% ★   \bigstar    Black Star
  ^^^^2606% ☆   \bigwhitestar   White Star
  ^^^^2609% ☉   \astrosun   Sun
  ^^^^260e% ☎   \:phone:    Black Telephone
  ^^^^2611% ☑   \:ballot_box_with_check:    Ballot Box With Check
  ^^^^2614% ☔   \:umbrella: Umbrella With Rain Drops
  ^^^^2615% ☕   \:coffee:   Hot Beverage
  ^^^^261d% ☝   \:point_up: White Up Pointing Index
  ^^^^2621% ☡   \danger Caution Sign
  ^^^^263a% ☺   \:relaxed:  White Smiling Face
  ^^^^263b% ☻   \blacksmiley    Black Smiling Face
  ^^^^263c% ☼   \sun    White Sun With Rays
  ^^^^263d% ☽   \rightmoon  First Quarter Moon
  ^^^^263e% ☾   \leftmoon   Last Quarter Moon
  ^^^^263f% ☿   \mercury    Mercury
  ^^^^2640% ♀   \venus, \female Female Sign
  ^^^^2642% ♂   \male, \mars    Male Sign
  ^^^^2643% ♃   \jupiter    Jupiter
  ^^^^2644% ♄   \saturn Saturn
  ^^^^2645% ♅   \uranus Uranus
  ^^^^2646% ♆   \neptune    Neptune
  ^^^^2647% ♇   \pluto  Pluto
  ^^^^2648% ♈   \aries, \:aries:    Aries
  ^^^^2649% ♉   \taurus, \:taurus:  Taurus
  ^^^^264a% ♊   \gemini, \:gemini:  Gemini
  ^^^^264b% ♋   \cancer, \:cancer:  Cancer
  ^^^^264c% ♌   \leo, \:leo:    Leo
  ^^^^264d% ♍   \virgo, \:virgo:    Virgo
  ^^^^264e% ♎   \libra, \:libra:    Libra
  ^^^^264f% ♏   \scorpio, \:scorpius:   Scorpius
  ^^^^2650% ♐   \sagittarius, \:sagittarius:    Sagittarius
  ^^^^2651% ♑   \capricornus, \:capricorn:  Capricorn
  ^^^^2652% ♒   \aquarius, \:aquarius:  Aquarius
  ^^^^2653% ♓   \pisces, \:pisces:  Pisces
  ^^^^2660% ♠   \spadesuit, \:spades:   Black Spade Suit
  ^^^^2661% ♡   \heartsuit  White Heart Suit
  ^^^^2662% ♢   \diamondsuit    White Diamond Suit
  ^^^^2663% ♣   \clubsuit, \:clubs: Black Club Suit
  ^^^^2664% ♤   \varspadesuit   White Spade Suit
  ^^^^2665% ♥   \varheartsuit, \:hearts:    Black Heart Suit
  ^^^^2666% ♦   \vardiamondsuit, \:diamonds:    Black Diamond Suit
  ^^^^2667% ♧   \varclubsuit    White Club Suit
  ^^^^2668% ♨   \:hotsprings:   Hot Springs
  ^^^^2669% ♩   \quarternote    Quarter Note
  ^^^^266a% ♪   \eighthnote Eighth Note
  ^^^^266b% ♫   \twonotes   Beamed Eighth Notes / Barred Eighth Notes
  ^^^^266d% ♭   \flat   Music Flat Sign / Flat
  ^^^^266e% ♮   \natural    Music Natural Sign / Natural
  ^^^^266f% ♯   \sharp  Music Sharp Sign / Sharp
  ^^^^267b% ♻   \:recycle:  Black Universal Recycling Symbol
  ^^^^267e% ♾   \acidfree   Permanent Paper Sign
  ^^^^267f% ♿   \:wheelchair:   Wheelchair Symbol
  ^^^^2680% ⚀   \dicei  Die Face-1
  ^^^^2681% ⚁   \diceii Die Face-2
  ^^^^2682% ⚂   \diceiii    Die Face-3
  ^^^^2683% ⚃   \diceiv Die Face-4
  ^^^^2684% ⚄   \dicev  Die Face-5
  ^^^^2685% ⚅   \dicevi Die Face-6
  ^^^^2686% ⚆   \circledrightdot    White Circle With Dot Right
  ^^^^2687% ⚇   \circledtwodots White Circle With Two Dots
  ^^^^2688% ⚈   \blackcircledrightdot   Black Circle With White Dot Right
  ^^^^2689% ⚉   \blackcircledtwodots    Black Circle With Two White Dots
  ^^^^2693% ⚓   \:anchor:   Anchor
  ^^^^26a0% ⚠   \:warning:  Warning Sign
  ^^^^26a1% ⚡   \:zap:  High Voltage Sign
  ^^^^26a5% ⚥   \hermaphrodite  Male And Female Sign
  ^^^^26aa% ⚪   \mdwhtcircle, \:white_circle:   Medium White Circle
  ^^^^26ab% ⚫   \mdblkcircle, \:black_circle:   Medium Black Circle
  ^^^^26ac% ⚬   \mdsmwhtcircle  Medium Small White Circle
  ^^^^26b2% ⚲   \neuter Neuter
  ^^^^26bd% ⚽   \:soccer:   Soccer Ball
  ^^^^26be% ⚾   \:baseball: Baseball
  ^^^^26c4% ⛄   \:snowman:  Snowman Without Snow
  ^^^^26c5% ⛅   \:partly_sunny: Sun Behind Cloud
  ^^^^26ce% ⛎   \:ophiuchus:    Ophiuchus
  ^^^^26d4% ⛔   \:no_entry: No Entry
  ^^^^26ea% ⛪   \:church:   Church
  ^^^^26f2% ⛲   \:fountain: Fountain
  ^^^^26f3% ⛳   \:golf: Flag In Hole
  ^^^^26f5% ⛵   \:boat: Sailboat
  ^^^^26fa% ⛺   \:tent: Tent
  ^^^^26fd% ⛽   \:fuelpump: Fuel Pump
  ^^^^2702% ✂   \:scissors: Black Scissors
  ^^^^2705% ✅   \:white_check_mark: White Heavy Check Mark
  ^^^^2708% ✈   \:airplane: Airplane
  ^^^^2709% ✉   \:email:    Envelope
  ^^^^270a% ✊   \:fist: Raised Fist
  ^^^^270b% ✋   \:hand: Raised Hand
  ^^^^270c% ✌   \:v:    Victory Hand
  ^^^^270f% ✏   \:pencil2:  Pencil
  ^^^^2712% ✒   \:black_nib:    Black Nib
  ^^^^2713% ✓   \checkmark  Check Mark
  ^^^^2714% ✔   \:heavy_check_mark: Heavy Check Mark
  ^^^^2716% ✖   \:heavy_multiplication_x:   Heavy Multiplication X
  ^^^^2720% ✠   \maltese    Maltese Cross
  ^^^^2728% ✨   \:sparkles: Sparkles
  ^^^^272a% ✪   \circledstar    Circled White Star
  ^^^^2733% ✳   \:eight_spoked_asterisk:    Eight Spoked Asterisk
  ^^^^2734% ✴   \:eight_pointed_black_star: Eight Pointed Black Star
  ^^^^2736% ✶   \varstar    Six Pointed Black Star
  ^^^^273d% ✽   \dingasterisk   Heavy Teardrop-Spoked Asterisk
  ^^^^2744% ❄   \:snowflake:    Snowflake
  ^^^^2747% ❇   \:sparkle:  Sparkle
  ^^^^274c% ❌   \:x:    Cross Mark
  ^^^^274e% ❎   \:negative_squared_cross_mark:  Negative Squared Cross Mark
  ^^^^2753% ❓   \:question: Black Question Mark Ornament
  ^^^^2754% ❔   \:grey_question:    White Question Mark Ornament
  ^^^^2755% ❕   \:grey_exclamation: White Exclamation Mark Ornament
  ^^^^2757% ❗   \:exclamation:  Heavy Exclamation Mark Symbol
  ^^^^2764% ❤   \:heart:    Heavy Black Heart
  ^^^^2795% ➕   \:heavy_plus_sign:  Heavy Plus Sign
  ^^^^2796% ➖   \:heavy_minus_sign: Heavy Minus Sign
  ^^^^2797% ➗   \:heavy_division_sign:  Heavy Division Sign
  ^^^^279b% ➛   \draftingarrow  Drafting Point Rightwards Arrow / Drafting Point Right Arrow
  ^^^^27a1% ➡   \:arrow_right:  Black Rightwards Arrow / Black Right Arrow
  ^^^^27b0% ➰   \:curly_loop:   Curly Loop
  ^^^^27bf% ➿   \:loop: Double Curly Loop
  ^^^^27c0% ⟀   \threedangle    Three Dimensional Angle
  ^^^^27c1% ⟁   \whiteinwhitetriangle   White Triangle Containing Small White Triangle
  ^^^^27c2% ⟂   \perp   Perpendicular
  ^^^^27c8% ⟈   \bsolhsub   Reverse Solidus Preceding Subset
  ^^^^27c9% ⟉   \suphsol    Superset Preceding Solidus
  ^^^^27d1% ⟑   \wedgedot   And With Dot
  ^^^^27d2% ⟒   \upin   Element Of Opening Upwards
  ^^^^27d5% ⟕   \leftouterjoin  Left Outer Join
  ^^^^27d6% ⟖   \rightouterjoin Right Outer Join
  ^^^^27d7% ⟗   \fullouterjoin  Full Outer Join
  ^^^^27d8% ⟘   \bigbot Large Up Tack
  ^^^^27d9% ⟙   \bigtop Large Down Tack
  ^^^^27e6% ⟦   \llbracket, \openbracketleft    Mathematical Left White Square Bracket
  ^^^^27e7% ⟧   \openbracketright, \rrbracket   Mathematical Right White Square Bracket
  ^^^^27e8% ⟨   \langle Mathematical Left Angle Bracket
  ^^^^27e9% ⟩   \rangle Mathematical Right Angle Bracket
  ^^^^27f0% ⟰   \UUparrow   Upwards Quadruple Arrow
  ^^^^27f1% ⟱   \DDownarrow Downwards Quadruple Arrow
  ^^^^27f5% ⟵   \longleftarrow  Long Leftwards Arrow
  ^^^^27f6% ⟶   \longrightarrow Long Rightwards Arrow
  ^^^^27f7% ⟷   \longleftrightarrow Long Left Right Arrow
  ^^^^27f8% ⟸   \impliedby, \Longleftarrow  Long Leftwards Double Arrow
  ^^^^27f9% ⟹   \implies, \Longrightarrow   Long Rightwards Double Arrow
  ^^^^27fa% ⟺   \Longleftrightarrow, \iff   Long Left Right Double Arrow
  ^^^^27fb% ⟻   \longmapsfrom   Long Leftwards Arrow From Bar
  ^^^^27fc% ⟼   \longmapsto Long Rightwards Arrow From Bar
  ^^^^27fd% ⟽   \Longmapsfrom   Long Leftwards Double Arrow From Bar
  ^^^^27fe% ⟾   \Longmapsto Long Rightwards Double Arrow From Bar
  ^^^^27ff% ⟿   \longrightsquigarrow    Long Rightwards Squiggle Arrow
  ^^^^2900% ⤀   \nvtwoheadrightarrow    Rightwards Two-Headed Arrow With Vertical Stroke
  ^^^^2901% ⤁   \nVtwoheadrightarrow    Rightwards Two-Headed Arrow With Double Vertical Stroke
  ^^^^2902% ⤂   \nvLeftarrow    Leftwards Double Arrow With Vertical Stroke
  ^^^^2903% ⤃   \nvRightarrow   Rightwards Double Arrow With Vertical Stroke
  ^^^^2904% ⤄   \nvLeftrightarrow   Left Right Double Arrow With Vertical Stroke
  ^^^^2905% ⤅   \twoheadmapsto  Rightwards Two-Headed Arrow From Bar
  ^^^^2906% ⤆   \Mapsfrom   Leftwards Double Arrow From Bar
  ^^^^2907% ⤇   \Mapsto Rightwards Double Arrow From Bar
  ^^^^2908% ⤈   \downarrowbarred    Downwards Arrow With Horizontal Stroke
  ^^^^2909% ⤉   \uparrowbarred  Upwards Arrow With Horizontal Stroke
  ^^^^290a% ⤊   \Uuparrow   Upwards Triple Arrow
  ^^^^290b% ⤋   \Ddownarrow Downwards Triple Arrow
  ^^^^290c% ⤌   \leftbkarrow    Leftwards Double Dash Arrow
  ^^^^290d% ⤍   \bkarow Rightwards Double Dash Arrow
  ^^^^290e% ⤎   \leftdbkarrow   Leftwards Triple Dash Arrow
  ^^^^290f% ⤏   \dbkarow    Rightwards Triple Dash Arrow
  ^^^^2910% ⤐   \drbkarrow  Rightwards Two-Headed Triple Dash Arrow
  ^^^^2911% ⤑   \rightdotarrow  Rightwards Arrow With Dotted Stem
  ^^^^2912% ⤒   \UpArrowBar Upwards Arrow To Bar
  ^^^^2913% ⤓   \DownArrowBar   Downwards Arrow To Bar
  ^^^^2914% ⤔   \nvrightarrowtail   Rightwards Arrow With Tail With Vertical Stroke
  ^^^^2915% ⤕   \nVrightarrowtail   Rightwards Arrow With Tail With Double Vertical Stroke
  ^^^^2916% ⤖   \twoheadrightarrowtail  Rightwards Two-Headed Arrow With Tail
  ^^^^2917% ⤗   \nvtwoheadrightarrowtail    Rightwards Two-Headed Arrow With Tail With Vertical Stroke
  ^^^^2918% ⤘   \nVtwoheadrightarrowtail    Rightwards Two-Headed Arrow With Tail With Double Vertical Stroke
  ^^^^291d% ⤝   \diamondleftarrow   Leftwards Arrow To Black Diamond
  ^^^^291e% ⤞   \rightarrowdiamond  Rightwards Arrow To Black Diamond
  ^^^^291f% ⤟   \diamondleftarrowbar    Leftwards Arrow From Bar To Black Diamond
  ^^^^2920% ⤠   \barrightarrowdiamond   Rightwards Arrow From Bar To Black Diamond
  ^^^^2925% ⤥   \hksearow   South East Arrow With Hook
  ^^^^2926% ⤦   \hkswarow   South West Arrow With Hook
  ^^^^2927% ⤧   \tona   North West Arrow And North East Arrow
  ^^^^2928% ⤨   \toea   North East Arrow And South East Arrow
  ^^^^2929% ⤩   \tosa   South East Arrow And South West Arrow
  ^^^^292a% ⤪   \towa   South West Arrow And North West Arrow
  ^^^^292b% ⤫   \rdiagovfdiag   Rising Diagonal Crossing Falling Diagonal
  ^^^^292c% ⤬   \fdiagovrdiag   Falling Diagonal Crossing Rising Diagonal
  ^^^^292d% ⤭   \seovnearrow    South East Arrow Crossing North East Arrow
  ^^^^292e% ⤮   \neovsearrow    North East Arrow Crossing South East Arrow
  ^^^^292f% ⤯   \fdiagovnearrow Falling Diagonal Crossing North East Arrow
  ^^^^2930% ⤰   \rdiagovsearrow Rising Diagonal Crossing South East Arrow
  ^^^^2931% ⤱   \neovnwarrow    North East Arrow Crossing North West Arrow
  ^^^^2932% ⤲   \nwovnearrow    North West Arrow Crossing North East Arrow
  ^^^^2934% ⤴   \:arrow_heading_up: Arrow Pointing Rightwards Then Curving Upwards
  ^^^^2935% ⤵   \:arrow_heading_down:   Arrow Pointing Rightwards Then Curving Downwards
  ^^^^2942% ⥂   \Rlarr  Rightwards Arrow Above Short Leftwards Arrow
  ^^^^2944% ⥄   \rLarr  Short Rightwards Arrow Above Leftwards Arrow
  ^^^^2945% ⥅   \rightarrowplus Rightwards Arrow With Plus Below
  ^^^^2946% ⥆   \leftarrowplus  Leftwards Arrow With Plus Below
  ^^^^2947% ⥇   \rarrx  Rightwards Arrow Through X
  ^^^^2948% ⥈   \leftrightarrowcircle   Left Right Arrow Through Small Circle
  ^^^^2949% ⥉   \twoheaduparrowcircle   Upwards Two-Headed Arrow From Small Circle
  ^^^^294a% ⥊   \leftrightharpoonupdown Left Barb Up Right Barb Down Harpoon
  ^^^^294b% ⥋   \leftrightharpoondownup Left Barb Down Right Barb Up Harpoon
  ^^^^294c% ⥌   \updownharpoonrightleft Up Barb Right Down Barb Left Harpoon
  ^^^^294d% ⥍   \updownharpoonleftright Up Barb Left Down Barb Right Harpoon
  ^^^^294e% ⥎   \LeftRightVector    Left Barb Up Right Barb Up Harpoon
  ^^^^294f% ⥏   \RightUpDownVector  Up Barb Right Down Barb Right Harpoon
  ^^^^2950% ⥐   \DownLeftRightVector    Left Barb Down Right Barb Down Harpoon
  ^^^^2951% ⥑   \LeftUpDownVector   Up Barb Left Down Barb Left Harpoon
  ^^^^2952% ⥒   \LeftVectorBar  Leftwards Harpoon With Barb Up To Bar
  ^^^^2953% ⥓   \RightVectorBar Rightwards Harpoon With Barb Up To Bar
  ^^^^2954% ⥔   \RightUpVectorBar   Upwards Harpoon With Barb Right To Bar
  ^^^^2955% ⥕   \RightDownVectorBar Downwards Harpoon With Barb Right To Bar
  ^^^^2956% ⥖   \DownLeftVectorBar  Leftwards Harpoon With Barb Down To Bar
  ^^^^2957% ⥗   \DownRightVectorBar Rightwards Harpoon With Barb Down To Bar
  ^^^^2958% ⥘   \LeftUpVectorBar    Upwards Harpoon With Barb Left To Bar
  ^^^^2959% ⥙   \LeftDownVectorBar  Downwards Harpoon With Barb Left To Bar
  ^^^^295a% ⥚   \LeftTeeVector  Leftwards Harpoon With Barb Up From Bar
  ^^^^295b% ⥛   \RightTeeVector Rightwards Harpoon With Barb Up From Bar
  ^^^^295c% ⥜   \RightUpTeeVector   Upwards Harpoon With Barb Right From Bar
  ^^^^295d% ⥝   \RightDownTeeVector Downwards Harpoon With Barb Right From Bar
  ^^^^295e% ⥞   \DownLeftTeeVector  Leftwards Harpoon With Barb Down From Bar
  ^^^^295f% ⥟   \DownRightTeeVector Rightwards Harpoon With Barb Down From Bar
  ^^^^2960% ⥠   \LeftUpTeeVector    Upwards Harpoon With Barb Left From Bar
  ^^^^2961% ⥡   \LeftDownTeeVector  Downwards Harpoon With Barb Left From Bar
  ^^^^2962% ⥢   \leftharpoonsupdown Leftwards Harpoon With Barb Up Above Leftwards Harpoon With Barb Down
  ^^^^2963% ⥣   \upharpoonsleftright    Upwards Harpoon With Barb Left Beside Upwards Harpoon With Barb Right
  ^^^^2964% ⥤   \rightharpoonsupdown    Rightwards Harpoon With Barb Up Above Rightwards Harpoon With Barb Down
  ^^^^2965% ⥥   \downharpoonsleftright  Downwards Harpoon With Barb Left Beside Downwards Harpoon With Barb Right
  ^^^^2966% ⥦   \leftrightharpoonsup    Leftwards Harpoon With Barb Up Above Rightwards Harpoon With Barb Up
  ^^^^2967% ⥧   \leftrightharpoonsdown  Leftwards Harpoon With Barb Down Above Rightwards Harpoon With Barb Down
  ^^^^2968% ⥨   \rightleftharpoonsup    Rightwards Harpoon With Barb Up Above Leftwards Harpoon With Barb Up
  ^^^^2969% ⥩   \rightleftharpoonsdown  Rightwards Harpoon With Barb Down Above Leftwards Harpoon With Barb Down
  ^^^^296a% ⥪   \leftharpoonupdash  Leftwards Harpoon With Barb Up Above Long Dash
  ^^^^296b% ⥫   \dashleftharpoondown    Leftwards Harpoon With Barb Down Below Long Dash
  ^^^^296c% ⥬   \rightharpoonupdash Rightwards Harpoon With Barb Up Above Long Dash
  ^^^^296d% ⥭   \dashrightharpoondown   Rightwards Harpoon With Barb Down Below Long Dash
  ^^^^296e% ⥮   \UpEquilibrium  Upwards Harpoon With Barb Left Beside Downwards Harpoon With Barb Right
  ^^^^296f% ⥯   \ReverseUpEquilibrium   Downwards Harpoon With Barb Left Beside Upwards Harpoon With Barb Right
  ^^^^2970% ⥰   \RoundImplies   Right Double Arrow With Rounded Head
  ^^^^2980% ⦀   \Vvert  Triple Vertical Bar Delimiter
  ^^^^2986% ⦆   \Elroang    Right White Parenthesis
  ^^^^2999% ⦙   \ddfnc  Dotted Fence
  ^^^^299b% ⦛   \measuredangleleft  Measured Angle Opening Left
  ^^^^299c% ⦜   \Angle  Right Angle Variant With Square
  ^^^^299d% ⦝   \rightanglemdot Measured Right Angle With Dot
  ^^^^299e% ⦞   \angles Angle With S Inside
  ^^^^299f% ⦟   \angdnr Acute Angle
  ^^^^29a0% ⦠   \lpargt Spherical Angle Opening Left
  ^^^^29a1% ⦡   \sphericalangleup   Spherical Angle Opening Up
  ^^^^29a2% ⦢   \turnangle  Turned Angle
  ^^^^29a3% ⦣   \revangle   Reversed Angle
  ^^^^29a4% ⦤   \angleubar  Angle With Underbar
  ^^^^29a5% ⦥   \revangleubar   Reversed Angle With Underbar
  ^^^^29a6% ⦦   \wideangledown  Oblique Angle Opening Up
  ^^^^29a7% ⦧   \wideangleup    Oblique Angle Opening Down
  ^^^^29a8% ⦨   \measanglerutone    Measured Angle With Open Arm Ending In Arrow Pointing Up And Right
  ^^^^29a9% ⦩   \measanglelutonw    Measured Angle With Open Arm Ending In Arrow Pointing Up And Left
  ^^^^29aa% ⦪   \measanglerdtose    Measured Angle With Open Arm Ending In Arrow Pointing Down And Right
  ^^^^29ab% ⦫   \measangleldtosw    Measured Angle With Open Arm Ending In Arrow Pointing Down And Left
  ^^^^29ac% ⦬   \measangleurtone    Measured Angle With Open Arm Ending In Arrow Pointing Right And Up
  ^^^^29ad% ⦭   \measangleultonw    Measured Angle With Open Arm Ending In Arrow Pointing Left And Up
  ^^^^29ae% ⦮   \measangledrtose    Measured Angle With Open Arm Ending In Arrow Pointing Right And Down
  ^^^^29af% ⦯   \measangledltosw    Measured Angle With Open Arm Ending In Arrow Pointing Left And Down
  ^^^^29b0% ⦰   \revemptyset    Reversed Empty Set
  ^^^^29b1% ⦱   \emptysetobar   Empty Set With Overbar
  ^^^^29b2% ⦲   \emptysetocirc  Empty Set With Small Circle Above
  ^^^^29b3% ⦳   \emptysetoarr   Empty Set With Right Arrow Above
  ^^^^29b4% ⦴   \emptysetoarrl  Empty Set With Left Arrow Above
  ^^^^29b7% ⦷   \circledparallel    Circled Parallel
  ^^^^29b8% ⦸   \obslash    Circled Reverse Solidus
  ^^^^29bc% ⦼   \odotslashdot   Circled Anticlockwise-Rotated Division Sign
  ^^^^29be% ⦾   \circledwhitebullet Circled White Bullet
  ^^^^29bf% ⦿   \circledbullet  Circled Bullet
  ^^^^29c0% ⧀   \olessthan  Circled Less-Than
  ^^^^29c1% ⧁   \ogreaterthan   Circled Greater-Than
  ^^^^29c4% ⧄   \boxdiag    Squared Rising Diagonal Slash
  ^^^^29c5% ⧅   \boxbslash  Squared Falling Diagonal Slash
  ^^^^29c6% ⧆   \boxast Squared Asterisk
  ^^^^29c7% ⧇   \boxcircle  Squared Small Circle
  ^^^^29ca% ⧊   \Lap    Triangle With Dot Above
  ^^^^29cb% ⧋   \defas  Triangle With Underbar
  ^^^^29cf% ⧏   \LeftTriangleBar    Left Triangle Beside Vertical Bar
  ^^^^29cf% + ^^^^0338%   ⧏̸  \NotLeftTriangleBar Left Triangle Beside Vertical Bar + Combining Long Solidus Overlay / Non-Spacing Long Slash Overlay
  ^^^^29d0% ⧐   \RightTriangleBar   Vertical Bar Beside Right Triangle
  ^^^^29d0% + ^^^^0338%   ⧐̸  \NotRightTriangleBar    Vertical Bar Beside Right Triangle + Combining Long Solidus Overlay / Non-Spacing Long Slash Overlay
  ^^^^29df% ⧟   \dualmap    Double-Ended Multimap
  ^^^^29e1% ⧡   \lrtriangleeq   Increases As
  ^^^^29e2% ⧢   \shuffle    Shuffle Product
  ^^^^29e3% ⧣   \eparsl Equals Sign And Slanted Parallel
  ^^^^29e4% ⧤   \smeparsl   Equals Sign And Slanted Parallel With Tilde Above
  ^^^^29e5% ⧥   \eqvparsl   Identical To And Slanted Parallel
  ^^^^29eb% ⧫   \blacklozenge   Black Lozenge
  ^^^^29f4% ⧴   \RuleDelayed    Rule-Delayed
  ^^^^29f6% ⧶   \dsol   Solidus With Overbar
  ^^^^29f7% ⧷   \rsolbar    Reverse Solidus With Horizontal Stroke
  ^^^^29fa% ⧺   \doubleplus Double Plus
  ^^^^29fb% ⧻   \tripleplus Triple Plus
  ^^^^2a00% ⨀   \bigodot    N-Ary Circled Dot Operator
  ^^^^2a01% ⨁   \bigoplus   N-Ary Circled Plus Operator
  ^^^^2a02% ⨂   \bigotimes  N-Ary Circled Times Operator
  ^^^^2a03% ⨃   \bigcupdot  N-Ary Union Operator With Dot
  ^^^^2a04% ⨄   \biguplus   N-Ary Union Operator With Plus
  ^^^^2a05% ⨅   \bigsqcap   N-Ary Square Intersection Operator
  ^^^^2a06% ⨆   \bigsqcup   N-Ary Square Union Operator
  ^^^^2a07% ⨇   \conjquant  Two Logical And Operator
  ^^^^2a08% ⨈   \disjquant  Two Logical Or Operator
  ^^^^2a09% ⨉   \bigtimes   N-Ary Times Operator
  ^^^^2a0a% ⨊   \modtwosum  Modulo Two Sum
  ^^^^2a0b% ⨋   \sumint Summation With Integral
  ^^^^2a0c% ⨌   \iiiint Quadruple Integral Operator
  ^^^^2a0d% ⨍   \intbar Finite Part Integral
  ^^^^2a0e% ⨎   \intBar Integral With Double Stroke
  ^^^^2a0f% ⨏   \clockoint  Integral Average With Slash
  ^^^^2a10% ⨐   \cirfnint   Circulation Function
  ^^^^2a11% ⨑   \awint  Anticlockwise Integration
  ^^^^2a12% ⨒   \rppolint   Line Integration With Rectangular Path Around Pole
  ^^^^2a13% ⨓   \scpolint   Line Integration With Semicircular Path Around Pole
  ^^^^2a14% ⨔   \npolint    Line Integration Not Including The Pole
  ^^^^2a15% ⨕   \pointint   Integral Around A Point Operator
  ^^^^2a16% ⨖   \sqrint Quaternion Integral Operator
  ^^^^2a18% ⨘   \intx   Integral With Times Sign
  ^^^^2a19% ⨙   \intcap Integral With Intersection
  ^^^^2a1a% ⨚   \intcup Integral With Union
  ^^^^2a1b% ⨛   \upint  Integral With Overbar
  ^^^^2a1c% ⨜   \lowint Integral With Underbar
  ^^^^2a1d% ⨝   \Join, \join    Join
  ^^^^2a1f% ⨟   \bbsemi Z Notation Schema Composition
  ^^^^2a22% ⨢   \ringplus   Plus Sign With Small Circle Above
  ^^^^2a23% ⨣   \plushat    Plus Sign With Circumflex Accent Above
  ^^^^2a24% ⨤   \simplus    Plus Sign With Tilde Above
  ^^^^2a25% ⨥   \plusdot    Plus Sign With Dot Below
  ^^^^2a26% ⨦   \plussim    Plus Sign With Tilde Below
  ^^^^2a27% ⨧   \plussubtwo Plus Sign With Subscript Two
  ^^^^2a28% ⨨   \plustrif   Plus Sign With Black Triangle
  ^^^^2a29% ⨩   \commaminus Minus Sign With Comma Above
  ^^^^2a2a% ⨪   \minusdot   Minus Sign With Dot Below
  ^^^^2a2b% ⨫   \minusfdots Minus Sign With Falling Dots
  ^^^^2a2c% ⨬   \minusrdots Minus Sign With Rising Dots
  ^^^^2a2d% ⨭   \opluslhrim Plus Sign In Left Half Circle
  ^^^^2a2e% ⨮   \oplusrhrim Plus Sign In Right Half Circle
  ^^^^2a2f% ⨯   \Times  Vector Or Cross Product
  ^^^^2a30% ⨰   \dottimes   Multiplication Sign With Dot Above
  ^^^^2a31% ⨱   \timesbar   Multiplication Sign With Underbar
  ^^^^2a32% ⨲   \btimes Semidirect Product With Bottom Closed
  ^^^^2a33% ⨳   \smashtimes Smash Product
  ^^^^2a34% ⨴   \otimeslhrim    Multiplication Sign In Left Half Circle
  ^^^^2a35% ⨵   \otimesrhrim    Multiplication Sign In Right Half Circle
  ^^^^2a36% ⨶   \otimeshat  Circled Multiplication Sign With Circumflex Accent
  ^^^^2a37% ⨷   \Otimes Multiplication Sign In Double Circle
  ^^^^2a38% ⨸   \odiv   Circled Division Sign
  ^^^^2a39% ⨹   \triangleplus   Plus Sign In Triangle
  ^^^^2a3a% ⨺   \triangleminus  Minus Sign In Triangle
  ^^^^2a3b% ⨻   \triangletimes  Multiplication Sign In Triangle
  ^^^^2a3c% ⨼   \intprod    Interior Product
  ^^^^2a3d% ⨽   \intprodr   Righthand Interior Product
  ^^^^2a3f% ⨿   \amalg  Amalgamation Or Coproduct
  ^^^^2a40% ⩀   \capdot Intersection With Dot
  ^^^^2a41% ⩁   \uminus Union With Minus Sign
  ^^^^2a42% ⩂   \barcup Union With Overbar
  ^^^^2a43% ⩃   \barcap Intersection With Overbar
  ^^^^2a44% ⩄   \capwedge   Intersection With Logical And
  ^^^^2a45% ⩅   \cupvee Union With Logical Or
  ^^^^2a4a% ⩊   \twocups    Union Beside And Joined With Union
  ^^^^2a4b% ⩋   \twocaps    Intersection Beside And Joined With Intersection
  ^^^^2a4c% ⩌   \closedvarcup   Closed Union With Serifs
  ^^^^2a4d% ⩍   \closedvarcap   Closed Intersection With Serifs
  ^^^^2a4e% ⩎   \Sqcap  Double Square Intersection
  ^^^^2a4f% ⩏   \Sqcup  Double Square Union
  ^^^^2a50% ⩐   \closedvarcupsmashprod  Closed Union With Serifs And Smash Product
  ^^^^2a51% ⩑   \wedgeodot  Logical And With Dot Above
  ^^^^2a52% ⩒   \veeodot    Logical Or With Dot Above
  ^^^^2a53% ⩓   \And    Double Logical And
  ^^^^2a54% ⩔   \Or Double Logical Or
  ^^^^2a55% ⩕   \wedgeonwedge   Two Intersecting Logical And
  ^^^^2a56% ⩖   \ElOr   Two Intersecting Logical Or
  ^^^^2a57% ⩗   \bigslopedvee   Sloping Large Or
  ^^^^2a58% ⩘   \bigslopedwedge Sloping Large And
  ^^^^2a5a% ⩚   \wedgemidvert   Logical And With Middle Stem
  ^^^^2a5b% ⩛   \veemidvert Logical Or With Middle Stem
  ^^^^2a5c% ⩜   \midbarwedge    Logical And With Horizontal Dash
  ^^^^2a5d% ⩝   \midbarvee  Logical Or With Horizontal Dash
  ^^^^2a5e% ⩞   \perspcorrespond    Logical And With Double Overbar
  ^^^^2a5f% ⩟   \minhat Logical And With Underbar
  ^^^^2a60% ⩠   \wedgedoublebar Logical And With Double Underbar
  ^^^^2a61% ⩡   \varveebar  Small Vee With Underbar
  ^^^^2a62% ⩢   \doublebarvee   Logical Or With Double Overbar
  ^^^^2a63% ⩣   \veedoublebar   Logical Or With Double Underbar
  ^^^^2a66% ⩦   \eqdot  Equals Sign With Dot Below
  ^^^^2a67% ⩧   \dotequiv   Identical With Dot Above
  ^^^^2a6a% ⩪   \dotsim Tilde Operator With Dot Above
  ^^^^2a6b% ⩫   \simrdots   Tilde Operator With Rising Dots
  ^^^^2a6c% ⩬   \simminussim    Similar Minus Similar
  ^^^^2a6d% ⩭   \congdot    Congruent With Dot Above
  ^^^^2a6e% ⩮   \asteq  Equals With Asterisk
  ^^^^2a6f% ⩯   \hatapprox  Almost Equal To With Circumflex Accent
  ^^^^2a70% ⩰   \approxeqq  Approximately Equal Or Equal To
  ^^^^2a71% ⩱   \eqqplus    Equals Sign Above Plus Sign
  ^^^^2a72% ⩲   \pluseqq    Plus Sign Above Equals Sign
  ^^^^2a73% ⩳   \eqqsim Equals Sign Above Tilde Operator
  ^^^^2a74% ⩴   \Coloneq    Double Colon Equal
  ^^^^2a75% ⩵   \Equal  Two Consecutive Equals Signs
  ^^^^2a76% ⩶   \eqeqeq Three Consecutive Equals Signs
  ^^^^2a77% ⩷   \ddotseq    Equals Sign With Two Dots Above And Two Dots Below
  ^^^^2a78% ⩸   \equivDD    Equivalent With Four Dots Above
  ^^^^2a79% ⩹   \ltcir  Less-Than With Circle Inside
  ^^^^2a7a% ⩺   \gtcir  Greater-Than With Circle Inside
  ^^^^2a7b% ⩻   \ltquest    Less-Than With Question Mark Above
  ^^^^2a7c% ⩼   \gtquest    Greater-Than With Question Mark Above
  ^^^^2a7d% ⩽   \leqslant   Less-Than Or Slanted Equal To
  ^^^^2a7d% + ^^^^0338%   ⩽̸  \nleqslant  Less-Than Or Slanted Equal To + Combining Long Solidus Overlay / Non-Spacing Long Slash Overlay
  ^^^^2a7e% ⩾   \geqslant   Greater-Than Or Slanted Equal To
  ^^^^2a7e% + ^^^^0338%   ⩾̸  \ngeqslant  Greater-Than Or Slanted Equal To + Combining Long Solidus Overlay / Non-Spacing Long Slash Overlay
  ^^^^2a7f% ⩿   \lesdot Less-Than Or Slanted Equal To With Dot Inside
  ^^^^2a80% ⪀   \gesdot Greater-Than Or Slanted Equal To With Dot Inside
  ^^^^2a81% ⪁   \lesdoto    Less-Than Or Slanted Equal To With Dot Above
  ^^^^2a82% ⪂   \gesdoto    Greater-Than Or Slanted Equal To With Dot Above
  ^^^^2a83% ⪃   \lesdotor   Less-Than Or Slanted Equal To With Dot Above Right
  ^^^^2a84% ⪄   \gesdotol   Greater-Than Or Slanted Equal To With Dot Above Left
  ^^^^2a85% ⪅   \lessapprox Less-Than Or Approximate
  ^^^^2a86% ⪆   \gtrapprox  Greater-Than Or Approximate
  ^^^^2a87% ⪇   \lneq   Less-Than And Single-Line Not Equal To
  ^^^^2a88% ⪈   \gneq   Greater-Than And Single-Line Not Equal To
  ^^^^2a89% ⪉   \lnapprox   Less-Than And Not Approximate
  ^^^^2a8a% ⪊   \gnapprox   Greater-Than And Not Approximate
  ^^^^2a8b% ⪋   \lesseqqgtr Less-Than Above Double-Line Equal Above Greater-Than
  ^^^^2a8c% ⪌   \gtreqqless Greater-Than Above Double-Line Equal Above Less-Than
  ^^^^2a8d% ⪍   \lsime  Less-Than Above Similar Or Equal
  ^^^^2a8e% ⪎   \gsime  Greater-Than Above Similar Or Equal
  ^^^^2a8f% ⪏   \lsimg  Less-Than Above Similar Above Greater-Than
  ^^^^2a90% ⪐   \gsiml  Greater-Than Above Similar Above Less-Than
  ^^^^2a91% ⪑   \lgE    Less-Than Above Greater-Than Above Double-Line Equal
  ^^^^2a92% ⪒   \glE    Greater-Than Above Less-Than Above Double-Line Equal
  ^^^^2a93% ⪓   \lesges Less-Than Above Slanted Equal Above Greater-Than Above Slanted Equal
  ^^^^2a94% ⪔   \gesles Greater-Than Above Slanted Equal Above Less-Than Above Slanted Equal
  ^^^^2a95% ⪕   \eqslantless    Slanted Equal To Or Less-Than
  ^^^^2a96% ⪖   \eqslantgtr Slanted Equal To Or Greater-Than
  ^^^^2a97% ⪗   \elsdot Slanted Equal To Or Less-Than With Dot Inside
  ^^^^2a98% ⪘   \egsdot Slanted Equal To Or Greater-Than With Dot Inside
  ^^^^2a99% ⪙   \eqqless    Double-Line Equal To Or Less-Than
  ^^^^2a9a% ⪚   \eqqgtr Double-Line Equal To Or Greater-Than
  ^^^^2a9b% ⪛   \eqqslantless   Double-Line Slanted Equal To Or Less-Than
  ^^^^2a9c% ⪜   \eqqslantgtr    Double-Line Slanted Equal To Or Greater-Than
  ^^^^2a9d% ⪝   \simless    Similar Or Less-Than
  ^^^^2a9e% ⪞   \simgtr Similar Or Greater-Than
  ^^^^2a9f% ⪟   \simlE  Similar Above Less-Than Above Equals Sign
  ^^^^2aa0% ⪠   \simgE  Similar Above Greater-Than Above Equals Sign
  ^^^^2aa1% ⪡   \NestedLessLess Double Nested Less-Than
  ^^^^2aa1% + ^^^^0338%   ⪡̸  \NotNestedLessLess  Double Nested Less-Than + Combining Long Solidus Overlay / Non-Spacing Long Slash Overlay
  ^^^^2aa2% ⪢   \NestedGreaterGreater   Double Nested Greater-Than
  ^^^^2aa2% + ^^^^0338%   ⪢̸  \NotNestedGreaterGreater    Double Nested Greater-Than + Combining Long Solidus Overlay / Non-Spacing Long Slash Overlay
  ^^^^2aa3% ⪣   \partialmeetcontraction Double Nested Less-Than With Underbar
  ^^^^2aa4% ⪤   \glj    Greater-Than Overlapping Less-Than
  ^^^^2aa5% ⪥   \gla    Greater-Than Beside Less-Than
  ^^^^2aa6% ⪦   \ltcc   Less-Than Closed By Curve
  ^^^^2aa7% ⪧   \gtcc   Greater-Than Closed By Curve
  ^^^^2aa8% ⪨   \lescc  Less-Than Closed By Curve Above Slanted Equal
  ^^^^2aa9% ⪩   \gescc  Greater-Than Closed By Curve Above Slanted Equal
  ^^^^2aaa% ⪪   \smt    Smaller Than
  ^^^^2aab% ⪫   \lat    Larger Than
  ^^^^2aac% ⪬   \smte   Smaller Than Or Equal To
  ^^^^2aad% ⪭   \late   Larger Than Or Equal To
  ^^^^2aae% ⪮   \bumpeqq    Equals Sign With Bumpy Above
  ^^^^2aaf% ⪯   \preceq Precedes Above Single-Line Equals Sign
  ^^^^2aaf% + ^^^^0338%   ⪯̸  \npreceq    Precedes Above Single-Line Equals Sign + Combining Long Solidus Overlay / Non-Spacing Long Slash Overlay
  ^^^^2ab0% ⪰   \succeq Succeeds Above Single-Line Equals Sign
  ^^^^2ab0% + ^^^^0338%   ⪰̸  \nsucceq    Succeeds Above Single-Line Equals Sign + Combining Long Solidus Overlay / Non-Spacing Long Slash Overlay
  ^^^^2ab1% ⪱   \precneq    Precedes Above Single-Line Not Equal To
  ^^^^2ab2% ⪲   \succneq    Succeeds Above Single-Line Not Equal To
  ^^^^2ab3% ⪳   \preceqq    Precedes Above Equals Sign
  ^^^^2ab4% ⪴   \succeqq    Succeeds Above Equals Sign
  ^^^^2ab5% ⪵   \precneqq   Precedes Above Not Equal To
  ^^^^2ab6% ⪶   \succneqq   Succeeds Above Not Equal To
  ^^^^2ab7% ⪷   \precapprox Precedes Above Almost Equal To
  ^^^^2ab8% ⪸   \succapprox Succeeds Above Almost Equal To
  ^^^^2ab9% ⪹   \precnapprox    Precedes Above Not Almost Equal To
  ^^^^2aba% ⪺   \succnapprox    Succeeds Above Not Almost Equal To
  ^^^^2abb% ⪻   \Prec   Double Precedes
  ^^^^2abc% ⪼   \Succ   Double Succeeds
  ^^^^2abd% ⪽   \subsetdot  Subset With Dot
  ^^^^2abe% ⪾   \supsetdot  Superset With Dot
  ^^^^2abf% ⪿   \subsetplus Subset With Plus Sign Below
  ^^^^2ac0% ⫀   \supsetplus Superset With Plus Sign Below
  ^^^^2ac1% ⫁   \submult    Subset With Multiplication Sign Below
  ^^^^2ac2% ⫂   \supmult    Superset With Multiplication Sign Below
  ^^^^2ac3% ⫃   \subedot    Subset Of Or Equal To With Dot Above
  ^^^^2ac4% ⫄   \supedot    Superset Of Or Equal To With Dot Above
  ^^^^2ac5% ⫅   \subseteqq  Subset Of Above Equals Sign
  ^^^^2ac5% + ^^^^0338%   ⫅̸  \nsubseteqq Subset Of Above Equals Sign + Combining Long Solidus Overlay / Non-Spacing Long Slash Overlay
  ^^^^2ac6% ⫆   \supseteqq  Superset Of Above Equals Sign
  ^^^^2ac6% + ^^^^0338%   ⫆̸  \nsupseteqq Superset Of Above Equals Sign + Combining Long Solidus Overlay / Non-Spacing Long Slash Overlay
  ^^^^2ac7% ⫇   \subsim Subset Of Above Tilde Operator
  ^^^^2ac8% ⫈   \supsim Superset Of Above Tilde Operator
  ^^^^2ac9% ⫉   \subsetapprox   Subset Of Above Almost Equal To
  ^^^^2aca% ⫊   \supsetapprox   Superset Of Above Almost Equal To
  ^^^^2acb% ⫋   \subsetneqq Subset Of Above Not Equal To
  ^^^^2acc% ⫌   \supsetneqq Superset Of Above Not Equal To
  ^^^^2acd% ⫍   \lsqhook    Square Left Open Box Operator
  ^^^^2ace% ⫎   \rsqhook    Square Right Open Box Operator
  ^^^^2acf% ⫏   \csub   Closed Subset
  ^^^^2ad0% ⫐   \csup   Closed Superset
  ^^^^2ad1% ⫑   \csube  Closed Subset Or Equal To
  ^^^^2ad2% ⫒   \csupe  Closed Superset Or Equal To
  ^^^^2ad3% ⫓   \subsup Subset Above Superset
  ^^^^2ad4% ⫔   \supsub Superset Above Subset
  ^^^^2ad5% ⫕   \subsub Subset Above Subset
  ^^^^2ad6% ⫖   \supsup Superset Above Superset
  ^^^^2ad7% ⫗   \suphsub    Superset Beside Subset
  ^^^^2ad8% ⫘   \supdsub    Superset Beside And Joined By Dash With Subset
  ^^^^2ad9% ⫙   \forkv  Element Of Opening Downwards
  ^^^^2adb% ⫛   \mlcp   Transversal Intersection
  ^^^^2adc% ⫝̸   \forks  Forking
  ^^^^2add% ⫝   \forksnot   Nonforking
  ^^^^2ae3% ⫣   \dashV  Double Vertical Bar Left Turnstile
  ^^^^2ae4% ⫤   \Dashv  Vertical Bar Double Left Turnstile
  ^^^^2af4% ⫴   \interleave Triple Vertical Bar Binary Relation
  ^^^^2af6% ⫶   \tdcol  Triple Colon Operator
  ^^^^2af7% ⫷   \lllnest    Triple Nested Less-Than
  ^^^^2af8% ⫸   \gggnest    Triple Nested Greater-Than
  ^^^^2af9% ⫹   \leqqslant  Double-Line Slanted Less-Than Or Equal To
  ^^^^2afa% ⫺   \geqqslant  Double-Line Slanted Greater-Than Or Equal To
  ^^^^2b05% ⬅   \:arrow_left:   Leftwards Black Arrow
  ^^^^2b06% ⬆   \:arrow_up: Upwards Black Arrow
  ^^^^2b07% ⬇   \:arrow_down:   Downwards Black Arrow
  ^^^^2b12% ⬒   \squaretopblack Square With Top Half Black
  ^^^^2b13% ⬓   \squarebotblack Square With Bottom Half Black
  ^^^^2b14% ⬔   \squareurblack  Square With Upper Right Diagonal Half Black
  ^^^^2b15% ⬕   \squarellblack  Square With Lower Left Diagonal Half Black
  ^^^^2b16% ⬖   \diamondleftblack   Diamond With Left Half Black
  ^^^^2b17% ⬗   \diamondrightblack  Diamond With Right Half Black
  ^^^^2b18% ⬘   \diamondtopblack    Diamond With Top Half Black
  ^^^^2b19% ⬙   \diamondbotblack    Diamond With Bottom Half Black
  ^^^^2b1a% ⬚   \dottedsquare   Dotted Square
  ^^^^2b1b% ⬛   \lgblksquare, \:black_large_square: Black Large Square
  ^^^^2b1c% ⬜   \lgwhtsquare, \:white_large_square: White Large Square
  ^^^^2b1d% ⬝   \vysmblksquare  Black Very Small Square
  ^^^^2b1e% ⬞   \vysmwhtsquare  White Very Small Square
  ^^^^2b1f% ⬟   \pentagonblack  Black Pentagon
  ^^^^2b20% ⬠   \pentagon   White Pentagon
  ^^^^2b21% ⬡   \varhexagon White Hexagon
  ^^^^2b22% ⬢   \varhexagonblack    Black Hexagon
  ^^^^2b23% ⬣   \hexagonblack   Horizontal Black Hexagon
  ^^^^2b24% ⬤   \lgblkcircle    Black Large Circle
  ^^^^2b25% ⬥   \mdblkdiamond   Black Medium Diamond
  ^^^^2b26% ⬦   \mdwhtdiamond   White Medium Diamond
  ^^^^2b27% ⬧   \mdblklozenge   Black Medium Lozenge
  ^^^^2b28% ⬨   \mdwhtlozenge   White Medium Lozenge
  ^^^^2b29% ⬩   \smblkdiamond   Black Small Diamond
  ^^^^2b2a% ⬪   \smblklozenge   Black Small Lozenge
  ^^^^2b2b% ⬫   \smwhtlozenge   White Small Lozenge
  ^^^^2b2c% ⬬   \blkhorzoval    Black Horizontal Ellipse
  ^^^^2b2d% ⬭   \whthorzoval    White Horizontal Ellipse
  ^^^^2b2e% ⬮   \blkvertoval    Black Vertical Ellipse
  ^^^^2b2f% ⬯   \whtvertoval    White Vertical Ellipse
  ^^^^2b30% ⬰   \circleonleftarrow  Left Arrow With Small Circle
  ^^^^2b31% ⬱   \leftthreearrows    Three Leftwards Arrows
  ^^^^2b32% ⬲   \leftarrowonoplus   Left Arrow With Circled Plus
  ^^^^2b33% ⬳   \longleftsquigarrow Long Leftwards Squiggle Arrow
  ^^^^2b34% ⬴   \nvtwoheadleftarrow Leftwards Two-Headed Arrow With Vertical Stroke
  ^^^^2b35% ⬵   \nVtwoheadleftarrow Leftwards Two-Headed Arrow With Double Vertical Stroke
  ^^^^2b36% ⬶   \twoheadmapsfrom    Leftwards Two-Headed Arrow From Bar
  ^^^^2b37% ⬷   \twoheadleftdbkarrow    Leftwards Two-Headed Triple Dash Arrow
  ^^^^2b38% ⬸   \leftdotarrow   Leftwards Arrow With Dotted Stem
  ^^^^2b39% ⬹   \nvleftarrowtail    Leftwards Arrow With Tail With Vertical Stroke
  ^^^^2b3a% ⬺   \nVleftarrowtail    Leftwards Arrow With Tail With Double Vertical Stroke
  ^^^^2b3b% ⬻   \twoheadleftarrowtail   Leftwards Two-Headed Arrow With Tail
  ^^^^2b3c% ⬼   \nvtwoheadleftarrowtail Leftwards Two-Headed Arrow With Tail With Vertical Stroke
  ^^^^2b3d% ⬽   \nVtwoheadleftarrowtail Leftwards Two-Headed Arrow With Tail With Double Vertical Stroke
  ^^^^2b3e% ⬾   \leftarrowx Leftwards Arrow Through X
  ^^^^2b3f% ⬿   \leftcurvedarrow    Wave Arrow Pointing Directly Left
  ^^^^2b40% ⭀   \equalleftarrow Equals Sign Above Leftwards Arrow
  ^^^^2b41% ⭁   \bsimilarleftarrow  Reverse Tilde Operator Above Leftwards Arrow
  ^^^^2b42% ⭂   \leftarrowbackapprox    Leftwards Arrow Above Reverse Almost Equal To
  ^^^^2b43% ⭃   \rightarrowgtr  Rightwards Arrow Through Greater-Than
  ^^^^2b44% ⭄   \rightarrowsupset   Rightwards Arrow Through Superset
  ^^^^2b45% ⭅   \LLeftarrow Leftwards Quadruple Arrow
  ^^^^2b46% ⭆   \RRightarrow    Rightwards Quadruple Arrow
  ^^^^2b47% ⭇   \bsimilarrightarrow Reverse Tilde Operator Above Rightwards Arrow
  ^^^^2b48% ⭈   \rightarrowbackapprox   Rightwards Arrow Above Reverse Almost Equal To
  ^^^^2b49% ⭉   \similarleftarrow   Tilde Operator Above Leftwards Arrow
  ^^^^2b4a% ⭊   \leftarrowapprox    Leftwards Arrow Above Almost Equal To
  ^^^^2b4b% ⭋   \leftarrowbsimilar  Leftwards Arrow Above Reverse Tilde Operator
  ^^^^2b4c% ⭌   \rightarrowbsimilar Rightwards Arrow Above Reverse Tilde Operator
  ^^^^2b50% ⭐   \medwhitestar, \:star:  White Medium Star
  ^^^^2b51% ⭑   \medblackstar   Black Small Star
  ^^^^2b52% ⭒   \smwhitestar    White Small Star
  ^^^^2b53% ⭓   \rightpentagonblack Black Right-Pointing Pentagon
  ^^^^2b54% ⭔   \rightpentagon  White Right-Pointing Pentagon
  ^^^^2b55% ⭕   \:o:    Heavy Large Circle
  ^^^^2c7c% ⱼ   \_j Latin Subscript Small Letter J
  ^^^^2c7d% ⱽ   \^V Modifier Letter Capital V
  ^^^^3012% 〒   \postalmark Postal Mark
  ^^^^3030% 〰   \:wavy_dash:    Wavy Dash
  ^^^^303d% 〽   \:part_alternation_mark:    Part Alternation Mark
  ^^^^3297% ㊗   \:congratulations:  Circled Ideograph Congratulation
  ^^^^3299% ㊙   \:secret:   Circled Ideograph Secret
  % zero-padded 6-digit hex
  ^^^^^^01d400% 𝐀   \bfA    Mathematical Bold Capital A
  ^^^^^^01d401% 𝐁   \bfB    Mathematical Bold Capital B
  ^^^^^^01d402% 𝐂   \bfC    Mathematical Bold Capital C
  ^^^^^^01d403% 𝐃   \bfD    Mathematical Bold Capital D
  ^^^^^^01d404% 𝐄   \bfE    Mathematical Bold Capital E
  ^^^^^^01d405% 𝐅   \bfF    Mathematical Bold Capital F
  ^^^^^^01d406% 𝐆   \bfG    Mathematical Bold Capital G
  ^^^^^^01d407% 𝐇   \bfH    Mathematical Bold Capital H
  ^^^^^^01d408% 𝐈   \bfI    Mathematical Bold Capital I
  ^^^^^^01d409% 𝐉   \bfJ    Mathematical Bold Capital J
  ^^^^^^01d40a% 𝐊   \bfK    Mathematical Bold Capital K
  ^^^^^^01d40b% 𝐋   \bfL    Mathematical Bold Capital L
  ^^^^^^01d40c% 𝐌   \bfM    Mathematical Bold Capital M
  ^^^^^^01d40d% 𝐍   \bfN    Mathematical Bold Capital N
  ^^^^^^01d40e% 𝐎   \bfO    Mathematical Bold Capital O
  ^^^^^^01d40f% 𝐏   \bfP    Mathematical Bold Capital P
  ^^^^^^01d410% 𝐐   \bfQ    Mathematical Bold Capital Q
  ^^^^^^01d411% 𝐑   \bfR    Mathematical Bold Capital R
  ^^^^^^01d412% 𝐒   \bfS    Mathematical Bold Capital S
  ^^^^^^01d413% 𝐓   \bfT    Mathematical Bold Capital T
  ^^^^^^01d414% 𝐔   \bfU    Mathematical Bold Capital U
  ^^^^^^01d415% 𝐕   \bfV    Mathematical Bold Capital V
  ^^^^^^01d416% 𝐖   \bfW    Mathematical Bold Capital W
  ^^^^^^01d417% 𝐗   \bfX    Mathematical Bold Capital X
  ^^^^^^01d418% 𝐘   \bfY    Mathematical Bold Capital Y
  ^^^^^^01d419% 𝐙   \bfZ    Mathematical Bold Capital Z
  ^^^^^^01d41a% 𝐚   \bfa    Mathematical Bold Small A
  ^^^^^^01d41b% 𝐛   \bfb    Mathematical Bold Small B
  ^^^^^^01d41c% 𝐜   \bfc    Mathematical Bold Small C
  ^^^^^^01d41d% 𝐝   \bfd    Mathematical Bold Small D
  ^^^^^^01d41e% 𝐞   \bfe    Mathematical Bold Small E
  ^^^^^^01d41f% 𝐟   \bff    Mathematical Bold Small F
  ^^^^^^01d420% 𝐠   \bfg    Mathematical Bold Small G
  ^^^^^^01d421% 𝐡   \bfh    Mathematical Bold Small H
  ^^^^^^01d422% 𝐢   \bfi    Mathematical Bold Small I
  ^^^^^^01d423% 𝐣   \bfj    Mathematical Bold Small J
  ^^^^^^01d424% 𝐤   \bfk    Mathematical Bold Small K
  ^^^^^^01d425% 𝐥   \bfl    Mathematical Bold Small L
  ^^^^^^01d426% 𝐦   \bfm    Mathematical Bold Small M
  ^^^^^^01d427% 𝐧   \bfn    Mathematical Bold Small N
  ^^^^^^01d428% 𝐨   \bfo    Mathematical Bold Small O
  ^^^^^^01d429% 𝐩   \bfp    Mathematical Bold Small P
  ^^^^^^01d42a% 𝐪   \bfq    Mathematical Bold Small Q
  ^^^^^^01d42b% 𝐫   \bfr    Mathematical Bold Small R
  ^^^^^^01d42c% 𝐬   \bfs    Mathematical Bold Small S
  ^^^^^^01d42d% 𝐭   \bft    Mathematical Bold Small T
  ^^^^^^01d42e% 𝐮   \bfu    Mathematical Bold Small U
  ^^^^^^01d42f% 𝐯   \bfv    Mathematical Bold Small V
  ^^^^^^01d430% 𝐰   \bfw    Mathematical Bold Small W
  ^^^^^^01d431% 𝐱   \bfx    Mathematical Bold Small X
  ^^^^^^01d432% 𝐲   \bfy    Mathematical Bold Small Y
  ^^^^^^01d433% 𝐳   \bfz    Mathematical Bold Small Z
  ^^^^^^01d434% 𝐴   \itA    Mathematical Italic Capital A
  ^^^^^^01d435% 𝐵   \itB    Mathematical Italic Capital B
  ^^^^^^01d436% 𝐶   \itC    Mathematical Italic Capital C
  ^^^^^^01d437% 𝐷   \itD    Mathematical Italic Capital D
  ^^^^^^01d438% 𝐸   \itE    Mathematical Italic Capital E
  ^^^^^^01d439% 𝐹   \itF    Mathematical Italic Capital F
  ^^^^^^01d43a% 𝐺   \itG    Mathematical Italic Capital G
  ^^^^^^01d43b% 𝐻   \itH    Mathematical Italic Capital H
  ^^^^^^01d43c% 𝐼   \itI    Mathematical Italic Capital I
  ^^^^^^01d43d% 𝐽   \itJ    Mathematical Italic Capital J
  ^^^^^^01d43e% 𝐾   \itK    Mathematical Italic Capital K
  ^^^^^^01d43f% 𝐿   \itL    Mathematical Italic Capital L
  ^^^^^^01d440% 𝑀   \itM    Mathematical Italic Capital M
  ^^^^^^01d441% 𝑁   \itN    Mathematical Italic Capital N
  ^^^^^^01d442% 𝑂   \itO    Mathematical Italic Capital O
  ^^^^^^01d443% 𝑃   \itP    Mathematical Italic Capital P
  ^^^^^^01d444% 𝑄   \itQ    Mathematical Italic Capital Q
  ^^^^^^01d445% 𝑅   \itR    Mathematical Italic Capital R
  ^^^^^^01d446% 𝑆   \itS    Mathematical Italic Capital S
  ^^^^^^01d447% 𝑇   \itT    Mathematical Italic Capital T
  ^^^^^^01d448% 𝑈   \itU    Mathematical Italic Capital U
  ^^^^^^01d449% 𝑉   \itV    Mathematical Italic Capital V
  ^^^^^^01d44a% 𝑊   \itW    Mathematical Italic Capital W
  ^^^^^^01d44b% 𝑋   \itX    Mathematical Italic Capital X
  ^^^^^^01d44c% 𝑌   \itY    Mathematical Italic Capital Y
  ^^^^^^01d44d% 𝑍   \itZ    Mathematical Italic Capital Z
  ^^^^^^01d44e% 𝑎   \ita    Mathematical Italic Small A
  ^^^^^^01d44f% 𝑏   \itb    Mathematical Italic Small B
  ^^^^^^01d450% 𝑐   \itc    Mathematical Italic Small C
  ^^^^^^01d451% 𝑑   \itd    Mathematical Italic Small D
  ^^^^^^01d452% 𝑒   \ite    Mathematical Italic Small E
  ^^^^^^01d453% 𝑓   \itf    Mathematical Italic Small F
  ^^^^^^01d454% 𝑔   \itg    Mathematical Italic Small G
  ^^^^^^01d456% 𝑖   \iti    Mathematical Italic Small I
  ^^^^^^01d457% 𝑗   \itj    Mathematical Italic Small J
  ^^^^^^01d458% 𝑘   \itk    Mathematical Italic Small K
  ^^^^^^01d459% 𝑙   \itl    Mathematical Italic Small L
  ^^^^^^01d45a% 𝑚   \itm    Mathematical Italic Small M
  ^^^^^^01d45b% 𝑛   \itn    Mathematical Italic Small N
  ^^^^^^01d45c% 𝑜   \ito    Mathematical Italic Small O
  ^^^^^^01d45d% 𝑝   \itp    Mathematical Italic Small P
  ^^^^^^01d45e% 𝑞   \itq    Mathematical Italic Small Q
  ^^^^^^01d45f% 𝑟   \itr    Mathematical Italic Small R
  ^^^^^^01d460% 𝑠   \its    Mathematical Italic Small S
  ^^^^^^01d461% 𝑡   \itt    Mathematical Italic Small T
  ^^^^^^01d462% 𝑢   \itu    Mathematical Italic Small U
  ^^^^^^01d463% 𝑣   \itv    Mathematical Italic Small V
  ^^^^^^01d464% 𝑤   \itw    Mathematical Italic Small W
  ^^^^^^01d465% 𝑥   \itx    Mathematical Italic Small X
  ^^^^^^01d466% 𝑦   \ity    Mathematical Italic Small Y
  ^^^^^^01d467% 𝑧   \itz    Mathematical Italic Small Z
  ^^^^^^01d468% 𝑨   \biA    Mathematical Bold Italic Capital A
  ^^^^^^01d469% 𝑩   \biB    Mathematical Bold Italic Capital B
  ^^^^^^01d46a% 𝑪   \biC    Mathematical Bold Italic Capital C
  ^^^^^^01d46b% 𝑫   \biD    Mathematical Bold Italic Capital D
  ^^^^^^01d46c% 𝑬   \biE    Mathematical Bold Italic Capital E
  ^^^^^^01d46d% 𝑭   \biF    Mathematical Bold Italic Capital F
  ^^^^^^01d46e% 𝑮   \biG    Mathematical Bold Italic Capital G
  ^^^^^^01d46f% 𝑯   \biH    Mathematical Bold Italic Capital H
  ^^^^^^01d470% 𝑰   \biI    Mathematical Bold Italic Capital I
  ^^^^^^01d471% 𝑱   \biJ    Mathematical Bold Italic Capital J
  ^^^^^^01d472% 𝑲   \biK    Mathematical Bold Italic Capital K
  ^^^^^^01d473% 𝑳   \biL    Mathematical Bold Italic Capital L
  ^^^^^^01d474% 𝑴   \biM    Mathematical Bold Italic Capital M
  ^^^^^^01d475% 𝑵   \biN    Mathematical Bold Italic Capital N
  ^^^^^^01d476% 𝑶   \biO    Mathematical Bold Italic Capital O
  ^^^^^^01d477% 𝑷   \biP    Mathematical Bold Italic Capital P
  ^^^^^^01d478% 𝑸   \biQ    Mathematical Bold Italic Capital Q
  ^^^^^^01d479% 𝑹   \biR    Mathematical Bold Italic Capital R
  ^^^^^^01d47a% 𝑺   \biS    Mathematical Bold Italic Capital S
  ^^^^^^01d47b% 𝑻   \biT    Mathematical Bold Italic Capital T
  ^^^^^^01d47c% 𝑼   \biU    Mathematical Bold Italic Capital U
  ^^^^^^01d47d% 𝑽   \biV    Mathematical Bold Italic Capital V
  ^^^^^^01d47e% 𝑾   \biW    Mathematical Bold Italic Capital W
  ^^^^^^01d47f% 𝑿   \biX    Mathematical Bold Italic Capital X
  ^^^^^^01d480% 𝒀   \biY    Mathematical Bold Italic Capital Y
  ^^^^^^01d481% 𝒁   \biZ    Mathematical Bold Italic Capital Z
  ^^^^^^01d482% 𝒂   \bia    Mathematical Bold Italic Small A
  ^^^^^^01d483% 𝒃   \bib    Mathematical Bold Italic Small B
  ^^^^^^01d484% 𝒄   \bic    Mathematical Bold Italic Small C
  ^^^^^^01d485% 𝒅   \bid    Mathematical Bold Italic Small D
  ^^^^^^01d486% 𝒆   \bie    Mathematical Bold Italic Small E
  ^^^^^^01d487% 𝒇   \bif    Mathematical Bold Italic Small F
  ^^^^^^01d488% 𝒈   \big    Mathematical Bold Italic Small G
  ^^^^^^01d489% 𝒉   \bih    Mathematical Bold Italic Small H
  ^^^^^^01d48a% 𝒊   \bii    Mathematical Bold Italic Small I
  ^^^^^^01d48b% 𝒋   \bij    Mathematical Bold Italic Small J
  ^^^^^^01d48c% 𝒌   \bik    Mathematical Bold Italic Small K
  ^^^^^^01d48d% 𝒍   \bil    Mathematical Bold Italic Small L
  ^^^^^^01d48e% 𝒎   \bim    Mathematical Bold Italic Small M
  ^^^^^^01d48f% 𝒏   \bin    Mathematical Bold Italic Small N
  ^^^^^^01d490% 𝒐   \bio    Mathematical Bold Italic Small O
  ^^^^^^01d491% 𝒑   \bip    Mathematical Bold Italic Small P
  ^^^^^^01d492% 𝒒   \biq    Mathematical Bold Italic Small Q
  ^^^^^^01d493% 𝒓   \bir    Mathematical Bold Italic Small R
  ^^^^^^01d494% 𝒔   \bis    Mathematical Bold Italic Small S
  ^^^^^^01d495% 𝒕   \bit    Mathematical Bold Italic Small T
  ^^^^^^01d496% 𝒖   \biu    Mathematical Bold Italic Small U
  ^^^^^^01d497% 𝒗   \biv    Mathematical Bold Italic Small V
  ^^^^^^01d498% 𝒘   \biw    Mathematical Bold Italic Small W
  ^^^^^^01d499% 𝒙   \bix    Mathematical Bold Italic Small X
  ^^^^^^01d49a% 𝒚   \biy    Mathematical Bold Italic Small Y
  ^^^^^^01d49b% 𝒛   \biz    Mathematical Bold Italic Small Z
  ^^^^^^01d49c% 𝒜   \scrA   Mathematical Script Capital A
  ^^^^^^01d49e% 𝒞   \scrC   Mathematical Script Capital C
  ^^^^^^01d49f% 𝒟   \scrD   Mathematical Script Capital D
  ^^^^^^01d4a2% 𝒢   \scrG   Mathematical Script Capital G
  ^^^^^^01d4a5% 𝒥   \scrJ   Mathematical Script Capital J
  ^^^^^^01d4a6% 𝒦   \scrK   Mathematical Script Capital K
  ^^^^^^01d4a9% 𝒩   \scrN   Mathematical Script Capital N
  ^^^^^^01d4aa% 𝒪   \scrO   Mathematical Script Capital O
  ^^^^^^01d4ab% 𝒫   \scrP   Mathematical Script Capital P
  ^^^^^^01d4ac% 𝒬   \scrQ   Mathematical Script Capital Q
  ^^^^^^01d4ae% 𝒮   \scrS   Mathematical Script Capital S
  ^^^^^^01d4af% 𝒯   \scrT   Mathematical Script Capital T
  ^^^^^^01d4b0% 𝒰   \scrU   Mathematical Script Capital U
  ^^^^^^01d4b1% 𝒱   \scrV   Mathematical Script Capital V
  ^^^^^^01d4b2% 𝒲   \scrW   Mathematical Script Capital W
  ^^^^^^01d4b3% 𝒳   \scrX   Mathematical Script Capital X
  ^^^^^^01d4b4% 𝒴   \scrY   Mathematical Script Capital Y
  ^^^^^^01d4b5% 𝒵   \scrZ   Mathematical Script Capital Z
  ^^^^^^01d4b6% 𝒶   \scra   Mathematical Script Small A
  ^^^^^^01d4b7% 𝒷   \scrb   Mathematical Script Small B
  ^^^^^^01d4b8% 𝒸   \scrc   Mathematical Script Small C
  ^^^^^^01d4b9% 𝒹   \scrd   Mathematical Script Small D
  ^^^^^^01d4bb% 𝒻   \scrf   Mathematical Script Small F
  ^^^^^^01d4bd% 𝒽   \scrh   Mathematical Script Small H
  ^^^^^^01d4be% 𝒾   \scri   Mathematical Script Small I
  ^^^^^^01d4bf% 𝒿   \scrj   Mathematical Script Small J
  ^^^^^^01d4c0% 𝓀   \scrk   Mathematical Script Small K
  ^^^^^^01d4c1% 𝓁   \scrl   Mathematical Script Small L
  ^^^^^^01d4c2% 𝓂   \scrm   Mathematical Script Small M
  ^^^^^^01d4c3% 𝓃   \scrn   Mathematical Script Small N
  ^^^^^^01d4c5% 𝓅   \scrp   Mathematical Script Small P
  ^^^^^^01d4c6% 𝓆   \scrq   Mathematical Script Small Q
  ^^^^^^01d4c7% 𝓇   \scrr   Mathematical Script Small R
  ^^^^^^01d4c8% 𝓈   \scrs   Mathematical Script Small S
  ^^^^^^01d4c9% 𝓉   \scrt   Mathematical Script Small T
  ^^^^^^01d4ca% 𝓊   \scru   Mathematical Script Small U
  ^^^^^^01d4cb% 𝓋   \scrv   Mathematical Script Small V
  ^^^^^^01d4cc% 𝓌   \scrw   Mathematical Script Small W
  ^^^^^^01d4cd% 𝓍   \scrx   Mathematical Script Small X
  ^^^^^^01d4ce% 𝓎   \scry   Mathematical Script Small Y
  ^^^^^^01d4cf% 𝓏   \scrz   Mathematical Script Small Z
  ^^^^^^01d4d0% 𝓐   \bscrA  Mathematical Bold Script Capital A
  ^^^^^^01d4d1% 𝓑   \bscrB  Mathematical Bold Script Capital B
  ^^^^^^01d4d2% 𝓒   \bscrC  Mathematical Bold Script Capital C
  ^^^^^^01d4d3% 𝓓   \bscrD  Mathematical Bold Script Capital D
  ^^^^^^01d4d4% 𝓔   \bscrE  Mathematical Bold Script Capital E
  ^^^^^^01d4d5% 𝓕   \bscrF  Mathematical Bold Script Capital F
  ^^^^^^01d4d6% 𝓖   \bscrG  Mathematical Bold Script Capital G
  ^^^^^^01d4d7% 𝓗   \bscrH  Mathematical Bold Script Capital H
  ^^^^^^01d4d8% 𝓘   \bscrI  Mathematical Bold Script Capital I
  ^^^^^^01d4d9% 𝓙   \bscrJ  Mathematical Bold Script Capital J
  ^^^^^^01d4da% 𝓚   \bscrK  Mathematical Bold Script Capital K
  ^^^^^^01d4db% 𝓛   \bscrL  Mathematical Bold Script Capital L
  ^^^^^^01d4dc% 𝓜   \bscrM  Mathematical Bold Script Capital M
  ^^^^^^01d4dd% 𝓝   \bscrN  Mathematical Bold Script Capital N
  ^^^^^^01d4de% 𝓞   \bscrO  Mathematical Bold Script Capital O
  ^^^^^^01d4df% 𝓟   \bscrP  Mathematical Bold Script Capital P
  ^^^^^^01d4e0% 𝓠   \bscrQ  Mathematical Bold Script Capital Q
  ^^^^^^01d4e1% 𝓡   \bscrR  Mathematical Bold Script Capital R
  ^^^^^^01d4e2% 𝓢   \bscrS  Mathematical Bold Script Capital S
  ^^^^^^01d4e3% 𝓣   \bscrT  Mathematical Bold Script Capital T
  ^^^^^^01d4e4% 𝓤   \bscrU  Mathematical Bold Script Capital U
  ^^^^^^01d4e5% 𝓥   \bscrV  Mathematical Bold Script Capital V
  ^^^^^^01d4e6% 𝓦   \bscrW  Mathematical Bold Script Capital W
  ^^^^^^01d4e7% 𝓧   \bscrX  Mathematical Bold Script Capital X
  ^^^^^^01d4e8% 𝓨   \bscrY  Mathematical Bold Script Capital Y
  ^^^^^^01d4e9% 𝓩   \bscrZ  Mathematical Bold Script Capital Z
  ^^^^^^01d4ea% 𝓪   \bscra  Mathematical Bold Script Small A
  ^^^^^^01d4eb% 𝓫   \bscrb  Mathematical Bold Script Small B
  ^^^^^^01d4ec% 𝓬   \bscrc  Mathematical Bold Script Small C
  ^^^^^^01d4ed% 𝓭   \bscrd  Mathematical Bold Script Small D
  ^^^^^^01d4ee% 𝓮   \bscre  Mathematical Bold Script Small E
  ^^^^^^01d4ef% 𝓯   \bscrf  Mathematical Bold Script Small F
  ^^^^^^01d4f0% 𝓰   \bscrg  Mathematical Bold Script Small G
  ^^^^^^01d4f1% 𝓱   \bscrh  Mathematical Bold Script Small H
  ^^^^^^01d4f2% 𝓲   \bscri  Mathematical Bold Script Small I
  ^^^^^^01d4f3% 𝓳   \bscrj  Mathematical Bold Script Small J
  ^^^^^^01d4f4% 𝓴   \bscrk  Mathematical Bold Script Small K
  ^^^^^^01d4f5% 𝓵   \bscrl  Mathematical Bold Script Small L
  ^^^^^^01d4f6% 𝓶   \bscrm  Mathematical Bold Script Small M
  ^^^^^^01d4f7% 𝓷   \bscrn  Mathematical Bold Script Small N
  ^^^^^^01d4f8% 𝓸   \bscro  Mathematical Bold Script Small O
  ^^^^^^01d4f9% 𝓹   \bscrp  Mathematical Bold Script Small P
  ^^^^^^01d4fa% 𝓺   \bscrq  Mathematical Bold Script Small Q
  ^^^^^^01d4fb% 𝓻   \bscrr  Mathematical Bold Script Small R
  ^^^^^^01d4fc% 𝓼   \bscrs  Mathematical Bold Script Small S
  ^^^^^^01d4fd% 𝓽   \bscrt  Mathematical Bold Script Small T
  ^^^^^^01d4fe% 𝓾   \bscru  Mathematical Bold Script Small U
  ^^^^^^01d4ff% 𝓿   \bscrv  Mathematical Bold Script Small V
  ^^^^^^01d500% 𝔀   \bscrw  Mathematical Bold Script Small W
  ^^^^^^01d501% 𝔁   \bscrx  Mathematical Bold Script Small X
  ^^^^^^01d502% 𝔂   \bscry  Mathematical Bold Script Small Y
  ^^^^^^01d503% 𝔃   \bscrz  Mathematical Bold Script Small Z
  ^^^^^^01d504% 𝔄   \frakA  Mathematical Fraktur Capital A
  ^^^^^^01d505% 𝔅   \frakB  Mathematical Fraktur Capital B
  ^^^^^^01d507% 𝔇   \frakD  Mathematical Fraktur Capital D
  ^^^^^^01d508% 𝔈   \frakE  Mathematical Fraktur Capital E
  ^^^^^^01d509% 𝔉   \frakF  Mathematical Fraktur Capital F
  ^^^^^^01d50a% 𝔊   \frakG  Mathematical Fraktur Capital G
  ^^^^^^01d50d% 𝔍   \frakJ  Mathematical Fraktur Capital J
  ^^^^^^01d50e% 𝔎   \frakK  Mathematical Fraktur Capital K
  ^^^^^^01d50f% 𝔏   \frakL  Mathematical Fraktur Capital L
  ^^^^^^01d510% 𝔐   \frakM  Mathematical Fraktur Capital M
  ^^^^^^01d511% 𝔑   \frakN  Mathematical Fraktur Capital N
  ^^^^^^01d512% 𝔒   \frakO  Mathematical Fraktur Capital O
  ^^^^^^01d513% 𝔓   \frakP  Mathematical Fraktur Capital P
  ^^^^^^01d514% 𝔔   \frakQ  Mathematical Fraktur Capital Q
  ^^^^^^01d516% 𝔖   \frakS  Mathematical Fraktur Capital S
  ^^^^^^01d517% 𝔗   \frakT  Mathematical Fraktur Capital T
  ^^^^^^01d518% 𝔘   \frakU  Mathematical Fraktur Capital U
  ^^^^^^01d519% 𝔙   \frakV  Mathematical Fraktur Capital V
  ^^^^^^01d51a% 𝔚   \frakW  Mathematical Fraktur Capital W
  ^^^^^^01d51b% 𝔛   \frakX  Mathematical Fraktur Capital X
  ^^^^^^01d51c% 𝔜   \frakY  Mathematical Fraktur Capital Y
  ^^^^^^01d51e% 𝔞   \fraka  Mathematical Fraktur Small A
  ^^^^^^01d51f% 𝔟   \frakb  Mathematical Fraktur Small B
  ^^^^^^01d520% 𝔠   \frakc  Mathematical Fraktur Small C
  ^^^^^^01d521% 𝔡   \frakd  Mathematical Fraktur Small D
  ^^^^^^01d522% 𝔢   \frake  Mathematical Fraktur Small E
  ^^^^^^01d523% 𝔣   \frakf  Mathematical Fraktur Small F
  ^^^^^^01d524% 𝔤   \frakg  Mathematical Fraktur Small G
  ^^^^^^01d525% 𝔥   \frakh  Mathematical Fraktur Small H
  ^^^^^^01d526% 𝔦   \fraki  Mathematical Fraktur Small I
  ^^^^^^01d527% 𝔧   \frakj  Mathematical Fraktur Small J
  ^^^^^^01d528% 𝔨   \frakk  Mathematical Fraktur Small K
  ^^^^^^01d529% 𝔩   \frakl  Mathematical Fraktur Small L
  ^^^^^^01d52a% 𝔪   \frakm  Mathematical Fraktur Small M
  ^^^^^^01d52b% 𝔫   \frakn  Mathematical Fraktur Small N
  ^^^^^^01d52c% 𝔬   \frako  Mathematical Fraktur Small O
  ^^^^^^01d52d% 𝔭   \frakp  Mathematical Fraktur Small P
  ^^^^^^01d52e% 𝔮   \frakq  Mathematical Fraktur Small Q
  ^^^^^^01d52f% 𝔯   \frakr  Mathematical Fraktur Small R
  ^^^^^^01d530% 𝔰   \fraks  Mathematical Fraktur Small S
  ^^^^^^01d531% 𝔱   \frakt  Mathematical Fraktur Small T
  ^^^^^^01d532% 𝔲   \fraku  Mathematical Fraktur Small U
  ^^^^^^01d533% 𝔳   \frakv  Mathematical Fraktur Small V
  ^^^^^^01d534% 𝔴   \frakw  Mathematical Fraktur Small W
  ^^^^^^01d535% 𝔵   \frakx  Mathematical Fraktur Small X
  ^^^^^^01d536% 𝔶   \fraky  Mathematical Fraktur Small Y
  ^^^^^^01d537% 𝔷   \frakz  Mathematical Fraktur Small Z
  ^^^^^^01d538% 𝔸   \bbA    Mathematical Double-Struck Capital A
  ^^^^^^01d539% 𝔹   \bbB    Mathematical Double-Struck Capital B
  ^^^^^^01d53b% 𝔻   \bbD    Mathematical Double-Struck Capital D
  ^^^^^^01d53c% 𝔼   \bbE    Mathematical Double-Struck Capital E
  ^^^^^^01d53d% 𝔽   \bbF    Mathematical Double-Struck Capital F
  ^^^^^^01d53e% 𝔾   \bbG    Mathematical Double-Struck Capital G
  ^^^^^^01d540% 𝕀   \bbI    Mathematical Double-Struck Capital I
  ^^^^^^01d541% 𝕁   \bbJ    Mathematical Double-Struck Capital J
  ^^^^^^01d542% 𝕂   \bbK    Mathematical Double-Struck Capital K
  ^^^^^^01d543% 𝕃   \bbL    Mathematical Double-Struck Capital L
  ^^^^^^01d544% 𝕄   \bbM    Mathematical Double-Struck Capital M
  ^^^^^^01d546% 𝕆   \bbO    Mathematical Double-Struck Capital O
  ^^^^^^01d54a% 𝕊   \bbS    Mathematical Double-Struck Capital S
  ^^^^^^01d54b% 𝕋   \bbT    Mathematical Double-Struck Capital T
  ^^^^^^01d54c% 𝕌   \bbU    Mathematical Double-Struck Capital U
  ^^^^^^01d54d% 𝕍   \bbV    Mathematical Double-Struck Capital V
  ^^^^^^01d54e% 𝕎   \bbW    Mathematical Double-Struck Capital W
  ^^^^^^01d54f% 𝕏   \bbX    Mathematical Double-Struck Capital X
  ^^^^^^01d550% 𝕐   \bbY    Mathematical Double-Struck Capital Y
  ^^^^^^01d552% 𝕒   \bba    Mathematical Double-Struck Small A
  ^^^^^^01d553% 𝕓   \bbb    Mathematical Double-Struck Small B
  ^^^^^^01d554% 𝕔   \bbc    Mathematical Double-Struck Small C
  ^^^^^^01d555% 𝕕   \bbd    Mathematical Double-Struck Small D
  ^^^^^^01d556% 𝕖   \bbe    Mathematical Double-Struck Small E
  ^^^^^^01d557% 𝕗   \bbf    Mathematical Double-Struck Small F
  ^^^^^^01d558% 𝕘   \bbg    Mathematical Double-Struck Small G
  ^^^^^^01d559% 𝕙   \bbh    Mathematical Double-Struck Small H
  ^^^^^^01d55a% 𝕚   \bbi    Mathematical Double-Struck Small I
  ^^^^^^01d55b% 𝕛   \bbj    Mathematical Double-Struck Small J
  ^^^^^^01d55c% 𝕜   \bbk    Mathematical Double-Struck Small K
  ^^^^^^01d55d% 𝕝   \bbl    Mathematical Double-Struck Small L
  ^^^^^^01d55e% 𝕞   \bbm    Mathematical Double-Struck Small M
  ^^^^^^01d55f% 𝕟   \bbn    Mathematical Double-Struck Small N
  ^^^^^^01d560% 𝕠   \bbo    Mathematical Double-Struck Small O
  ^^^^^^01d561% 𝕡   \bbp    Mathematical Double-Struck Small P
  ^^^^^^01d562% 𝕢   \bbq    Mathematical Double-Struck Small Q
  ^^^^^^01d563% 𝕣   \bbr    Mathematical Double-Struck Small R
  ^^^^^^01d564% 𝕤   \bbs    Mathematical Double-Struck Small S
  ^^^^^^01d565% 𝕥   \bbt    Mathematical Double-Struck Small T
  ^^^^^^01d566% 𝕦   \bbu    Mathematical Double-Struck Small U
  ^^^^^^01d567% 𝕧   \bbv    Mathematical Double-Struck Small V
  ^^^^^^01d568% 𝕨   \bbw    Mathematical Double-Struck Small W
  ^^^^^^01d569% 𝕩   \bbx    Mathematical Double-Struck Small X
  ^^^^^^01d56a% 𝕪   \bby    Mathematical Double-Struck Small Y
  ^^^^^^01d56b% 𝕫   \bbz    Mathematical Double-Struck Small Z
  ^^^^^^01d56c% 𝕬   \bfrakA Mathematical Bold Fraktur Capital A
  ^^^^^^01d56d% 𝕭   \bfrakB Mathematical Bold Fraktur Capital B
  ^^^^^^01d56e% 𝕮   \bfrakC Mathematical Bold Fraktur Capital C
  ^^^^^^01d56f% 𝕯   \bfrakD Mathematical Bold Fraktur Capital D
  ^^^^^^01d570% 𝕰   \bfrakE Mathematical Bold Fraktur Capital E
  ^^^^^^01d571% 𝕱   \bfrakF Mathematical Bold Fraktur Capital F
  ^^^^^^01d572% 𝕲   \bfrakG Mathematical Bold Fraktur Capital G
  ^^^^^^01d573% 𝕳   \bfrakH Mathematical Bold Fraktur Capital H
  ^^^^^^01d574% 𝕴   \bfrakI Mathematical Bold Fraktur Capital I
  ^^^^^^01d575% 𝕵   \bfrakJ Mathematical Bold Fraktur Capital J
  ^^^^^^01d576% 𝕶   \bfrakK Mathematical Bold Fraktur Capital K
  ^^^^^^01d577% 𝕷   \bfrakL Mathematical Bold Fraktur Capital L
  ^^^^^^01d578% 𝕸   \bfrakM Mathematical Bold Fraktur Capital M
  ^^^^^^01d579% 𝕹   \bfrakN Mathematical Bold Fraktur Capital N
  ^^^^^^01d57a% 𝕺   \bfrakO Mathematical Bold Fraktur Capital O
  ^^^^^^01d57b% 𝕻   \bfrakP Mathematical Bold Fraktur Capital P
  ^^^^^^01d57c% 𝕼   \bfrakQ Mathematical Bold Fraktur Capital Q
  ^^^^^^01d57d% 𝕽   \bfrakR Mathematical Bold Fraktur Capital R
  ^^^^^^01d57e% 𝕾   \bfrakS Mathematical Bold Fraktur Capital S
  ^^^^^^01d57f% 𝕿   \bfrakT Mathematical Bold Fraktur Capital T
  ^^^^^^01d580% 𝖀   \bfrakU Mathematical Bold Fraktur Capital U
  ^^^^^^01d581% 𝖁   \bfrakV Mathematical Bold Fraktur Capital V
  ^^^^^^01d582% 𝖂   \bfrakW Mathematical Bold Fraktur Capital W
  ^^^^^^01d583% 𝖃   \bfrakX Mathematical Bold Fraktur Capital X
  ^^^^^^01d584% 𝖄   \bfrakY Mathematical Bold Fraktur Capital Y
  ^^^^^^01d585% 𝖅   \bfrakZ Mathematical Bold Fraktur Capital Z
  ^^^^^^01d586% 𝖆   \bfraka Mathematical Bold Fraktur Small A
  ^^^^^^01d587% 𝖇   \bfrakb Mathematical Bold Fraktur Small B
  ^^^^^^01d588% 𝖈   \bfrakc Mathematical Bold Fraktur Small C
  ^^^^^^01d589% 𝖉   \bfrakd Mathematical Bold Fraktur Small D
  ^^^^^^01d58a% 𝖊   \bfrake Mathematical Bold Fraktur Small E
  ^^^^^^01d58b% 𝖋   \bfrakf Mathematical Bold Fraktur Small F
  ^^^^^^01d58c% 𝖌   \bfrakg Mathematical Bold Fraktur Small G
  ^^^^^^01d58d% 𝖍   \bfrakh Mathematical Bold Fraktur Small H
  ^^^^^^01d58e% 𝖎   \bfraki Mathematical Bold Fraktur Small I
  ^^^^^^01d58f% 𝖏   \bfrakj Mathematical Bold Fraktur Small J
  ^^^^^^01d590% 𝖐   \bfrakk Mathematical Bold Fraktur Small K
  ^^^^^^01d591% 𝖑   \bfrakl Mathematical Bold Fraktur Small L
  ^^^^^^01d592% 𝖒   \bfrakm Mathematical Bold Fraktur Small M
  ^^^^^^01d593% 𝖓   \bfrakn Mathematical Bold Fraktur Small N
  ^^^^^^01d594% 𝖔   \bfrako Mathematical Bold Fraktur Small O
  ^^^^^^01d595% 𝖕   \bfrakp Mathematical Bold Fraktur Small P
  ^^^^^^01d596% 𝖖   \bfrakq Mathematical Bold Fraktur Small Q
  ^^^^^^01d597% 𝖗   \bfrakr Mathematical Bold Fraktur Small R
  ^^^^^^01d598% 𝖘   \bfraks Mathematical Bold Fraktur Small S
  ^^^^^^01d599% 𝖙   \bfrakt Mathematical Bold Fraktur Small T
  ^^^^^^01d59a% 𝖚   \bfraku Mathematical Bold Fraktur Small U
  ^^^^^^01d59b% 𝖛   \bfrakv Mathematical Bold Fraktur Small V
  ^^^^^^01d59c% 𝖜   \bfrakw Mathematical Bold Fraktur Small W
  ^^^^^^01d59d% 𝖝   \bfrakx Mathematical Bold Fraktur Small X
  ^^^^^^01d59e% 𝖞   \bfraky Mathematical Bold Fraktur Small Y
  ^^^^^^01d59f% 𝖟   \bfrakz Mathematical Bold Fraktur Small Z
  ^^^^^^01d5a0% 𝖠   \sansA  Mathematical Sans-Serif Capital A
  ^^^^^^01d5a1% 𝖡   \sansB  Mathematical Sans-Serif Capital B
  ^^^^^^01d5a2% 𝖢   \sansC  Mathematical Sans-Serif Capital C
  ^^^^^^01d5a3% 𝖣   \sansD  Mathematical Sans-Serif Capital D
  ^^^^^^01d5a4% 𝖤   \sansE  Mathematical Sans-Serif Capital E
  ^^^^^^01d5a5% 𝖥   \sansF  Mathematical Sans-Serif Capital F
  ^^^^^^01d5a6% 𝖦   \sansG  Mathematical Sans-Serif Capital G
  ^^^^^^01d5a7% 𝖧   \sansH  Mathematical Sans-Serif Capital H
  ^^^^^^01d5a8% 𝖨   \sansI  Mathematical Sans-Serif Capital I
  ^^^^^^01d5a9% 𝖩   \sansJ  Mathematical Sans-Serif Capital J
  ^^^^^^01d5aa% 𝖪   \sansK  Mathematical Sans-Serif Capital K
  ^^^^^^01d5ab% 𝖫   \sansL  Mathematical Sans-Serif Capital L
  ^^^^^^01d5ac% 𝖬   \sansM  Mathematical Sans-Serif Capital M
  ^^^^^^01d5ad% 𝖭   \sansN  Mathematical Sans-Serif Capital N
  ^^^^^^01d5ae% 𝖮   \sansO  Mathematical Sans-Serif Capital O
  ^^^^^^01d5af% 𝖯   \sansP  Mathematical Sans-Serif Capital P
  ^^^^^^01d5b0% 𝖰   \sansQ  Mathematical Sans-Serif Capital Q
  ^^^^^^01d5b1% 𝖱   \sansR  Mathematical Sans-Serif Capital R
  ^^^^^^01d5b2% 𝖲   \sansS  Mathematical Sans-Serif Capital S
  ^^^^^^01d5b3% 𝖳   \sansT  Mathematical Sans-Serif Capital T
  ^^^^^^01d5b4% 𝖴   \sansU  Mathematical Sans-Serif Capital U
  ^^^^^^01d5b5% 𝖵   \sansV  Mathematical Sans-Serif Capital V
  ^^^^^^01d5b6% 𝖶   \sansW  Mathematical Sans-Serif Capital W
  ^^^^^^01d5b7% 𝖷   \sansX  Mathematical Sans-Serif Capital X
  ^^^^^^01d5b8% 𝖸   \sansY  Mathematical Sans-Serif Capital Y
  ^^^^^^01d5b9% 𝖹   \sansZ  Mathematical Sans-Serif Capital Z
  ^^^^^^01d5ba% 𝖺   \sansa  Mathematical Sans-Serif Small A
  ^^^^^^01d5bb% 𝖻   \sansb  Mathematical Sans-Serif Small B
  ^^^^^^01d5bc% 𝖼   \sansc  Mathematical Sans-Serif Small C
  ^^^^^^01d5bd% 𝖽   \sansd  Mathematical Sans-Serif Small D
  ^^^^^^01d5be% 𝖾   \sanse  Mathematical Sans-Serif Small E
  ^^^^^^01d5bf% 𝖿   \sansf  Mathematical Sans-Serif Small F
  ^^^^^^01d5c0% 𝗀   \sansg  Mathematical Sans-Serif Small G
  ^^^^^^01d5c1% 𝗁   \sansh  Mathematical Sans-Serif Small H
  ^^^^^^01d5c2% 𝗂   \sansi  Mathematical Sans-Serif Small I
  ^^^^^^01d5c3% 𝗃   \sansj  Mathematical Sans-Serif Small J
  ^^^^^^01d5c4% 𝗄   \sansk  Mathematical Sans-Serif Small K
  ^^^^^^01d5c5% 𝗅   \sansl  Mathematical Sans-Serif Small L
  ^^^^^^01d5c6% 𝗆   \sansm  Mathematical Sans-Serif Small M
  ^^^^^^01d5c7% 𝗇   \sansn  Mathematical Sans-Serif Small N
  ^^^^^^01d5c8% 𝗈   \sanso  Mathematical Sans-Serif Small O
  ^^^^^^01d5c9% 𝗉   \sansp  Mathematical Sans-Serif Small P
  ^^^^^^01d5ca% 𝗊   \sansq  Mathematical Sans-Serif Small Q
  ^^^^^^01d5cb% 𝗋   \sansr  Mathematical Sans-Serif Small R
  ^^^^^^01d5cc% 𝗌   \sanss  Mathematical Sans-Serif Small S
  ^^^^^^01d5cd% 𝗍   \sanst  Mathematical Sans-Serif Small T
  ^^^^^^01d5ce% 𝗎   \sansu  Mathematical Sans-Serif Small U
  ^^^^^^01d5cf% 𝗏   \sansv  Mathematical Sans-Serif Small V
  ^^^^^^01d5d0% 𝗐   \sansw  Mathematical Sans-Serif Small W
  ^^^^^^01d5d1% 𝗑   \sansx  Mathematical Sans-Serif Small X
  ^^^^^^01d5d2% 𝗒   \sansy  Mathematical Sans-Serif Small Y
  ^^^^^^01d5d3% 𝗓   \sansz  Mathematical Sans-Serif Small Z
  ^^^^^^01d5d4% 𝗔   \bsansA Mathematical Sans-Serif Bold Capital A
  ^^^^^^01d5d5% 𝗕   \bsansB Mathematical Sans-Serif Bold Capital B
  ^^^^^^01d5d6% 𝗖   \bsansC Mathematical Sans-Serif Bold Capital C
  ^^^^^^01d5d7% 𝗗   \bsansD Mathematical Sans-Serif Bold Capital D
  ^^^^^^01d5d8% 𝗘   \bsansE Mathematical Sans-Serif Bold Capital E
  ^^^^^^01d5d9% 𝗙   \bsansF Mathematical Sans-Serif Bold Capital F
  ^^^^^^01d5da% 𝗚   \bsansG Mathematical Sans-Serif Bold Capital G
  ^^^^^^01d5db% 𝗛   \bsansH Mathematical Sans-Serif Bold Capital H
  ^^^^^^01d5dc% 𝗜   \bsansI Mathematical Sans-Serif Bold Capital I
  ^^^^^^01d5dd% 𝗝   \bsansJ Mathematical Sans-Serif Bold Capital J
  ^^^^^^01d5de% 𝗞   \bsansK Mathematical Sans-Serif Bold Capital K
  ^^^^^^01d5df% 𝗟   \bsansL Mathematical Sans-Serif Bold Capital L
  ^^^^^^01d5e0% 𝗠   \bsansM Mathematical Sans-Serif Bold Capital M
  ^^^^^^01d5e1% 𝗡   \bsansN Mathematical Sans-Serif Bold Capital N
  ^^^^^^01d5e2% 𝗢   \bsansO Mathematical Sans-Serif Bold Capital O
  ^^^^^^01d5e3% 𝗣   \bsansP Mathematical Sans-Serif Bold Capital P
  ^^^^^^01d5e4% 𝗤   \bsansQ Mathematical Sans-Serif Bold Capital Q
  ^^^^^^01d5e5% 𝗥   \bsansR Mathematical Sans-Serif Bold Capital R
  ^^^^^^01d5e6% 𝗦   \bsansS Mathematical Sans-Serif Bold Capital S
  ^^^^^^01d5e7% 𝗧   \bsansT Mathematical Sans-Serif Bold Capital T
  ^^^^^^01d5e8% 𝗨   \bsansU Mathematical Sans-Serif Bold Capital U
  ^^^^^^01d5e9% 𝗩   \bsansV Mathematical Sans-Serif Bold Capital V
  ^^^^^^01d5ea% 𝗪   \bsansW Mathematical Sans-Serif Bold Capital W
  ^^^^^^01d5eb% 𝗫   \bsansX Mathematical Sans-Serif Bold Capital X
  ^^^^^^01d5ec% 𝗬   \bsansY Mathematical Sans-Serif Bold Capital Y
  ^^^^^^01d5ed% 𝗭   \bsansZ Mathematical Sans-Serif Bold Capital Z
  ^^^^^^01d5ee% 𝗮   \bsansa Mathematical Sans-Serif Bold Small A
  ^^^^^^01d5ef% 𝗯   \bsansb Mathematical Sans-Serif Bold Small B
  ^^^^^^01d5f0% 𝗰   \bsansc Mathematical Sans-Serif Bold Small C
  ^^^^^^01d5f1% 𝗱   \bsansd Mathematical Sans-Serif Bold Small D
  ^^^^^^01d5f2% 𝗲   \bsanse Mathematical Sans-Serif Bold Small E
  ^^^^^^01d5f3% 𝗳   \bsansf Mathematical Sans-Serif Bold Small F
  ^^^^^^01d5f4% 𝗴   \bsansg Mathematical Sans-Serif Bold Small G
  ^^^^^^01d5f5% 𝗵   \bsansh Mathematical Sans-Serif Bold Small H
  ^^^^^^01d5f6% 𝗶   \bsansi Mathematical Sans-Serif Bold Small I
  ^^^^^^01d5f7% 𝗷   \bsansj Mathematical Sans-Serif Bold Small J
  ^^^^^^01d5f8% 𝗸   \bsansk Mathematical Sans-Serif Bold Small K
  ^^^^^^01d5f9% 𝗹   \bsansl Mathematical Sans-Serif Bold Small L
  ^^^^^^01d5fa% 𝗺   \bsansm Mathematical Sans-Serif Bold Small M
  ^^^^^^01d5fb% 𝗻   \bsansn Mathematical Sans-Serif Bold Small N
  ^^^^^^01d5fc% 𝗼   \bsanso Mathematical Sans-Serif Bold Small O
  ^^^^^^01d5fd% 𝗽   \bsansp Mathematical Sans-Serif Bold Small P
  ^^^^^^01d5fe% 𝗾   \bsansq Mathematical Sans-Serif Bold Small Q
  ^^^^^^01d5ff% 𝗿   \bsansr Mathematical Sans-Serif Bold Small R
  ^^^^^^01d600% 𝘀   \bsanss Mathematical Sans-Serif Bold Small S
  ^^^^^^01d601% 𝘁   \bsanst Mathematical Sans-Serif Bold Small T
  ^^^^^^01d602% 𝘂   \bsansu Mathematical Sans-Serif Bold Small U
  ^^^^^^01d603% 𝘃   \bsansv Mathematical Sans-Serif Bold Small V
  ^^^^^^01d604% 𝘄   \bsansw Mathematical Sans-Serif Bold Small W
  ^^^^^^01d605% 𝘅   \bsansx Mathematical Sans-Serif Bold Small X
  ^^^^^^01d606% 𝘆   \bsansy Mathematical Sans-Serif Bold Small Y
  ^^^^^^01d607% 𝘇   \bsansz Mathematical Sans-Serif Bold Small Z
  ^^^^^^01d608% 𝘈   \isansA Mathematical Sans-Serif Italic Capital A
  ^^^^^^01d609% 𝘉   \isansB Mathematical Sans-Serif Italic Capital B
  ^^^^^^01d60a% 𝘊   \isansC Mathematical Sans-Serif Italic Capital C
  ^^^^^^01d60b% 𝘋   \isansD Mathematical Sans-Serif Italic Capital D
  ^^^^^^01d60c% 𝘌   \isansE Mathematical Sans-Serif Italic Capital E
  ^^^^^^01d60d% 𝘍   \isansF Mathematical Sans-Serif Italic Capital F
  ^^^^^^01d60e% 𝘎   \isansG Mathematical Sans-Serif Italic Capital G
  ^^^^^^01d60f% 𝘏   \isansH Mathematical Sans-Serif Italic Capital H
  ^^^^^^01d610% 𝘐   \isansI Mathematical Sans-Serif Italic Capital I
  ^^^^^^01d611% 𝘑   \isansJ Mathematical Sans-Serif Italic Capital J
  ^^^^^^01d612% 𝘒   \isansK Mathematical Sans-Serif Italic Capital K
  ^^^^^^01d613% 𝘓   \isansL Mathematical Sans-Serif Italic Capital L
  ^^^^^^01d614% 𝘔   \isansM Mathematical Sans-Serif Italic Capital M
  ^^^^^^01d615% 𝘕   \isansN Mathematical Sans-Serif Italic Capital N
  ^^^^^^01d616% 𝘖   \isansO Mathematical Sans-Serif Italic Capital O
  ^^^^^^01d617% 𝘗   \isansP Mathematical Sans-Serif Italic Capital P
  ^^^^^^01d618% 𝘘   \isansQ Mathematical Sans-Serif Italic Capital Q
  ^^^^^^01d619% 𝘙   \isansR Mathematical Sans-Serif Italic Capital R
  ^^^^^^01d61a% 𝘚   \isansS Mathematical Sans-Serif Italic Capital S
  ^^^^^^01d61b% 𝘛   \isansT Mathematical Sans-Serif Italic Capital T
  ^^^^^^01d61c% 𝘜   \isansU Mathematical Sans-Serif Italic Capital U
  ^^^^^^01d61d% 𝘝   \isansV Mathematical Sans-Serif Italic Capital V
  ^^^^^^01d61e% 𝘞   \isansW Mathematical Sans-Serif Italic Capital W
  ^^^^^^01d61f% 𝘟   \isansX Mathematical Sans-Serif Italic Capital X
  ^^^^^^01d620% 𝘠   \isansY Mathematical Sans-Serif Italic Capital Y
  ^^^^^^01d621% 𝘡   \isansZ Mathematical Sans-Serif Italic Capital Z
  ^^^^^^01d622% 𝘢   \isansa Mathematical Sans-Serif Italic Small A
  ^^^^^^01d623% 𝘣   \isansb Mathematical Sans-Serif Italic Small B
  ^^^^^^01d624% 𝘤   \isansc Mathematical Sans-Serif Italic Small C
  ^^^^^^01d625% 𝘥   \isansd Mathematical Sans-Serif Italic Small D
  ^^^^^^01d626% 𝘦   \isanse Mathematical Sans-Serif Italic Small E
  ^^^^^^01d627% 𝘧   \isansf Mathematical Sans-Serif Italic Small F
  ^^^^^^01d628% 𝘨   \isansg Mathematical Sans-Serif Italic Small G
  ^^^^^^01d629% 𝘩   \isansh Mathematical Sans-Serif Italic Small H
  ^^^^^^01d62a% 𝘪   \isansi Mathematical Sans-Serif Italic Small I
  ^^^^^^01d62b% 𝘫   \isansj Mathematical Sans-Serif Italic Small J
  ^^^^^^01d62c% 𝘬   \isansk Mathematical Sans-Serif Italic Small K
  ^^^^^^01d62d% 𝘭   \isansl Mathematical Sans-Serif Italic Small L
  ^^^^^^01d62e% 𝘮   \isansm Mathematical Sans-Serif Italic Small M
  ^^^^^^01d62f% 𝘯   \isansn Mathematical Sans-Serif Italic Small N
  ^^^^^^01d630% 𝘰   \isanso Mathematical Sans-Serif Italic Small O
  ^^^^^^01d631% 𝘱   \isansp Mathematical Sans-Serif Italic Small P
  ^^^^^^01d632% 𝘲   \isansq Mathematical Sans-Serif Italic Small Q
  ^^^^^^01d633% 𝘳   \isansr Mathematical Sans-Serif Italic Small R
  ^^^^^^01d634% 𝘴   \isanss Mathematical Sans-Serif Italic Small S
  ^^^^^^01d635% 𝘵   \isanst Mathematical Sans-Serif Italic Small T
  ^^^^^^01d636% 𝘶   \isansu Mathematical Sans-Serif Italic Small U
  ^^^^^^01d637% 𝘷   \isansv Mathematical Sans-Serif Italic Small V
  ^^^^^^01d638% 𝘸   \isansw Mathematical Sans-Serif Italic Small W
  ^^^^^^01d639% 𝘹   \isansx Mathematical Sans-Serif Italic Small X
  ^^^^^^01d63a% 𝘺   \isansy Mathematical Sans-Serif Italic Small Y
  ^^^^^^01d63b% 𝘻   \isansz Mathematical Sans-Serif Italic Small Z
  ^^^^^^01d63c% 𝘼   \bisansA    Mathematical Sans-Serif Bold Italic Capital A
  ^^^^^^01d63d% 𝘽   \bisansB    Mathematical Sans-Serif Bold Italic Capital B
  ^^^^^^01d63e% 𝘾   \bisansC    Mathematical Sans-Serif Bold Italic Capital C
  ^^^^^^01d63f% 𝘿   \bisansD    Mathematical Sans-Serif Bold Italic Capital D
  ^^^^^^01d640% 𝙀   \bisansE    Mathematical Sans-Serif Bold Italic Capital E
  ^^^^^^01d641% 𝙁   \bisansF    Mathematical Sans-Serif Bold Italic Capital F
  ^^^^^^01d642% 𝙂   \bisansG    Mathematical Sans-Serif Bold Italic Capital G
  ^^^^^^01d643% 𝙃   \bisansH    Mathematical Sans-Serif Bold Italic Capital H
  ^^^^^^01d644% 𝙄   \bisansI    Mathematical Sans-Serif Bold Italic Capital I
  ^^^^^^01d645% 𝙅   \bisansJ    Mathematical Sans-Serif Bold Italic Capital J
  ^^^^^^01d646% 𝙆   \bisansK    Mathematical Sans-Serif Bold Italic Capital K
  ^^^^^^01d647% 𝙇   \bisansL    Mathematical Sans-Serif Bold Italic Capital L
  ^^^^^^01d648% 𝙈   \bisansM    Mathematical Sans-Serif Bold Italic Capital M
  ^^^^^^01d649% 𝙉   \bisansN    Mathematical Sans-Serif Bold Italic Capital N
  ^^^^^^01d64a% 𝙊   \bisansO    Mathematical Sans-Serif Bold Italic Capital O
  ^^^^^^01d64b% 𝙋   \bisansP    Mathematical Sans-Serif Bold Italic Capital P
  ^^^^^^01d64c% 𝙌   \bisansQ    Mathematical Sans-Serif Bold Italic Capital Q
  ^^^^^^01d64d% 𝙍   \bisansR    Mathematical Sans-Serif Bold Italic Capital R
  ^^^^^^01d64e% 𝙎   \bisansS    Mathematical Sans-Serif Bold Italic Capital S
  ^^^^^^01d64f% 𝙏   \bisansT    Mathematical Sans-Serif Bold Italic Capital T
  ^^^^^^01d650% 𝙐   \bisansU    Mathematical Sans-Serif Bold Italic Capital U
  ^^^^^^01d651% 𝙑   \bisansV    Mathematical Sans-Serif Bold Italic Capital V
  ^^^^^^01d652% 𝙒   \bisansW    Mathematical Sans-Serif Bold Italic Capital W
  ^^^^^^01d653% 𝙓   \bisansX    Mathematical Sans-Serif Bold Italic Capital X
  ^^^^^^01d654% 𝙔   \bisansY    Mathematical Sans-Serif Bold Italic Capital Y
  ^^^^^^01d655% 𝙕   \bisansZ    Mathematical Sans-Serif Bold Italic Capital Z
  ^^^^^^01d656% 𝙖   \bisansa    Mathematical Sans-Serif Bold Italic Small A
  ^^^^^^01d657% 𝙗   \bisansb    Mathematical Sans-Serif Bold Italic Small B
  ^^^^^^01d658% 𝙘   \bisansc    Mathematical Sans-Serif Bold Italic Small C
  ^^^^^^01d659% 𝙙   \bisansd    Mathematical Sans-Serif Bold Italic Small D
  ^^^^^^01d65a% 𝙚   \bisanse    Mathematical Sans-Serif Bold Italic Small E
  ^^^^^^01d65b% 𝙛   \bisansf    Mathematical Sans-Serif Bold Italic Small F
  ^^^^^^01d65c% 𝙜   \bisansg    Mathematical Sans-Serif Bold Italic Small G
  ^^^^^^01d65d% 𝙝   \bisansh    Mathematical Sans-Serif Bold Italic Small H
  ^^^^^^01d65e% 𝙞   \bisansi    Mathematical Sans-Serif Bold Italic Small I
  ^^^^^^01d65f% 𝙟   \bisansj    Mathematical Sans-Serif Bold Italic Small J
  ^^^^^^01d660% 𝙠   \bisansk    Mathematical Sans-Serif Bold Italic Small K
  ^^^^^^01d661% 𝙡   \bisansl    Mathematical Sans-Serif Bold Italic Small L
  ^^^^^^01d662% 𝙢   \bisansm    Mathematical Sans-Serif Bold Italic Small M
  ^^^^^^01d663% 𝙣   \bisansn    Mathematical Sans-Serif Bold Italic Small N
  ^^^^^^01d664% 𝙤   \bisanso    Mathematical Sans-Serif Bold Italic Small O
  ^^^^^^01d665% 𝙥   \bisansp    Mathematical Sans-Serif Bold Italic Small P
  ^^^^^^01d666% 𝙦   \bisansq    Mathematical Sans-Serif Bold Italic Small Q
  ^^^^^^01d667% 𝙧   \bisansr    Mathematical Sans-Serif Bold Italic Small R
  ^^^^^^01d668% 𝙨   \bisanss    Mathematical Sans-Serif Bold Italic Small S
  ^^^^^^01d669% 𝙩   \bisanst    Mathematical Sans-Serif Bold Italic Small T
  ^^^^^^01d66a% 𝙪   \bisansu    Mathematical Sans-Serif Bold Italic Small U
  ^^^^^^01d66b% 𝙫   \bisansv    Mathematical Sans-Serif Bold Italic Small V
  ^^^^^^01d66c% 𝙬   \bisansw    Mathematical Sans-Serif Bold Italic Small W
  ^^^^^^01d66d% 𝙭   \bisansx    Mathematical Sans-Serif Bold Italic Small X
  ^^^^^^01d66e% 𝙮   \bisansy    Mathematical Sans-Serif Bold Italic Small Y
  ^^^^^^01d66f% 𝙯   \bisansz    Mathematical Sans-Serif Bold Italic Small Z
  ^^^^^^01d670% 𝙰   \ttA    Mathematical Monospace Capital A
  ^^^^^^01d671% 𝙱   \ttB    Mathematical Monospace Capital B
  ^^^^^^01d672% 𝙲   \ttC    Mathematical Monospace Capital C
  ^^^^^^01d673% 𝙳   \ttD    Mathematical Monospace Capital D
  ^^^^^^01d674% 𝙴   \ttE    Mathematical Monospace Capital E
  ^^^^^^01d675% 𝙵   \ttF    Mathematical Monospace Capital F
  ^^^^^^01d676% 𝙶   \ttG    Mathematical Monospace Capital G
  ^^^^^^01d677% 𝙷   \ttH    Mathematical Monospace Capital H
  ^^^^^^01d678% 𝙸   \ttI    Mathematical Monospace Capital I
  ^^^^^^01d679% 𝙹   \ttJ    Mathematical Monospace Capital J
  ^^^^^^01d67a% 𝙺   \ttK    Mathematical Monospace Capital K
  ^^^^^^01d67b% 𝙻   \ttL    Mathematical Monospace Capital L
  ^^^^^^01d67c% 𝙼   \ttM    Mathematical Monospace Capital M
  ^^^^^^01d67d% 𝙽   \ttN    Mathematical Monospace Capital N
  ^^^^^^01d67e% 𝙾   \ttO    Mathematical Monospace Capital O
  ^^^^^^01d67f% 𝙿   \ttP    Mathematical Monospace Capital P
  ^^^^^^01d680% 𝚀   \ttQ    Mathematical Monospace Capital Q
  ^^^^^^01d681% 𝚁   \ttR    Mathematical Monospace Capital R
  ^^^^^^01d682% 𝚂   \ttS    Mathematical Monospace Capital S
  ^^^^^^01d683% 𝚃   \ttT    Mathematical Monospace Capital T
  ^^^^^^01d684% 𝚄   \ttU    Mathematical Monospace Capital U
  ^^^^^^01d685% 𝚅   \ttV    Mathematical Monospace Capital V
  ^^^^^^01d686% 𝚆   \ttW    Mathematical Monospace Capital W
  ^^^^^^01d687% 𝚇   \ttX    Mathematical Monospace Capital X
  ^^^^^^01d688% 𝚈   \ttY    Mathematical Monospace Capital Y
  ^^^^^^01d689% 𝚉   \ttZ    Mathematical Monospace Capital Z
  ^^^^^^01d68a% 𝚊   \tta    Mathematical Monospace Small A
  ^^^^^^01d68b% 𝚋   \ttb    Mathematical Monospace Small B
  ^^^^^^01d68c% 𝚌   \ttc    Mathematical Monospace Small C
  ^^^^^^01d68d% 𝚍   \ttd    Mathematical Monospace Small D
  ^^^^^^01d68e% 𝚎   \tte    Mathematical Monospace Small E
  ^^^^^^01d68f% 𝚏   \ttf    Mathematical Monospace Small F
  ^^^^^^01d690% 𝚐   \ttg    Mathematical Monospace Small G
  ^^^^^^01d691% 𝚑   \tth    Mathematical Monospace Small H
  ^^^^^^01d692% 𝚒   \tti    Mathematical Monospace Small I
  ^^^^^^01d693% 𝚓   \ttj    Mathematical Monospace Small J
  ^^^^^^01d694% 𝚔   \ttk    Mathematical Monospace Small K
  ^^^^^^01d695% 𝚕   \ttl    Mathematical Monospace Small L
  ^^^^^^01d696% 𝚖   \ttm    Mathematical Monospace Small M
  ^^^^^^01d697% 𝚗   \ttn    Mathematical Monospace Small N
  ^^^^^^01d698% 𝚘   \tto    Mathematical Monospace Small O
  ^^^^^^01d699% 𝚙   \ttp    Mathematical Monospace Small P
  ^^^^^^01d69a% 𝚚   \ttq    Mathematical Monospace Small Q
  ^^^^^^01d69b% 𝚛   \ttr    Mathematical Monospace Small R
  ^^^^^^01d69c% 𝚜   \tts    Mathematical Monospace Small S
  ^^^^^^01d69d% 𝚝   \ttt    Mathematical Monospace Small T
  ^^^^^^01d69e% 𝚞   \ttu    Mathematical Monospace Small U
  ^^^^^^01d69f% 𝚟   \ttv    Mathematical Monospace Small V
  ^^^^^^01d6a0% 𝚠   \ttw    Mathematical Monospace Small W
  ^^^^^^01d6a1% 𝚡   \ttx    Mathematical Monospace Small X
  ^^^^^^01d6a2% 𝚢   \tty    Mathematical Monospace Small Y
  ^^^^^^01d6a3% 𝚣   \ttz    Mathematical Monospace Small Z
  ^^^^^^01d6a4% 𝚤   \itimath    Mathematical Italic Small Dotless I
  ^^^^^^01d6a5% 𝚥   \itjmath    Mathematical Italic Small Dotless J
  ^^^^^^01d6a8% 𝚨   \bfAlpha    Mathematical Bold Capital Alpha
  ^^^^^^01d6a9% 𝚩   \bfBeta Mathematical Bold Capital Beta
  ^^^^^^01d6aa% 𝚪   \bfGamma    Mathematical Bold Capital Gamma
  ^^^^^^01d6ab% 𝚫   \bfDelta    Mathematical Bold Capital Delta
  ^^^^^^01d6ac% 𝚬   \bfEpsilon  Mathematical Bold Capital Epsilon
  ^^^^^^01d6ad% 𝚭   \bfZeta Mathematical Bold Capital Zeta
  ^^^^^^01d6ae% 𝚮   \bfEta  Mathematical Bold Capital Eta
  ^^^^^^01d6af% 𝚯   \bfTheta    Mathematical Bold Capital Theta
  ^^^^^^01d6b0% 𝚰   \bfIota Mathematical Bold Capital Iota
  ^^^^^^01d6b1% 𝚱   \bfKappa    Mathematical Bold Capital Kappa
  ^^^^^^01d6b2% 𝚲   \bfLambda   Mathematical Bold Capital Lamda
  ^^^^^^01d6b3% 𝚳   \bfMu   Mathematical Bold Capital Mu
  ^^^^^^01d6b4% 𝚴   \bfNu   Mathematical Bold Capital Nu
  ^^^^^^01d6b5% 𝚵   \bfXi   Mathematical Bold Capital Xi
  ^^^^^^01d6b6% 𝚶   \bfOmicron  Mathematical Bold Capital Omicron
  ^^^^^^01d6b7% 𝚷   \bfPi   Mathematical Bold Capital Pi
  ^^^^^^01d6b8% 𝚸   \bfRho  Mathematical Bold Capital Rho
  ^^^^^^01d6b9% 𝚹   \bfvarTheta Mathematical Bold Capital Theta Symbol
  ^^^^^^01d6ba% 𝚺   \bfSigma    Mathematical Bold Capital Sigma
  ^^^^^^01d6bb% 𝚻   \bfTau  Mathematical Bold Capital Tau
  ^^^^^^01d6bc% 𝚼   \bfUpsilon  Mathematical Bold Capital Upsilon
  ^^^^^^01d6bd% 𝚽   \bfPhi  Mathematical Bold Capital Phi
  ^^^^^^01d6be% 𝚾   \bfChi  Mathematical Bold Capital Chi
  ^^^^^^01d6bf% 𝚿   \bfPsi  Mathematical Bold Capital Psi
  ^^^^^^01d6c0% 𝛀   \bfOmega    Mathematical Bold Capital Omega
  ^^^^^^01d6c1% 𝛁   \bfnabla    Mathematical Bold Nabla
  ^^^^^^01d6c2% 𝛂   \bfalpha    Mathematical Bold Small Alpha
  ^^^^^^01d6c3% 𝛃   \bfbeta Mathematical Bold Small Beta
  ^^^^^^01d6c4% 𝛄   \bfgamma    Mathematical Bold Small Gamma
  ^^^^^^01d6c5% 𝛅   \bfdelta    Mathematical Bold Small Delta
  ^^^^^^01d6c6% 𝛆   \bfepsilon  Mathematical Bold Small Epsilon
  ^^^^^^01d6c7% 𝛇   \bfzeta Mathematical Bold Small Zeta
  ^^^^^^01d6c8% 𝛈   \bfeta  Mathematical Bold Small Eta
  ^^^^^^01d6c9% 𝛉   \bftheta    Mathematical Bold Small Theta
  ^^^^^^01d6ca% 𝛊   \bfiota Mathematical Bold Small Iota
  ^^^^^^01d6cb% 𝛋   \bfkappa    Mathematical Bold Small Kappa
  ^^^^^^01d6cc% 𝛌   \bflambda   Mathematical Bold Small Lamda
  ^^^^^^01d6cd% 𝛍   \bfmu   Mathematical Bold Small Mu
  ^^^^^^01d6ce% 𝛎   \bfnu   Mathematical Bold Small Nu
  ^^^^^^01d6cf% 𝛏   \bfxi   Mathematical Bold Small Xi
  ^^^^^^01d6d0% 𝛐   \bfomicron  Mathematical Bold Small Omicron
  ^^^^^^01d6d1% 𝛑   \bfpi   Mathematical Bold Small Pi
  ^^^^^^01d6d2% 𝛒   \bfrho  Mathematical Bold Small Rho
  ^^^^^^01d6d3% 𝛓   \bfvarsigma Mathematical Bold Small Final Sigma
  ^^^^^^01d6d4% 𝛔   \bfsigma    Mathematical Bold Small Sigma
  ^^^^^^01d6d5% 𝛕   \bftau  Mathematical Bold Small Tau
  ^^^^^^01d6d6% 𝛖   \bfupsilon  Mathematical Bold Small Upsilon
  ^^^^^^01d6d7% 𝛗   \bfvarphi   Mathematical Bold Small Phi
  ^^^^^^01d6d8% 𝛘   \bfchi  Mathematical Bold Small Chi
  ^^^^^^01d6d9% 𝛙   \bfpsi  Mathematical Bold Small Psi
  ^^^^^^01d6da% 𝛚   \bfomega    Mathematical Bold Small Omega
  ^^^^^^01d6db% 𝛛   \bfpartial  Mathematical Bold Partial Differential
  ^^^^^^01d6dc% 𝛜   \bfvarepsilon   Mathematical Bold Epsilon Symbol
  ^^^^^^01d6dd% 𝛝   \bfvartheta Mathematical Bold Theta Symbol
  ^^^^^^01d6de% 𝛞   \bfvarkappa Mathematical Bold Kappa Symbol
  ^^^^^^01d6df% 𝛟   \bfphi  Mathematical Bold Phi Symbol
  ^^^^^^01d6e0% 𝛠   \bfvarrho   Mathematical Bold Rho Symbol
  ^^^^^^01d6e1% 𝛡   \bfvarpi    Mathematical Bold Pi Symbol
  ^^^^^^01d6e2% 𝛢   \itAlpha    Mathematical Italic Capital Alpha
  ^^^^^^01d6e3% 𝛣   \itBeta Mathematical Italic Capital Beta
  ^^^^^^01d6e4% 𝛤   \itGamma    Mathematical Italic Capital Gamma
  ^^^^^^01d6e5% 𝛥   \itDelta    Mathematical Italic Capital Delta
  ^^^^^^01d6e6% 𝛦   \itEpsilon  Mathematical Italic Capital Epsilon
  ^^^^^^01d6e7% 𝛧   \itZeta Mathematical Italic Capital Zeta
  ^^^^^^01d6e8% 𝛨   \itEta  Mathematical Italic Capital Eta
  ^^^^^^01d6e9% 𝛩   \itTheta    Mathematical Italic Capital Theta
  ^^^^^^01d6ea% 𝛪   \itIota Mathematical Italic Capital Iota
  ^^^^^^01d6eb% 𝛫   \itKappa    Mathematical Italic Capital Kappa
  ^^^^^^01d6ec% 𝛬   \itLambda   Mathematical Italic Capital Lamda
  ^^^^^^01d6ed% 𝛭   \itMu   Mathematical Italic Capital Mu
  ^^^^^^01d6ee% 𝛮   \itNu   Mathematical Italic Capital Nu
  ^^^^^^01d6ef% 𝛯   \itXi   Mathematical Italic Capital Xi
  ^^^^^^01d6f0% 𝛰   \itOmicron  Mathematical Italic Capital Omicron
  ^^^^^^01d6f1% 𝛱   \itPi   Mathematical Italic Capital Pi
  ^^^^^^01d6f2% 𝛲   \itRho  Mathematical Italic Capital Rho
  ^^^^^^01d6f3% 𝛳   \itvarTheta Mathematical Italic Capital Theta Symbol
  ^^^^^^01d6f4% 𝛴   \itSigma    Mathematical Italic Capital Sigma
  ^^^^^^01d6f5% 𝛵   \itTau  Mathematical Italic Capital Tau
  ^^^^^^01d6f6% 𝛶   \itUpsilon  Mathematical Italic Capital Upsilon
  ^^^^^^01d6f7% 𝛷   \itPhi  Mathematical Italic Capital Phi
  ^^^^^^01d6f8% 𝛸   \itChi  Mathematical Italic Capital Chi
  ^^^^^^01d6f9% 𝛹   \itPsi  Mathematical Italic Capital Psi
  ^^^^^^01d6fa% 𝛺   \itOmega    Mathematical Italic Capital Omega
  ^^^^^^01d6fb% 𝛻   \itnabla    Mathematical Italic Nabla
  ^^^^^^01d6fc% 𝛼   \italpha    Mathematical Italic Small Alpha
  ^^^^^^01d6fd% 𝛽   \itbeta Mathematical Italic Small Beta
  ^^^^^^01d6fe% 𝛾   \itgamma    Mathematical Italic Small Gamma
  ^^^^^^01d6ff% 𝛿   \itdelta    Mathematical Italic Small Delta
  ^^^^^^01d700% 𝜀   \itepsilon  Mathematical Italic Small Epsilon
  ^^^^^^01d701% 𝜁   \itzeta Mathematical Italic Small Zeta
  ^^^^^^01d702% 𝜂   \iteta  Mathematical Italic Small Eta
  ^^^^^^01d703% 𝜃   \ittheta    Mathematical Italic Small Theta
  ^^^^^^01d704% 𝜄   \itiota Mathematical Italic Small Iota
  ^^^^^^01d705% 𝜅   \itkappa    Mathematical Italic Small Kappa
  ^^^^^^01d706% 𝜆   \itlambda   Mathematical Italic Small Lamda
  ^^^^^^01d707% 𝜇   \itmu   Mathematical Italic Small Mu
  ^^^^^^01d708% 𝜈   \itnu   Mathematical Italic Small Nu
  ^^^^^^01d709% 𝜉   \itxi   Mathematical Italic Small Xi
  ^^^^^^01d70a% 𝜊   \itomicron  Mathematical Italic Small Omicron
  ^^^^^^01d70b% 𝜋   \itpi   Mathematical Italic Small Pi
  ^^^^^^01d70c% 𝜌   \itrho  Mathematical Italic Small Rho
  ^^^^^^01d70d% 𝜍   \itvarsigma Mathematical Italic Small Final Sigma
  ^^^^^^01d70e% 𝜎   \itsigma    Mathematical Italic Small Sigma
  ^^^^^^01d70f% 𝜏   \ittau  Mathematical Italic Small Tau
  ^^^^^^01d710% 𝜐   \itupsilon  Mathematical Italic Small Upsilon
  ^^^^^^01d711% 𝜑   \itphi  Mathematical Italic Small Phi
  ^^^^^^01d712% 𝜒   \itchi  Mathematical Italic Small Chi
  ^^^^^^01d713% 𝜓   \itpsi  Mathematical Italic Small Psi
  ^^^^^^01d714% 𝜔   \itomega    Mathematical Italic Small Omega
  ^^^^^^01d715% 𝜕   \itpartial  Mathematical Italic Partial Differential
  ^^^^^^01d716% 𝜖   \itvarepsilon   Mathematical Italic Epsilon Symbol
  ^^^^^^01d717% 𝜗   \itvartheta Mathematical Italic Theta Symbol
  ^^^^^^01d718% 𝜘   \itvarkappa Mathematical Italic Kappa Symbol
  ^^^^^^01d719% 𝜙   \itvarphi   Mathematical Italic Phi Symbol
  ^^^^^^01d71a% 𝜚   \itvarrho   Mathematical Italic Rho Symbol
  ^^^^^^01d71b% 𝜛   \itvarpi    Mathematical Italic Pi Symbol
  ^^^^^^01d71c% 𝜜   \biAlpha    Mathematical Bold Italic Capital Alpha
  ^^^^^^01d71d% 𝜝   \biBeta Mathematical Bold Italic Capital Beta
  ^^^^^^01d71e% 𝜞   \biGamma    Mathematical Bold Italic Capital Gamma
  ^^^^^^01d71f% 𝜟   \biDelta    Mathematical Bold Italic Capital Delta
  ^^^^^^01d720% 𝜠   \biEpsilon  Mathematical Bold Italic Capital Epsilon
  ^^^^^^01d721% 𝜡   \biZeta Mathematical Bold Italic Capital Zeta
  ^^^^^^01d722% 𝜢   \biEta  Mathematical Bold Italic Capital Eta
  ^^^^^^01d723% 𝜣   \biTheta    Mathematical Bold Italic Capital Theta
  ^^^^^^01d724% 𝜤   \biIota Mathematical Bold Italic Capital Iota
  ^^^^^^01d725% 𝜥   \biKappa    Mathematical Bold Italic Capital Kappa
  ^^^^^^01d726% 𝜦   \biLambda   Mathematical Bold Italic Capital Lamda
  ^^^^^^01d727% 𝜧   \biMu   Mathematical Bold Italic Capital Mu
  ^^^^^^01d728% 𝜨   \biNu   Mathematical Bold Italic Capital Nu
  ^^^^^^01d729% 𝜩   \biXi   Mathematical Bold Italic Capital Xi
  ^^^^^^01d72a% 𝜪   \biOmicron  Mathematical Bold Italic Capital Omicron
  ^^^^^^01d72b% 𝜫   \biPi   Mathematical Bold Italic Capital Pi
  ^^^^^^01d72c% 𝜬   \biRho  Mathematical Bold Italic Capital Rho
  ^^^^^^01d72d% 𝜭   \bivarTheta Mathematical Bold Italic Capital Theta Symbol
  ^^^^^^01d72e% 𝜮   \biSigma    Mathematical Bold Italic Capital Sigma
  ^^^^^^01d72f% 𝜯   \biTau  Mathematical Bold Italic Capital Tau
  ^^^^^^01d730% 𝜰   \biUpsilon  Mathematical Bold Italic Capital Upsilon
  ^^^^^^01d731% 𝜱   \biPhi  Mathematical Bold Italic Capital Phi
  ^^^^^^01d732% 𝜲   \biChi  Mathematical Bold Italic Capital Chi
  ^^^^^^01d733% 𝜳   \biPsi  Mathematical Bold Italic Capital Psi
  ^^^^^^01d734% 𝜴   \biOmega    Mathematical Bold Italic Capital Omega
  ^^^^^^01d735% 𝜵   \binabla    Mathematical Bold Italic Nabla
  ^^^^^^01d736% 𝜶   \bialpha    Mathematical Bold Italic Small Alpha
  ^^^^^^01d737% 𝜷   \bibeta Mathematical Bold Italic Small Beta
  ^^^^^^01d738% 𝜸   \bigamma    Mathematical Bold Italic Small Gamma
  ^^^^^^01d739% 𝜹   \bidelta    Mathematical Bold Italic Small Delta
  ^^^^^^01d73a% 𝜺   \biepsilon  Mathematical Bold Italic Small Epsilon
  ^^^^^^01d73b% 𝜻   \bizeta Mathematical Bold Italic Small Zeta
  ^^^^^^01d73c% 𝜼   \bieta  Mathematical Bold Italic Small Eta
  ^^^^^^01d73d% 𝜽   \bitheta    Mathematical Bold Italic Small Theta
  ^^^^^^01d73e% 𝜾   \biiota Mathematical Bold Italic Small Iota
  ^^^^^^01d73f% 𝜿   \bikappa    Mathematical Bold Italic Small Kappa
  ^^^^^^01d740% 𝝀   \bilambda   Mathematical Bold Italic Small Lamda
  ^^^^^^01d741% 𝝁   \bimu   Mathematical Bold Italic Small Mu
  ^^^^^^01d742% 𝝂   \binu   Mathematical Bold Italic Small Nu
  ^^^^^^01d743% 𝝃   \bixi   Mathematical Bold Italic Small Xi
  ^^^^^^01d744% 𝝄   \biomicron  Mathematical Bold Italic Small Omicron
  ^^^^^^01d745% 𝝅   \bipi   Mathematical Bold Italic Small Pi
  ^^^^^^01d746% 𝝆   \birho  Mathematical Bold Italic Small Rho
  ^^^^^^01d747% 𝝇   \bivarsigma Mathematical Bold Italic Small Final Sigma
  ^^^^^^01d748% 𝝈   \bisigma    Mathematical Bold Italic Small Sigma
  ^^^^^^01d749% 𝝉   \bitau  Mathematical Bold Italic Small Tau
  ^^^^^^01d74a% 𝝊   \biupsilon  Mathematical Bold Italic Small Upsilon
  ^^^^^^01d74b% 𝝋   \biphi  Mathematical Bold Italic Small Phi
  ^^^^^^01d74c% 𝝌   \bichi  Mathematical Bold Italic Small Chi
  ^^^^^^01d74d% 𝝍   \bipsi  Mathematical Bold Italic Small Psi
  ^^^^^^01d74e% 𝝎   \biomega    Mathematical Bold Italic Small Omega
  ^^^^^^01d74f% 𝝏   \bipartial  Mathematical Bold Italic Partial Differential
  ^^^^^^01d750% 𝝐   \bivarepsilon   Mathematical Bold Italic Epsilon Symbol
  ^^^^^^01d751% 𝝑   \bivartheta Mathematical Bold Italic Theta Symbol
  ^^^^^^01d752% 𝝒   \bivarkappa Mathematical Bold Italic Kappa Symbol
  ^^^^^^01d753% 𝝓   \bivarphi   Mathematical Bold Italic Phi Symbol
  ^^^^^^01d754% 𝝔   \bivarrho   Mathematical Bold Italic Rho Symbol
  ^^^^^^01d755% 𝝕   \bivarpi    Mathematical Bold Italic Pi Symbol
  ^^^^^^01d756% 𝝖   \bsansAlpha Mathematical Sans-Serif Bold Capital Alpha
  ^^^^^^01d757% 𝝗   \bsansBeta  Mathematical Sans-Serif Bold Capital Beta
  ^^^^^^01d758% 𝝘   \bsansGamma Mathematical Sans-Serif Bold Capital Gamma
  ^^^^^^01d759% 𝝙   \bsansDelta Mathematical Sans-Serif Bold Capital Delta
  ^^^^^^01d75a% 𝝚   \bsansEpsilon   Mathematical Sans-Serif Bold Capital Epsilon
  ^^^^^^01d75b% 𝝛   \bsansZeta  Mathematical Sans-Serif Bold Capital Zeta
  ^^^^^^01d75c% 𝝜   \bsansEta   Mathematical Sans-Serif Bold Capital Eta
  ^^^^^^01d75d% 𝝝   \bsansTheta Mathematical Sans-Serif Bold Capital Theta
  ^^^^^^01d75e% 𝝞   \bsansIota  Mathematical Sans-Serif Bold Capital Iota
  ^^^^^^01d75f% 𝝟   \bsansKappa Mathematical Sans-Serif Bold Capital Kappa
  ^^^^^^01d760% 𝝠   \bsansLambda    Mathematical Sans-Serif Bold Capital Lamda
  ^^^^^^01d761% 𝝡   \bsansMu    Mathematical Sans-Serif Bold Capital Mu
  ^^^^^^01d762% 𝝢   \bsansNu    Mathematical Sans-Serif Bold Capital Nu
  ^^^^^^01d763% 𝝣   \bsansXi    Mathematical Sans-Serif Bold Capital Xi
  ^^^^^^01d764% 𝝤   \bsansOmicron   Mathematical Sans-Serif Bold Capital Omicron
  ^^^^^^01d765% 𝝥   \bsansPi    Mathematical Sans-Serif Bold Capital Pi
  ^^^^^^01d766% 𝝦   \bsansRho   Mathematical Sans-Serif Bold Capital Rho
  ^^^^^^01d767% 𝝧   \bsansvarTheta  Mathematical Sans-Serif Bold Capital Theta Symbol
  ^^^^^^01d768% 𝝨   \bsansSigma Mathematical Sans-Serif Bold Capital Sigma
  ^^^^^^01d769% 𝝩   \bsansTau   Mathematical Sans-Serif Bold Capital Tau
  ^^^^^^01d76a% 𝝪   \bsansUpsilon   Mathematical Sans-Serif Bold Capital Upsilon
  ^^^^^^01d76b% 𝝫   \bsansPhi   Mathematical Sans-Serif Bold Capital Phi
  ^^^^^^01d76c% 𝝬   \bsansChi   Mathematical Sans-Serif Bold Capital Chi
  ^^^^^^01d76d% 𝝭   \bsansPsi   Mathematical Sans-Serif Bold Capital Psi
  ^^^^^^01d76e% 𝝮   \bsansOmega Mathematical Sans-Serif Bold Capital Omega
  ^^^^^^01d76f% 𝝯   \bsansnabla Mathematical Sans-Serif Bold Nabla
  ^^^^^^01d770% 𝝰   \bsansalpha Mathematical Sans-Serif Bold Small Alpha
  ^^^^^^01d771% 𝝱   \bsansbeta  Mathematical Sans-Serif Bold Small Beta
  ^^^^^^01d772% 𝝲   \bsansgamma Mathematical Sans-Serif Bold Small Gamma
  ^^^^^^01d773% 𝝳   \bsansdelta Mathematical Sans-Serif Bold Small Delta
  ^^^^^^01d774% 𝝴   \bsansepsilon   Mathematical Sans-Serif Bold Small Epsilon
  ^^^^^^01d775% 𝝵   \bsanszeta  Mathematical Sans-Serif Bold Small Zeta
  ^^^^^^01d776% 𝝶   \bsanseta   Mathematical Sans-Serif Bold Small Eta
  ^^^^^^01d777% 𝝷   \bsanstheta Mathematical Sans-Serif Bold Small Theta
  ^^^^^^01d778% 𝝸   \bsansiota  Mathematical Sans-Serif Bold Small Iota
  ^^^^^^01d779% 𝝹   \bsanskappa Mathematical Sans-Serif Bold Small Kappa
  ^^^^^^01d77a% 𝝺   \bsanslambda    Mathematical Sans-Serif Bold Small Lamda
  ^^^^^^01d77b% 𝝻   \bsansmu    Mathematical Sans-Serif Bold Small Mu
  ^^^^^^01d77c% 𝝼   \bsansnu    Mathematical Sans-Serif Bold Small Nu
  ^^^^^^01d77d% 𝝽   \bsansxi    Mathematical Sans-Serif Bold Small Xi
  ^^^^^^01d77e% 𝝾   \bsansomicron   Mathematical Sans-Serif Bold Small Omicron
  ^^^^^^01d77f% 𝝿   \bsanspi    Mathematical Sans-Serif Bold Small Pi
  ^^^^^^01d780% 𝞀   \bsansrho   Mathematical Sans-Serif Bold Small Rho
  ^^^^^^01d781% 𝞁   \bsansvarsigma  Mathematical Sans-Serif Bold Small Final Sigma
  ^^^^^^01d782% 𝞂   \bsanssigma Mathematical Sans-Serif Bold Small Sigma
  ^^^^^^01d783% 𝞃   \bsanstau   Mathematical Sans-Serif Bold Small Tau
  ^^^^^^01d784% 𝞄   \bsansupsilon   Mathematical Sans-Serif Bold Small Upsilon
  ^^^^^^01d785% 𝞅   \bsansphi   Mathematical Sans-Serif Bold Small Phi
  ^^^^^^01d786% 𝞆   \bsanschi   Mathematical Sans-Serif Bold Small Chi
  ^^^^^^01d787% 𝞇   \bsanspsi   Mathematical Sans-Serif Bold Small Psi
  ^^^^^^01d788% 𝞈   \bsansomega Mathematical Sans-Serif Bold Small Omega
  ^^^^^^01d789% 𝞉   \bsanspartial   Mathematical Sans-Serif Bold Partial Differential
  ^^^^^^01d78a% 𝞊   \bsansvarepsilon    Mathematical Sans-Serif Bold Epsilon Symbol
  ^^^^^^01d78b% 𝞋   \bsansvartheta  Mathematical Sans-Serif Bold Theta Symbol
  ^^^^^^01d78c% 𝞌   \bsansvarkappa  Mathematical Sans-Serif Bold Kappa Symbol
  ^^^^^^01d78d% 𝞍   \bsansvarphi    Mathematical Sans-Serif Bold Phi Symbol
  ^^^^^^01d78e% 𝞎   \bsansvarrho    Mathematical Sans-Serif Bold Rho Symbol
  ^^^^^^01d78f% 𝞏   \bsansvarpi Mathematical Sans-Serif Bold Pi Symbol
  ^^^^^^01d790% 𝞐   \bisansAlpha    Mathematical Sans-Serif Bold Italic Capital Alpha
  ^^^^^^01d791% 𝞑   \bisansBeta Mathematical Sans-Serif Bold Italic Capital Beta
  ^^^^^^01d792% 𝞒   \bisansGamma    Mathematical Sans-Serif Bold Italic Capital Gamma
  ^^^^^^01d793% 𝞓   \bisansDelta    Mathematical Sans-Serif Bold Italic Capital Delta
  ^^^^^^01d794% 𝞔   \bisansEpsilon  Mathematical Sans-Serif Bold Italic Capital Epsilon
  ^^^^^^01d795% 𝞕   \bisansZeta Mathematical Sans-Serif Bold Italic Capital Zeta
  ^^^^^^01d796% 𝞖   \bisansEta  Mathematical Sans-Serif Bold Italic Capital Eta
  ^^^^^^01d797% 𝞗   \bisansTheta    Mathematical Sans-Serif Bold Italic Capital Theta
  ^^^^^^01d798% 𝞘   \bisansIota Mathematical Sans-Serif Bold Italic Capital Iota
  ^^^^^^01d799% 𝞙   \bisansKappa    Mathematical Sans-Serif Bold Italic Capital Kappa
  ^^^^^^01d79a% 𝞚   \bisansLambda   Mathematical Sans-Serif Bold Italic Capital Lamda
  ^^^^^^01d79b% 𝞛   \bisansMu   Mathematical Sans-Serif Bold Italic Capital Mu
  ^^^^^^01d79c% 𝞜   \bisansNu   Mathematical Sans-Serif Bold Italic Capital Nu
  ^^^^^^01d79d% 𝞝   \bisansXi   Mathematical Sans-Serif Bold Italic Capital Xi
  ^^^^^^01d79e% 𝞞   \bisansOmicron  Mathematical Sans-Serif Bold Italic Capital Omicron
  ^^^^^^01d79f% 𝞟   \bisansPi   Mathematical Sans-Serif Bold Italic Capital Pi
  ^^^^^^01d7a0% 𝞠   \bisansRho  Mathematical Sans-Serif Bold Italic Capital Rho
  ^^^^^^01d7a1% 𝞡   \bisansvarTheta Mathematical Sans-Serif Bold Italic Capital Theta Symbol
  ^^^^^^01d7a2% 𝞢   \bisansSigma    Mathematical Sans-Serif Bold Italic Capital Sigma
  ^^^^^^01d7a3% 𝞣   \bisansTau  Mathematical Sans-Serif Bold Italic Capital Tau
  ^^^^^^01d7a4% 𝞤   \bisansUpsilon  Mathematical Sans-Serif Bold Italic Capital Upsilon
  ^^^^^^01d7a5% 𝞥   \bisansPhi  Mathematical Sans-Serif Bold Italic Capital Phi
  ^^^^^^01d7a6% 𝞦   \bisansChi  Mathematical Sans-Serif Bold Italic Capital Chi
  ^^^^^^01d7a7% 𝞧   \bisansPsi  Mathematical Sans-Serif Bold Italic Capital Psi
  ^^^^^^01d7a8% 𝞨   \bisansOmega    Mathematical Sans-Serif Bold Italic Capital Omega
  ^^^^^^01d7a9% 𝞩   \bisansnabla    Mathematical Sans-Serif Bold Italic Nabla
  ^^^^^^01d7aa% 𝞪   \bisansalpha    Mathematical Sans-Serif Bold Italic Small Alpha
  ^^^^^^01d7ab% 𝞫   \bisansbeta Mathematical Sans-Serif Bold Italic Small Beta
  ^^^^^^01d7ac% 𝞬   \bisansgamma    Mathematical Sans-Serif Bold Italic Small Gamma
  ^^^^^^01d7ad% 𝞭   \bisansdelta    Mathematical Sans-Serif Bold Italic Small Delta
  ^^^^^^01d7ae% 𝞮   \bisansepsilon  Mathematical Sans-Serif Bold Italic Small Epsilon
  ^^^^^^01d7af% 𝞯   \bisanszeta Mathematical Sans-Serif Bold Italic Small Zeta
  ^^^^^^01d7b0% 𝞰   \bisanseta  Mathematical Sans-Serif Bold Italic Small Eta
  ^^^^^^01d7b1% 𝞱   \bisanstheta    Mathematical Sans-Serif Bold Italic Small Theta
  ^^^^^^01d7b2% 𝞲   \bisansiota Mathematical Sans-Serif Bold Italic Small Iota
  ^^^^^^01d7b3% 𝞳   \bisanskappa    Mathematical Sans-Serif Bold Italic Small Kappa
  ^^^^^^01d7b4% 𝞴   \bisanslambda   Mathematical Sans-Serif Bold Italic Small Lamda
  ^^^^^^01d7b5% 𝞵   \bisansmu   Mathematical Sans-Serif Bold Italic Small Mu
  ^^^^^^01d7b6% 𝞶   \bisansnu   Mathematical Sans-Serif Bold Italic Small Nu
  ^^^^^^01d7b7% 𝞷   \bisansxi   Mathematical Sans-Serif Bold Italic Small Xi
  ^^^^^^01d7b8% 𝞸   \bisansomicron  Mathematical Sans-Serif Bold Italic Small Omicron
  ^^^^^^01d7b9% 𝞹   \bisanspi   Mathematical Sans-Serif Bold Italic Small Pi
  ^^^^^^01d7ba% 𝞺   \bisansrho  Mathematical Sans-Serif Bold Italic Small Rho
  ^^^^^^01d7bb% 𝞻   \bisansvarsigma Mathematical Sans-Serif Bold Italic Small Final Sigma
  ^^^^^^01d7bc% 𝞼   \bisanssigma    Mathematical Sans-Serif Bold Italic Small Sigma
  ^^^^^^01d7bd% 𝞽   \bisanstau  Mathematical Sans-Serif Bold Italic Small Tau
  ^^^^^^01d7be% 𝞾   \bisansupsilon  Mathematical Sans-Serif Bold Italic Small Upsilon
  ^^^^^^01d7bf% 𝞿   \bisansphi  Mathematical Sans-Serif Bold Italic Small Phi
  ^^^^^^01d7c0% 𝟀   \bisanschi  Mathematical Sans-Serif Bold Italic Small Chi
  ^^^^^^01d7c1% 𝟁   \bisanspsi  Mathematical Sans-Serif Bold Italic Small Psi
  ^^^^^^01d7c2% 𝟂   \bisansomega    Mathematical Sans-Serif Bold Italic Small Omega
  ^^^^^^01d7c3% 𝟃   \bisanspartial  Mathematical Sans-Serif Bold Italic Partial Differential
  ^^^^^^01d7c4% 𝟄   \bisansvarepsilon   Mathematical Sans-Serif Bold Italic Epsilon Symbol
  ^^^^^^01d7c5% 𝟅   \bisansvartheta Mathematical Sans-Serif Bold Italic Theta Symbol
  ^^^^^^01d7c6% 𝟆   \bisansvarkappa Mathematical Sans-Serif Bold Italic Kappa Symbol
  ^^^^^^01d7c7% 𝟇   \bisansvarphi   Mathematical Sans-Serif Bold Italic Phi Symbol
  ^^^^^^01d7c8% 𝟈   \bisansvarrho   Mathematical Sans-Serif Bold Italic Rho Symbol
  ^^^^^^01d7c9% 𝟉   \bisansvarpi    Mathematical Sans-Serif Bold Italic Pi Symbol
  ^^^^^^01d7ca% 𝟊   \bfDigamma  Mathematical Bold Capital Digamma
  ^^^^^^01d7cb% 𝟋   \bfdigamma  Mathematical Bold Small Digamma
  ^^^^^^01d7ce% 𝟎   \bfzero Mathematical Bold Digit Zero
  ^^^^^^01d7cf% 𝟏   \bfone  Mathematical Bold Digit One
  ^^^^^^01d7d0% 𝟐   \bftwo  Mathematical Bold Digit Two
  ^^^^^^01d7d1% 𝟑   \bfthree    Mathematical Bold Digit Three
  ^^^^^^01d7d2% 𝟒   \bffour Mathematical Bold Digit Four
  ^^^^^^01d7d3% 𝟓   \bffive Mathematical Bold Digit Five
  ^^^^^^01d7d4% 𝟔   \bfsix  Mathematical Bold Digit Six
  ^^^^^^01d7d5% 𝟕   \bfseven    Mathematical Bold Digit Seven
  ^^^^^^01d7d6% 𝟖   \bfeight    Mathematical Bold Digit Eight
  ^^^^^^01d7d7% 𝟗   \bfnine Mathematical Bold Digit Nine
  ^^^^^^01d7d8% 𝟘   \bbzero Mathematical Double-Struck Digit Zero
  ^^^^^^01d7d9% 𝟙   \bbone  Mathematical Double-Struck Digit One
  ^^^^^^01d7da% 𝟚   \bbtwo  Mathematical Double-Struck Digit Two
  ^^^^^^01d7db% 𝟛   \bbthree    Mathematical Double-Struck Digit Three
  ^^^^^^01d7dc% 𝟜   \bbfour Mathematical Double-Struck Digit Four
  ^^^^^^01d7dd% 𝟝   \bbfive Mathematical Double-Struck Digit Five
  ^^^^^^01d7de% 𝟞   \bbsix  Mathematical Double-Struck Digit Six
  ^^^^^^01d7df% 𝟟   \bbseven    Mathematical Double-Struck Digit Seven
  ^^^^^^01d7e0% 𝟠   \bbeight    Mathematical Double-Struck Digit Eight
  ^^^^^^01d7e1% 𝟡   \bbnine Mathematical Double-Struck Digit Nine
  ^^^^^^01d7e2% 𝟢   \sanszero   Mathematical Sans-Serif Digit Zero
  ^^^^^^01d7e3% 𝟣   \sansone    Mathematical Sans-Serif Digit One
  ^^^^^^01d7e4% 𝟤   \sanstwo    Mathematical Sans-Serif Digit Two
  ^^^^^^01d7e5% 𝟥   \sansthree  Mathematical Sans-Serif Digit Three
  ^^^^^^01d7e6% 𝟦   \sansfour   Mathematical Sans-Serif Digit Four
  ^^^^^^01d7e7% 𝟧   \sansfive   Mathematical Sans-Serif Digit Five
  ^^^^^^01d7e8% 𝟨   \sanssix    Mathematical Sans-Serif Digit Six
  ^^^^^^01d7e9% 𝟩   \sansseven  Mathematical Sans-Serif Digit Seven
  ^^^^^^01d7ea% 𝟪   \sanseight  Mathematical Sans-Serif Digit Eight
  ^^^^^^01d7eb% 𝟫   \sansnine   Mathematical Sans-Serif Digit Nine
  ^^^^^^01d7ec% 𝟬   \bsanszero  Mathematical Sans-Serif Bold Digit Zero
  ^^^^^^01d7ed% 𝟭   \bsansone   Mathematical Sans-Serif Bold Digit One
  ^^^^^^01d7ee% 𝟮   \bsanstwo   Mathematical Sans-Serif Bold Digit Two
  ^^^^^^01d7ef% 𝟯   \bsansthree Mathematical Sans-Serif Bold Digit Three
  ^^^^^^01d7f0% 𝟰   \bsansfour  Mathematical Sans-Serif Bold Digit Four
  ^^^^^^01d7f1% 𝟱   \bsansfive  Mathematical Sans-Serif Bold Digit Five
  ^^^^^^01d7f2% 𝟲   \bsanssix   Mathematical Sans-Serif Bold Digit Six
  ^^^^^^01d7f3% 𝟳   \bsansseven Mathematical Sans-Serif Bold Digit Seven
  ^^^^^^01d7f4% 𝟴   \bsanseight Mathematical Sans-Serif Bold Digit Eight
  ^^^^^^01d7f5% 𝟵   \bsansnine  Mathematical Sans-Serif Bold Digit Nine
  ^^^^^^01d7f6% 𝟶   \ttzero Mathematical Monospace Digit Zero
  ^^^^^^01d7f7% 𝟷   \ttone  Mathematical Monospace Digit One
  ^^^^^^01d7f8% 𝟸   \tttwo  Mathematical Monospace Digit Two
  ^^^^^^01d7f9% 𝟹   \ttthree    Mathematical Monospace Digit Three
  ^^^^^^01d7fa% 𝟺   \ttfour Mathematical Monospace Digit Four
  ^^^^^^01d7fb% 𝟻   \ttfive Mathematical Monospace Digit Five
  ^^^^^^01d7fc% 𝟼   \ttsix  Mathematical Monospace Digit Six
  ^^^^^^01d7fd% 𝟽   \ttseven    Mathematical Monospace Digit Seven
  ^^^^^^01d7fe% 𝟾   \tteight    Mathematical Monospace Digit Eight
  ^^^^^^01d7ff% 𝟿   \ttnine Mathematical Monospace Digit Nine
  % zero-padded 6-digit hex (emoji)
  ^^^^^^01f004% 🀄   \:mahjong:  Mahjong Tile Red Dragon
  ^^^^^^01f0cf% 🃏   \:black_joker:  Playing Card Black Joker
  ^^^^^^01f170% 🅰   \:a:    Negative Squared Latin Capital Letter A
  ^^^^^^01f171% 🅱   \:b:    Negative Squared Latin Capital Letter B
  ^^^^^^01f17e% 🅾   \:o2:   Negative Squared Latin Capital Letter O
  ^^^^^^01f17f% 🅿   \:parking:  Negative Squared Latin Capital Letter P
  ^^^^^^01f18e% 🆎   \:ab:   Negative Squared Ab
  ^^^^^^01f191% 🆑   \:cl:   Squared Cl
  ^^^^^^01f192% 🆒   \:cool: Squared Cool
  ^^^^^^01f193% 🆓   \:free: Squared Free
  ^^^^^^01f194% 🆔   \:id:   Squared Id
  ^^^^^^01f195% 🆕   \:new:  Squared New
  ^^^^^^01f196% 🆖   \:ng:   Squared Ng
  ^^^^^^01f197% 🆗   \:ok:   Squared Ok
  ^^^^^^01f198% 🆘   \:sos:  Squared Sos
  ^^^^^^01f199% 🆙   \:up:   Squared Up With Exclamation Mark
  ^^^^^^01f19a% 🆚   \:vs:   Squared Vs
  ^^^^^^01f201% 🈁   \:koko: Squared Katakana Koko
  ^^^^^^01f202% 🈂   \:sa:   Squared Katakana Sa
  ^^^^^^01f21a% 🈚   \:u7121:    Squared Cjk Unified Ideograph-7121
  ^^^^^^01f22f% 🈯   \:u6307:    Squared Cjk Unified Ideograph-6307
  ^^^^^^01f232% 🈲   \:u7981:    Squared Cjk Unified Ideograph-7981
  ^^^^^^01f233% 🈳   \:u7a7a:    Squared Cjk Unified Ideograph-7A7A
  ^^^^^^01f234% 🈴   \:u5408:    Squared Cjk Unified Ideograph-5408
  ^^^^^^01f235% 🈵   \:u6e80:    Squared Cjk Unified Ideograph-6E80
  ^^^^^^01f236% 🈶   \:u6709:    Squared Cjk Unified Ideograph-6709
  ^^^^^^01f237% 🈷   \:u6708:    Squared Cjk Unified Ideograph-6708
  ^^^^^^01f238% 🈸   \:u7533:    Squared Cjk Unified Ideograph-7533
  ^^^^^^01f239% 🈹   \:u5272:    Squared Cjk Unified Ideograph-5272
  ^^^^^^01f23a% 🈺   \:u55b6:    Squared Cjk Unified Ideograph-55B6
  ^^^^^^01f250% 🉐   \:ideograph_advantage:  Circled Ideograph Advantage
  ^^^^^^01f251% 🉑   \:accept:   Circled Ideograph Accept
  ^^^^^^01f300% 🌀   \:cyclone:  Cyclone
  ^^^^^^01f301% 🌁   \:foggy:    Foggy
  ^^^^^^01f302% 🌂   \:closed_umbrella:  Closed Umbrella
  ^^^^^^01f303% 🌃   \:night_with_stars: Night With Stars
  ^^^^^^01f304% 🌄   \:sunrise_over_mountains:   Sunrise Over Mountains
  ^^^^^^01f305% 🌅   \:sunrise:  Sunrise
  ^^^^^^01f306% 🌆   \:city_sunset:  Cityscape At Dusk
  ^^^^^^01f307% 🌇   \:city_sunrise: Sunset Over Buildings
  ^^^^^^01f308% 🌈   \:rainbow:  Rainbow
  ^^^^^^01f309% 🌉   \:bridge_at_night:  Bridge At Night
  ^^^^^^01f30a% 🌊   \:ocean:    Water Wave
  ^^^^^^01f30b% 🌋   \:volcano:  Volcano
  ^^^^^^01f30c% 🌌   \:milky_way:    Milky Way
  ^^^^^^01f30d% 🌍   \:earth_africa: Earth Globe Europe-Africa
  ^^^^^^01f30e% 🌎   \:earth_americas:   Earth Globe Americas
  ^^^^^^01f30f% 🌏   \:earth_asia:   Earth Globe Asia-Australia
  ^^^^^^01f310% 🌐   \:globe_with_meridians: Globe With Meridians
  ^^^^^^01f311% 🌑   \:new_moon: New Moon Symbol
  ^^^^^^01f312% 🌒   \:waxing_crescent_moon: Waxing Crescent Moon Symbol
  ^^^^^^01f313% 🌓   \:first_quarter_moon:   First Quarter Moon Symbol
  ^^^^^^01f314% 🌔   \:moon: Waxing Gibbous Moon Symbol
  ^^^^^^01f315% 🌕   \:full_moon:    Full Moon Symbol
  ^^^^^^01f316% 🌖   \:waning_gibbous_moon:  Waning Gibbous Moon Symbol
  ^^^^^^01f317% 🌗   \:last_quarter_moon:    Last Quarter Moon Symbol
  ^^^^^^01f318% 🌘   \:waning_crescent_moon: Waning Crescent Moon Symbol
  ^^^^^^01f319% 🌙   \:crescent_moon:    Crescent Moon
  ^^^^^^01f31a% 🌚   \:new_moon_with_face:   New Moon With Face
  ^^^^^^01f31b% 🌛   \:first_quarter_moon_with_face: First Quarter Moon With Face
  ^^^^^^01f31c% 🌜   \:last_quarter_moon_with_face:  Last Quarter Moon With Face
  ^^^^^^01f31d% 🌝   \:full_moon_with_face:  Full Moon With Face
  ^^^^^^01f31e% 🌞   \:sun_with_face:    Sun With Face
  ^^^^^^01f31f% 🌟   \:star2:    Glowing Star
  ^^^^^^01f320% 🌠   \:stars:    Shooting Star
  ^^^^^^01f330% 🌰   \:chestnut: Chestnut
  ^^^^^^01f331% 🌱   \:seedling: Seedling
  ^^^^^^01f332% 🌲   \:evergreen_tree:   Evergreen Tree
  ^^^^^^01f333% 🌳   \:deciduous_tree:   Deciduous Tree
  ^^^^^^01f334% 🌴   \:palm_tree:    Palm Tree
  ^^^^^^01f335% 🌵   \:cactus:   Cactus
  ^^^^^^01f337% 🌷   \:tulip:    Tulip
  ^^^^^^01f338% 🌸   \:cherry_blossom:   Cherry Blossom
  ^^^^^^01f339% 🌹   \:rose: Rose
  ^^^^^^01f33a% 🌺   \:hibiscus: Hibiscus
  ^^^^^^01f33b% 🌻   \:sunflower:    Sunflower
  ^^^^^^01f33c% 🌼   \:blossom:  Blossom
  ^^^^^^01f33d% 🌽   \:corn: Ear Of Maize
  ^^^^^^01f33e% 🌾   \:ear_of_rice:  Ear Of Rice
  ^^^^^^01f33f% 🌿   \:herb: Herb
  ^^^^^^01f340% 🍀   \:four_leaf_clover: Four Leaf Clover
  ^^^^^^01f341% 🍁   \:maple_leaf:   Maple Leaf
  ^^^^^^01f342% 🍂   \:fallen_leaf:  Fallen Leaf
  ^^^^^^01f343% 🍃   \:leaves:   Leaf Fluttering In Wind
  ^^^^^^01f344% 🍄   \:mushroom: Mushroom
  ^^^^^^01f345% 🍅   \:tomato:   Tomato
  ^^^^^^01f346% 🍆   \:eggplant: Aubergine
  ^^^^^^01f347% 🍇   \:grapes:   Grapes
  ^^^^^^01f348% 🍈   \:melon:    Melon
  ^^^^^^01f349% 🍉   \:watermelon:   Watermelon
  ^^^^^^01f34a% 🍊   \:tangerine:    Tangerine
  ^^^^^^01f34b% 🍋   \:lemon:    Lemon
  ^^^^^^01f34c% 🍌   \:banana:   Banana
  ^^^^^^01f34d% 🍍   \:pineapple:    Pineapple
  ^^^^^^01f34e% 🍎   \:apple:    Red Apple
  ^^^^^^01f34f% 🍏   \:green_apple:  Green Apple
  ^^^^^^01f350% 🍐   \:pear: Pear
  ^^^^^^01f351% 🍑   \:peach:    Peach
  ^^^^^^01f352% 🍒   \:cherries: Cherries
  ^^^^^^01f353% 🍓   \:strawberry:   Strawberry
  ^^^^^^01f354% 🍔   \:hamburger:    Hamburger
  ^^^^^^01f355% 🍕   \:pizza:    Slice Of Pizza
  ^^^^^^01f356% 🍖   \:meat_on_bone: Meat On Bone
  ^^^^^^01f357% 🍗   \:poultry_leg:  Poultry Leg
  ^^^^^^01f358% 🍘   \:rice_cracker: Rice Cracker
  ^^^^^^01f359% 🍙   \:rice_ball:    Rice Ball
  ^^^^^^01f35a% 🍚   \:rice: Cooked Rice
  ^^^^^^01f35b% 🍛   \:curry:    Curry And Rice
  ^^^^^^01f35c% 🍜   \:ramen:    Steaming Bowl
  ^^^^^^01f35d% 🍝   \:spaghetti:    Spaghetti
  ^^^^^^01f35e% 🍞   \:bread:    Bread
  ^^^^^^01f35f% 🍟   \:fries:    French Fries
  ^^^^^^01f360% 🍠   \:sweet_potato: Roasted Sweet Potato
  ^^^^^^01f361% 🍡   \:dango:    Dango
  ^^^^^^01f362% 🍢   \:oden: Oden
  ^^^^^^01f363% 🍣   \:sushi:    Sushi
  ^^^^^^01f364% 🍤   \:fried_shrimp: Fried Shrimp
  ^^^^^^01f365% 🍥   \:fish_cake:    Fish Cake With Swirl Design
  ^^^^^^01f366% 🍦   \:icecream: Soft Ice Cream
  ^^^^^^01f367% 🍧   \:shaved_ice:   Shaved Ice
  ^^^^^^01f368% 🍨   \:ice_cream:    Ice Cream
  ^^^^^^01f369% 🍩   \:doughnut: Doughnut
  ^^^^^^01f36a% 🍪   \:cookie:   Cookie
  ^^^^^^01f36b% 🍫   \:chocolate_bar:    Chocolate Bar
  ^^^^^^01f36c% 🍬   \:candy:    Candy
  ^^^^^^01f36d% 🍭   \:lollipop: Lollipop
  ^^^^^^01f36e% 🍮   \:custard:  Custard
  ^^^^^^01f36f% 🍯   \:honey_pot:    Honey Pot
  ^^^^^^01f370% 🍰   \:cake: Shortcake
  ^^^^^^01f371% 🍱   \:bento:    Bento Box
  ^^^^^^01f372% 🍲   \:stew: Pot Of Food
  ^^^^^^01f373% 🍳   \:egg:  Cooking
  ^^^^^^01f374% 🍴   \:fork_and_knife:   Fork And Knife
  ^^^^^^01f375% 🍵   \:tea:  Teacup Without Handle
  ^^^^^^01f376% 🍶   \:sake: Sake Bottle And Cup
  ^^^^^^01f377% 🍷   \:wine_glass:   Wine Glass
  ^^^^^^01f378% 🍸   \:cocktail: Cocktail Glass
  ^^^^^^01f379% 🍹   \:tropical_drink:   Tropical Drink
  ^^^^^^01f37a% 🍺   \:beer: Beer Mug
  ^^^^^^01f37b% 🍻   \:beers:    Clinking Beer Mugs
  ^^^^^^01f37c% 🍼   \:baby_bottle:  Baby Bottle
  ^^^^^^01f380% 🎀   \:ribbon:   Ribbon
  ^^^^^^01f381% 🎁   \:gift: Wrapped Present
  ^^^^^^01f382% 🎂   \:birthday: Birthday Cake
  ^^^^^^01f383% 🎃   \:jack_o_lantern:   Jack-O-Lantern
  ^^^^^^01f384% 🎄   \:christmas_tree:   Christmas Tree
  ^^^^^^01f385% 🎅   \:santa:    Father Christmas
  ^^^^^^01f386% 🎆   \:fireworks:    Fireworks
  ^^^^^^01f387% 🎇   \:sparkler: Firework Sparkler
  ^^^^^^01f388% 🎈   \:balloon:  Balloon
  ^^^^^^01f389% 🎉   \:tada: Party Popper
  ^^^^^^01f38a% 🎊   \:confetti_ball:    Confetti Ball
  ^^^^^^01f38b% 🎋   \:tanabata_tree:    Tanabata Tree
  ^^^^^^01f38c% 🎌   \:crossed_flags:    Crossed Flags
  ^^^^^^01f38d% 🎍   \:bamboo:   Pine Decoration
  ^^^^^^01f38e% 🎎   \:dolls:    Japanese Dolls
  ^^^^^^01f38f% 🎏   \:flags:    Carp Streamer
  ^^^^^^01f390% 🎐   \:wind_chime:   Wind Chime
  ^^^^^^01f391% 🎑   \:rice_scene:   Moon Viewing Ceremony
  ^^^^^^01f392% 🎒   \:school_satchel:   School Satchel
  ^^^^^^01f393% 🎓   \:mortar_board: Graduation Cap
  ^^^^^^01f3a0% 🎠   \:carousel_horse:   Carousel Horse
  ^^^^^^01f3a1% 🎡   \:ferris_wheel: Ferris Wheel
  ^^^^^^01f3a2% 🎢   \:roller_coaster:   Roller Coaster
  ^^^^^^01f3a3% 🎣   \:fishing_pole_and_fish:    Fishing Pole And Fish
  ^^^^^^01f3a4% 🎤   \:microphone:   Microphone
  ^^^^^^01f3a5% 🎥   \:movie_camera: Movie Camera
  ^^^^^^01f3a6% 🎦   \:cinema:   Cinema
  ^^^^^^01f3a7% 🎧   \:headphones:   Headphone
  ^^^^^^01f3a8% 🎨   \:art:  Artist Palette
  ^^^^^^01f3a9% 🎩   \:tophat:   Top Hat
  ^^^^^^01f3aa% 🎪   \:circus_tent:  Circus Tent
  ^^^^^^01f3ab% 🎫   \:ticket:   Ticket
  ^^^^^^01f3ac% 🎬   \:clapper:  Clapper Board
  ^^^^^^01f3ad% 🎭   \:performing_arts:  Performing Arts
  ^^^^^^01f3ae% 🎮   \:video_game:   Video Game
  ^^^^^^01f3af% 🎯   \:dart: Direct Hit
  ^^^^^^01f3b0% 🎰   \:slot_machine: Slot Machine
  ^^^^^^01f3b1% 🎱   \:8ball:    Billiards
  ^^^^^^01f3b2% 🎲   \:game_die: Game Die
  ^^^^^^01f3b3% 🎳   \:bowling:  Bowling
  ^^^^^^01f3b4% 🎴   \:flower_playing_cards: Flower Playing Cards
  ^^^^^^01f3b5% 🎵   \:musical_note: Musical Note
  ^^^^^^01f3b6% 🎶   \:notes:    Multiple Musical Notes
  ^^^^^^01f3b7% 🎷   \:saxophone:    Saxophone
  ^^^^^^01f3b8% 🎸   \:guitar:   Guitar
  ^^^^^^01f3b9% 🎹   \:musical_keyboard: Musical Keyboard
  ^^^^^^01f3ba% 🎺   \:trumpet:  Trumpet
  ^^^^^^01f3bb% 🎻   \:violin:   Violin
  ^^^^^^01f3bc% 🎼   \:musical_score:    Musical Score
  ^^^^^^01f3bd% 🎽   \:running_shirt_with_sash:  Running Shirt With Sash
  ^^^^^^01f3be% 🎾   \:tennis:   Tennis Racquet And Ball
  ^^^^^^01f3bf% 🎿   \:ski:  Ski And Ski Boot
  ^^^^^^01f3c0% 🏀   \:basketball:   Basketball And Hoop
  ^^^^^^01f3c1% 🏁   \:checkered_flag:   Chequered Flag
  ^^^^^^01f3c2% 🏂   \:snowboarder:  Snowboarder
  ^^^^^^01f3c3% 🏃   \:runner:   Runner
  ^^^^^^01f3c4% 🏄   \:surfer:   Surfer
  ^^^^^^01f3c6% 🏆   \:trophy:   Trophy
  ^^^^^^01f3c7% 🏇   \:horse_racing: Horse Racing
  ^^^^^^01f3c8% 🏈   \:football: American Football
  ^^^^^^01f3c9% 🏉   \:rugby_football:   Rugby Football
  ^^^^^^01f3ca% 🏊   \:swimmer:  Swimmer
  ^^^^^^01f3e0% 🏠   \:house:    House Building
  ^^^^^^01f3e1% 🏡   \:house_with_garden:    House With Garden
  ^^^^^^01f3e2% 🏢   \:office:   Office Building
  ^^^^^^01f3e3% 🏣   \:post_office:  Japanese Post Office
  ^^^^^^01f3e4% 🏤   \:european_post_office: European Post Office
  ^^^^^^01f3e5% 🏥   \:hospital: Hospital
  ^^^^^^01f3e6% 🏦   \:bank: Bank
  ^^^^^^01f3e7% 🏧   \:atm:  Automated Teller Machine
  ^^^^^^01f3e8% 🏨   \:hotel:    Hotel
  ^^^^^^01f3e9% 🏩   \:love_hotel:   Love Hotel
  ^^^^^^01f3ea% 🏪   \:convenience_store:    Convenience Store
  ^^^^^^01f3eb% 🏫   \:school:   School
  ^^^^^^01f3ec% 🏬   \:department_store: Department Store
  ^^^^^^01f3ed% 🏭   \:factory:  Factory
  ^^^^^^01f3ee% 🏮   \:izakaya_lantern:  Izakaya Lantern
  ^^^^^^01f3ef% 🏯   \:japanese_castle:  Japanese Castle
  ^^^^^^01f3f0% 🏰   \:european_castle:  European Castle
  ^^^^^^01f3fb% 🏻   \:skin-tone-2:  Emoji Modifier Fitzpatrick Type-1-2
  ^^^^^^01f3fc% 🏼   \:skin-tone-3:  Emoji Modifier Fitzpatrick Type-3
  ^^^^^^01f3fd% 🏽   \:skin-tone-4:  Emoji Modifier Fitzpatrick Type-4
  ^^^^^^01f3fe% 🏾   \:skin-tone-5:  Emoji Modifier Fitzpatrick Type-5
  ^^^^^^01f3ff% 🏿   \:skin-tone-6:  Emoji Modifier Fitzpatrick Type-6
  ^^^^^^01f400% 🐀   \:rat:  Rat
  ^^^^^^01f401% 🐁   \:mouse2:   Mouse
  ^^^^^^01f402% 🐂   \:ox:   Ox
  ^^^^^^01f403% 🐃   \:water_buffalo:    Water Buffalo
  ^^^^^^01f404% 🐄   \:cow2: Cow
  ^^^^^^01f405% 🐅   \:tiger2:   Tiger
  ^^^^^^01f406% 🐆   \:leopard:  Leopard
  ^^^^^^01f407% 🐇   \:rabbit2:  Rabbit
  ^^^^^^01f408% 🐈   \:cat2: Cat
  ^^^^^^01f409% 🐉   \:dragon:   Dragon
  ^^^^^^01f40a% 🐊   \:crocodile:    Crocodile
  ^^^^^^01f40b% 🐋   \:whale2:   Whale
  ^^^^^^01f40c% 🐌   \:snail:    Snail
  ^^^^^^01f40d% 🐍   \:snake:    Snake
  ^^^^^^01f40e% 🐎   \:racehorse:    Horse
  ^^^^^^01f40f% 🐏   \:ram:  Ram
  ^^^^^^01f410% 🐐   \:goat: Goat
  ^^^^^^01f411% 🐑   \:sheep:    Sheep
  ^^^^^^01f412% 🐒   \:monkey:   Monkey
  ^^^^^^01f413% 🐓   \:rooster:  Rooster
  ^^^^^^01f414% 🐔   \:chicken:  Chicken
  ^^^^^^01f415% 🐕   \:dog2: Dog
  ^^^^^^01f416% 🐖   \:pig2: Pig
  ^^^^^^01f417% 🐗   \:boar: Boar
  ^^^^^^01f418% 🐘   \:elephant: Elephant
  ^^^^^^01f419% 🐙   \:octopus:  Octopus
  ^^^^^^01f41a% 🐚   \:shell:    Spiral Shell
  ^^^^^^01f41b% 🐛   \:bug:  Bug
  ^^^^^^01f41c% 🐜   \:ant:  Ant
  ^^^^^^01f41d% 🐝   \:bee:  Honeybee
  ^^^^^^01f41e% 🐞   \:beetle:   Lady Beetle
  ^^^^^^01f41f% 🐟   \:fish: Fish
  ^^^^^^01f420% 🐠   \:tropical_fish:    Tropical Fish
  ^^^^^^01f421% 🐡   \:blowfish: Blowfish
  ^^^^^^01f422% 🐢   \:turtle:   Turtle
  ^^^^^^01f423% 🐣   \:hatching_chick:   Hatching Chick
  ^^^^^^01f424% 🐤   \:baby_chick:   Baby Chick
  ^^^^^^01f425% 🐥   \:hatched_chick:    Front-Facing Baby Chick
  ^^^^^^01f426% 🐦   \:bird: Bird
  ^^^^^^01f427% 🐧   \:penguin:  Penguin
  ^^^^^^01f428% 🐨   \:koala:    Koala
  ^^^^^^01f429% 🐩   \:poodle:   Poodle
  ^^^^^^01f42a% 🐪   \:dromedary_camel:  Dromedary Camel
  ^^^^^^01f42b% 🐫   \:camel:    Bactrian Camel
  ^^^^^^01f42c% 🐬   \:dolphin:  Dolphin
  ^^^^^^01f42d% 🐭   \:mouse:    Mouse Face
  ^^^^^^01f42e% 🐮   \:cow:  Cow Face
  ^^^^^^01f42f% 🐯   \:tiger:    Tiger Face
  ^^^^^^01f430% 🐰   \:rabbit:   Rabbit Face
  ^^^^^^01f431% 🐱   \:cat:  Cat Face
  ^^^^^^01f432% 🐲   \:dragon_face:  Dragon Face
  ^^^^^^01f433% 🐳   \:whale:    Spouting Whale
  ^^^^^^01f434% 🐴   \:horse:    Horse Face
  ^^^^^^01f435% 🐵   \:monkey_face:  Monkey Face
  ^^^^^^01f436% 🐶   \:dog:  Dog Face
  ^^^^^^01f437% 🐷   \:pig:  Pig Face
  ^^^^^^01f438% 🐸   \:frog: Frog Face
  ^^^^^^01f439% 🐹   \:hamster:  Hamster Face
  ^^^^^^01f43a% 🐺   \:wolf: Wolf Face
  ^^^^^^01f43b% 🐻   \:bear: Bear Face
  ^^^^^^01f43c% 🐼   \:panda_face:   Panda Face
  ^^^^^^01f43d% 🐽   \:pig_nose: Pig Nose
  ^^^^^^01f43e% 🐾   \:feet: Paw Prints
  ^^^^^^01f440% 👀   \:eyes: Eyes
  ^^^^^^01f442% 👂   \:ear:  Ear
  ^^^^^^01f443% 👃   \:nose: Nose
  ^^^^^^01f444% 👄   \:lips: Mouth
  ^^^^^^01f445% 👅   \:tongue:   Tongue
  ^^^^^^01f446% 👆   \:point_up_2:   White Up Pointing Backhand Index
  ^^^^^^01f447% 👇   \:point_down:   White Down Pointing Backhand Index
  ^^^^^^01f448% 👈   \:point_left:   White Left Pointing Backhand Index
  ^^^^^^01f449% 👉   \:point_right:  White Right Pointing Backhand Index
  ^^^^^^01f44a% 👊   \:facepunch:    Fisted Hand Sign
  ^^^^^^01f44b% 👋   \:wave: Waving Hand Sign
  ^^^^^^01f44c% 👌   \:ok_hand:  Ok Hand Sign
  ^^^^^^01f44d% 👍   \:+1:   Thumbs Up Sign
  ^^^^^^01f44e% 👎   \:-1:   Thumbs Down Sign
  ^^^^^^01f44f% 👏   \:clap: Clapping Hands Sign
  ^^^^^^01f450% 👐   \:open_hands:   Open Hands Sign
  ^^^^^^01f451% 👑   \:crown:    Crown
  ^^^^^^01f452% 👒   \:womans_hat:   Womans Hat
  ^^^^^^01f453% 👓   \:eyeglasses:   Eyeglasses
  ^^^^^^01f454% 👔   \:necktie:  Necktie
  ^^^^^^01f455% 👕   \:shirt:    T-Shirt
  ^^^^^^01f456% 👖   \:jeans:    Jeans
  ^^^^^^01f457% 👗   \:dress:    Dress
  ^^^^^^01f458% 👘   \:kimono:   Kimono
  ^^^^^^01f459% 👙   \:bikini:   Bikini
  ^^^^^^01f45a% 👚   \:womans_clothes:   Womans Clothes
  ^^^^^^01f45b% 👛   \:purse:    Purse
  ^^^^^^01f45c% 👜   \:handbag:  Handbag
  ^^^^^^01f45d% 👝   \:pouch:    Pouch
  ^^^^^^01f45e% 👞   \:mans_shoe:    Mans Shoe
  ^^^^^^01f45f% 👟   \:athletic_shoe:    Athletic Shoe
  ^^^^^^01f460% 👠   \:high_heel:    High-Heeled Shoe
  ^^^^^^01f461% 👡   \:sandal:   Womans Sandal
  ^^^^^^01f462% 👢   \:boot: Womans Boots
  ^^^^^^01f463% 👣   \:footprints:   Footprints
  ^^^^^^01f464% 👤   \:bust_in_silhouette:   Bust In Silhouette
  ^^^^^^01f465% 👥   \:busts_in_silhouette:  Busts In Silhouette
  ^^^^^^01f466% 👦   \:boy:  Boy
  ^^^^^^01f467% 👧   \:girl: Girl
  ^^^^^^01f468% 👨   \:man:  Man
  ^^^^^^01f469% 👩   \:woman:    Woman
  ^^^^^^01f46a% 👪   \:family:   Family
  ^^^^^^01f46b% 👫   \:couple:   Man And Woman Holding Hands
  ^^^^^^01f46c% 👬   \:two_men_holding_hands:    Two Men Holding Hands
  ^^^^^^01f46d% 👭   \:two_women_holding_hands:  Two Women Holding Hands
  ^^^^^^01f46e% 👮   \:cop:  Police Officer
  ^^^^^^01f46f% 👯   \:dancers:  Woman With Bunny Ears
  ^^^^^^01f470% 👰   \:bride_with_veil:  Bride With Veil
  ^^^^^^01f471% 👱   \:person_with_blond_hair:   Person With Blond Hair
  ^^^^^^01f472% 👲   \:man_with_gua_pi_mao:  Man With Gua Pi Mao
  ^^^^^^01f473% 👳   \:man_with_turban:  Man With Turban
  ^^^^^^01f474% 👴   \:older_man:    Older Man
  ^^^^^^01f475% 👵   \:older_woman:  Older Woman
  ^^^^^^01f476% 👶   \:baby: Baby
  ^^^^^^01f477% 👷   \:construction_worker:  Construction Worker
  ^^^^^^01f478% 👸   \:princess: Princess
  ^^^^^^01f479% 👹   \:japanese_ogre:    Japanese Ogre
  ^^^^^^01f47a% 👺   \:japanese_goblin:  Japanese Goblin
  ^^^^^^01f47b% 👻   \:ghost:    Ghost
  ^^^^^^01f47c% 👼   \:angel:    Baby Angel
  ^^^^^^01f47d% 👽   \:alien:    Extraterrestrial Alien
  ^^^^^^01f47e% 👾   \:space_invader:    Alien Monster
  ^^^^^^01f47f% 👿   \:imp:  Imp
  ^^^^^^01f480% 💀   \:skull:    Skull
  ^^^^^^01f481% 💁   \:information_desk_person:  Information Desk Person
  ^^^^^^01f482% 💂   \:guardsman:    Guardsman
  ^^^^^^01f483% 💃   \:dancer:   Dancer
  ^^^^^^01f484% 💄   \:lipstick: Lipstick
  ^^^^^^01f485% 💅   \:nail_care:    Nail Polish
  ^^^^^^01f486% 💆   \:massage:  Face Massage
  ^^^^^^01f487% 💇   \:haircut:  Haircut
  ^^^^^^01f488% 💈   \:barber:   Barber Pole
  ^^^^^^01f489% 💉   \:syringe:  Syringe
  ^^^^^^01f48a% 💊   \:pill: Pill
  ^^^^^^01f48b% 💋   \:kiss: Kiss Mark
  ^^^^^^01f48c% 💌   \:love_letter:  Love Letter
  ^^^^^^01f48d% 💍   \:ring: Ring
  ^^^^^^01f48e% 💎   \:gem:  Gem Stone
  ^^^^^^01f48f% 💏   \:couplekiss:   Kiss
  ^^^^^^01f490% 💐   \:bouquet:  Bouquet
  ^^^^^^01f491% 💑   \:couple_with_heart:    Couple With Heart
  ^^^^^^01f492% 💒   \:wedding:  Wedding
  ^^^^^^01f493% 💓   \:heartbeat:    Beating Heart
  ^^^^^^01f494% 💔   \:broken_heart: Broken Heart
  ^^^^^^01f495% 💕   \:two_hearts:   Two Hearts
  ^^^^^^01f496% 💖   \:sparkling_heart:  Sparkling Heart
  ^^^^^^01f497% 💗   \:heartpulse:   Growing Heart
  ^^^^^^01f498% 💘   \:cupid:    Heart With Arrow
  ^^^^^^01f499% 💙   \:blue_heart:   Blue Heart
  ^^^^^^01f49a% 💚   \:green_heart:  Green Heart
  ^^^^^^01f49b% 💛   \:yellow_heart: Yellow Heart
  ^^^^^^01f49c% 💜   \:purple_heart: Purple Heart
  ^^^^^^01f49d% 💝   \:gift_heart:   Heart With Ribbon
  ^^^^^^01f49e% 💞   \:revolving_hearts: Revolving Hearts
  ^^^^^^01f49f% 💟   \:heart_decoration: Heart Decoration
  ^^^^^^01f4a0% 💠   \:diamond_shape_with_a_dot_inside:  Diamond Shape With A Dot Inside
  ^^^^^^01f4a1% 💡   \:bulb: Electric Light Bulb
  ^^^^^^01f4a2% 💢   \:anger:    Anger Symbol
  ^^^^^^01f4a3% 💣   \:bomb: Bomb
  ^^^^^^01f4a4% 💤   \:zzz:  Sleeping Symbol
  ^^^^^^01f4a5% 💥   \:boom: Collision Symbol
  ^^^^^^01f4a6% 💦   \:sweat_drops:  Splashing Sweat Symbol
  ^^^^^^01f4a7% 💧   \:droplet:  Droplet
  ^^^^^^01f4a8% 💨   \:dash: Dash Symbol
  ^^^^^^01f4a9% 💩   \:hankey:   Pile Of Poo
  ^^^^^^01f4aa% 💪   \:muscle:   Flexed Biceps
  ^^^^^^01f4ab% 💫   \:dizzy:    Dizzy Symbol
  ^^^^^^01f4ac% 💬   \:speech_balloon:   Speech Balloon
  ^^^^^^01f4ad% 💭   \:thought_balloon:  Thought Balloon
  ^^^^^^01f4ae% 💮   \:white_flower: White Flower
  ^^^^^^01f4af% 💯   \:100:  Hundred Points Symbol
  ^^^^^^01f4b0% 💰   \:moneybag: Money Bag
  ^^^^^^01f4b1% 💱   \:currency_exchange:    Currency Exchange
  ^^^^^^01f4b2% 💲   \:heavy_dollar_sign:    Heavy Dollar Sign
  ^^^^^^01f4b3% 💳   \:credit_card:  Credit Card
  ^^^^^^01f4b4% 💴   \:yen:  Banknote With Yen Sign
  ^^^^^^01f4b5% 💵   \:dollar:   Banknote With Dollar Sign
  ^^^^^^01f4b6% 💶   \:euro: Banknote With Euro Sign
  ^^^^^^01f4b7% 💷   \:pound:    Banknote With Pound Sign
  ^^^^^^01f4b8% 💸   \:money_with_wings: Money With Wings
  ^^^^^^01f4b9% 💹   \:chart:    Chart With Upwards Trend And Yen Sign
  ^^^^^^01f4ba% 💺   \:seat: Seat
  ^^^^^^01f4bb% 💻   \:computer: Personal Computer
  ^^^^^^01f4bc% 💼   \:briefcase:    Briefcase
  ^^^^^^01f4bd% 💽   \:minidisc: Minidisc
  ^^^^^^01f4be% 💾   \:floppy_disk:  Floppy Disk
  ^^^^^^01f4bf% 💿   \:cd:   Optical Disc
  ^^^^^^01f4c0% 📀   \:dvd:  Dvd
  ^^^^^^01f4c1% 📁   \:file_folder:  File Folder
  ^^^^^^01f4c2% 📂   \:open_file_folder: Open File Folder
  ^^^^^^01f4c3% 📃   \:page_with_curl:   Page With Curl
  ^^^^^^01f4c4% 📄   \:page_facing_up:   Page Facing Up
  ^^^^^^01f4c5% 📅   \:date: Calendar
  ^^^^^^01f4c6% 📆   \:calendar: Tear-Off Calendar
  ^^^^^^01f4c7% 📇   \:card_index:   Card Index
  ^^^^^^01f4c8% 📈   \:chart_with_upwards_trend: Chart With Upwards Trend
  ^^^^^^01f4c9% 📉   \:chart_with_downwards_trend:   Chart With Downwards Trend
  ^^^^^^01f4ca% 📊   \:bar_chart:    Bar Chart
  ^^^^^^01f4cb% 📋   \:clipboard:    Clipboard
  ^^^^^^01f4cc% 📌   \:pushpin:  Pushpin
  ^^^^^^01f4cd% 📍   \:round_pushpin:    Round Pushpin
  ^^^^^^01f4ce% 📎   \:paperclip:    Paperclip
  ^^^^^^01f4cf% 📏   \:straight_ruler:   Straight Ruler
  ^^^^^^01f4d0% 📐   \:triangular_ruler: Triangular Ruler
  ^^^^^^01f4d1% 📑   \:bookmark_tabs:    Bookmark Tabs
  ^^^^^^01f4d2% 📒   \:ledger:   Ledger
  ^^^^^^01f4d3% 📓   \:notebook: Notebook
  ^^^^^^01f4d4% 📔   \:notebook_with_decorative_cover:   Notebook With Decorative Cover
  ^^^^^^01f4d5% 📕   \:closed_book:  Closed Book
  ^^^^^^01f4d6% 📖   \:book: Open Book
  ^^^^^^01f4d7% 📗   \:green_book:   Green Book
  ^^^^^^01f4d8% 📘   \:blue_book:    Blue Book
  ^^^^^^01f4d9% 📙   \:orange_book:  Orange Book
  ^^^^^^01f4da% 📚   \:books:    Books
  ^^^^^^01f4db% 📛   \:name_badge:   Name Badge
  ^^^^^^01f4dc% 📜   \:scroll:   Scroll
  ^^^^^^01f4dd% 📝   \:memo: Memo
  ^^^^^^01f4de% 📞   \:telephone_receiver:   Telephone Receiver
  ^^^^^^01f4df% 📟   \:pager:    Pager
  ^^^^^^01f4e0% 📠   \:fax:  Fax Machine
  ^^^^^^01f4e1% 📡   \:satellite:    Satellite Antenna
  ^^^^^^01f4e2% 📢   \:loudspeaker:  Public Address Loudspeaker
  ^^^^^^01f4e3% 📣   \:mega: Cheering Megaphone
  ^^^^^^01f4e4% 📤   \:outbox_tray:  Outbox Tray
  ^^^^^^01f4e5% 📥   \:inbox_tray:   Inbox Tray
  ^^^^^^01f4e6% 📦   \:package:  Package
  ^^^^^^01f4e7% 📧   \:e-mail:   E-Mail Symbol
  ^^^^^^01f4e8% 📨   \:incoming_envelope:    Incoming Envelope
  ^^^^^^01f4e9% 📩   \:envelope_with_arrow:  Envelope With Downwards Arrow Above
  ^^^^^^01f4ea% 📪   \:mailbox_closed:   Closed Mailbox With Lowered Flag
  ^^^^^^01f4eb% 📫   \:mailbox:  Closed Mailbox With Raised Flag
  ^^^^^^01f4ec% 📬   \:mailbox_with_mail:    Open Mailbox With Raised Flag
  ^^^^^^01f4ed% 📭   \:mailbox_with_no_mail: Open Mailbox With Lowered Flag
  ^^^^^^01f4ee% 📮   \:postbox:  Postbox
  ^^^^^^01f4ef% 📯   \:postal_horn:  Postal Horn
  ^^^^^^01f4f0% 📰   \:newspaper:    Newspaper
  ^^^^^^01f4f1% 📱   \:iphone:   Mobile Phone
  ^^^^^^01f4f2% 📲   \:calling:  Mobile Phone With Rightwards Arrow At Left
  ^^^^^^01f4f3% 📳   \:vibration_mode:   Vibration Mode
  ^^^^^^01f4f4% 📴   \:mobile_phone_off: Mobile Phone Off
  ^^^^^^01f4f5% 📵   \:no_mobile_phones: No Mobile Phones
  ^^^^^^01f4f6% 📶   \:signal_strength:  Antenna With Bars
  ^^^^^^01f4f7% 📷   \:camera:   Camera
  ^^^^^^01f4f9% 📹   \:video_camera: Video Camera
  ^^^^^^01f4fa% 📺   \:tv:   Television
  ^^^^^^01f4fb% 📻   \:radio:    Radio
  ^^^^^^01f4fc% 📼   \:vhs:  Videocassette
  ^^^^^^01f500% 🔀   \:twisted_rightwards_arrows:    Twisted Rightwards Arrows
  ^^^^^^01f501% 🔁   \:repeat:   Clockwise Rightwards And Leftwards Open Circle Arrows
  ^^^^^^01f502% 🔂   \:repeat_one:   Clockwise Rightwards And Leftwards Open Circle Arrows With Circled One Overlay
  ^^^^^^01f503% 🔃   \:arrows_clockwise: Clockwise Downwards And Upwards Open Circle Arrows
  ^^^^^^01f504% 🔄   \:arrows_counterclockwise:  Anticlockwise Downwards And Upwards Open Circle Arrows
  ^^^^^^01f505% 🔅   \:low_brightness:   Low Brightness Symbol
  ^^^^^^01f506% 🔆   \:high_brightness:  High Brightness Symbol
  ^^^^^^01f507% 🔇   \:mute: Speaker With Cancellation Stroke
  ^^^^^^01f508% 🔈   \:speaker:  Speaker
  ^^^^^^01f509% 🔉   \:sound:    Speaker With One Sound Wave
  ^^^^^^01f50a% 🔊   \:loud_sound:   Speaker With Three Sound Waves
  ^^^^^^01f50b% 🔋   \:battery:  Battery
  ^^^^^^01f50c% 🔌   \:electric_plug:    Electric Plug
  ^^^^^^01f50d% 🔍   \:mag:  Left-Pointing Magnifying Glass
  ^^^^^^01f50e% 🔎   \:mag_right:    Right-Pointing Magnifying Glass
  ^^^^^^01f50f% 🔏   \:lock_with_ink_pen:    Lock With Ink Pen
  ^^^^^^01f510% 🔐   \:closed_lock_with_key: Closed Lock With Key
  ^^^^^^01f511% 🔑   \:key:  Key
  ^^^^^^01f512% 🔒   \:lock: Lock
  ^^^^^^01f513% 🔓   \:unlock:   Open Lock
  ^^^^^^01f514% 🔔   \:bell: Bell
  ^^^^^^01f515% 🔕   \:no_bell:  Bell With Cancellation Stroke
  ^^^^^^01f516% 🔖   \:bookmark: Bookmark
  ^^^^^^01f517% 🔗   \:link: Link Symbol
  ^^^^^^01f518% 🔘   \:radio_button: Radio Button
  ^^^^^^01f519% 🔙   \:back: Back With Leftwards Arrow Above
  ^^^^^^01f51a% 🔚   \:end:  End With Leftwards Arrow Above
  ^^^^^^01f51b% 🔛   \:on:   On With Exclamation Mark With Left Right Arrow Above
  ^^^^^^01f51c% 🔜   \:soon: Soon With Rightwards Arrow Above
  ^^^^^^01f51d% 🔝   \:top:  Top With Upwards Arrow Above
  ^^^^^^01f51e% 🔞   \:underage: No One Under Eighteen Symbol
  ^^^^^^01f51f% 🔟   \:keycap_ten:   Keycap Ten
  ^^^^^^01f520% 🔠   \:capital_abcd: Input Symbol For Latin Capital Letters
  ^^^^^^01f521% 🔡   \:abcd: Input Symbol For Latin Small Letters
  ^^^^^^01f522% 🔢   \:1234: Input Symbol For Numbers
  ^^^^^^01f523% 🔣   \:symbols:  Input Symbol For Symbols
  ^^^^^^01f524% 🔤   \:abc:  Input Symbol For Latin Letters
  ^^^^^^01f525% 🔥   \:fire: Fire
  ^^^^^^01f526% 🔦   \:flashlight:   Electric Torch
  ^^^^^^01f527% 🔧   \:wrench:   Wrench
  ^^^^^^01f528% 🔨   \:hammer:   Hammer
  ^^^^^^01f529% 🔩   \:nut_and_bolt: Nut And Bolt
  ^^^^^^01f52a% 🔪   \:hocho:    Hocho
  ^^^^^^01f52b% 🔫   \:gun:  Pistol
  ^^^^^^01f52c% 🔬   \:microscope:   Microscope
  ^^^^^^01f52d% 🔭   \:telescope:    Telescope
  ^^^^^^01f52e% 🔮   \:crystal_ball: Crystal Ball
  ^^^^^^01f52f% 🔯   \:six_pointed_star: Six Pointed Star With Middle Dot
  ^^^^^^01f530% 🔰   \:beginner: Japanese Symbol For Beginner
  ^^^^^^01f531% 🔱   \:trident:  Trident Emblem
  ^^^^^^01f532% 🔲   \:black_square_button:  Black Square Button
  ^^^^^^01f533% 🔳   \:white_square_button:  White Square Button
  ^^^^^^01f534% 🔴   \:red_circle:   Large Red Circle
  ^^^^^^01f535% 🔵   \:large_blue_circle:    Large Blue Circle
  ^^^^^^01f536% 🔶   \:large_orange_diamond: Large Orange Diamond
  ^^^^^^01f537% 🔷   \:large_blue_diamond:   Large Blue Diamond
  ^^^^^^01f538% 🔸   \:small_orange_diamond: Small Orange Diamond
  ^^^^^^01f539% 🔹   \:small_blue_diamond:   Small Blue Diamond
  ^^^^^^01f53a% 🔺   \:small_red_triangle:   Up-Pointing Red Triangle
  ^^^^^^01f53b% 🔻   \:small_red_triangle_down:  Down-Pointing Red Triangle
  ^^^^^^01f53c% 🔼   \:arrow_up_small:   Up-Pointing Small Red Triangle
  ^^^^^^01f53d% 🔽   \:arrow_down_small: Down-Pointing Small Red Triangle
  ^^^^^^01f550% 🕐   \:clock1:   Clock Face One Oclock
  ^^^^^^01f551% 🕑   \:clock2:   Clock Face Two Oclock
  ^^^^^^01f552% 🕒   \:clock3:   Clock Face Three Oclock
  ^^^^^^01f553% 🕓   \:clock4:   Clock Face Four Oclock
  ^^^^^^01f554% 🕔   \:clock5:   Clock Face Five Oclock
  ^^^^^^01f555% 🕕   \:clock6:   Clock Face Six Oclock
  ^^^^^^01f556% 🕖   \:clock7:   Clock Face Seven Oclock
  ^^^^^^01f557% 🕗   \:clock8:   Clock Face Eight Oclock
  ^^^^^^01f558% 🕘   \:clock9:   Clock Face Nine Oclock
  ^^^^^^01f559% 🕙   \:clock10:  Clock Face Ten Oclock
  ^^^^^^01f55a% 🕚   \:clock11:  Clock Face Eleven Oclock
  ^^^^^^01f55b% 🕛   \:clock12:  Clock Face Twelve Oclock
  ^^^^^^01f55c% 🕜   \:clock130: Clock Face One-Thirty
  ^^^^^^01f55d% 🕝   \:clock230: Clock Face Two-Thirty
  ^^^^^^01f55e% 🕞   \:clock330: Clock Face Three-Thirty
  ^^^^^^01f55f% 🕟   \:clock430: Clock Face Four-Thirty
  ^^^^^^01f560% 🕠   \:clock530: Clock Face Five-Thirty
  ^^^^^^01f561% 🕡   \:clock630: Clock Face Six-Thirty
  ^^^^^^01f562% 🕢   \:clock730: Clock Face Seven-Thirty
  ^^^^^^01f563% 🕣   \:clock830: Clock Face Eight-Thirty
  ^^^^^^01f564% 🕤   \:clock930: Clock Face Nine-Thirty
  ^^^^^^01f565% 🕥   \:clock1030:    Clock Face Ten-Thirty
  ^^^^^^01f566% 🕦   \:clock1130:    Clock Face Eleven-Thirty
  ^^^^^^01f567% 🕧   \:clock1230:    Clock Face Twelve-Thirty
  ^^^^^^01f5fb% 🗻   \:mount_fuji:   Mount Fuji
  ^^^^^^01f5fc% 🗼   \:tokyo_tower:  Tokyo Tower
  ^^^^^^01f5fd% 🗽   \:statue_of_liberty:    Statue Of Liberty
  ^^^^^^01f5fe% 🗾   \:japan:    Silhouette Of Japan
  ^^^^^^01f5ff% 🗿   \:moyai:    Moyai
  ^^^^^^01f600% 😀   \:grinning: Grinning Face
  ^^^^^^01f601% 😁   \:grin: Grinning Face With Smiling Eyes
  ^^^^^^01f602% 😂   \:joy:  Face With Tears Of Joy
  ^^^^^^01f603% 😃   \:smiley:   Smiling Face With Open Mouth
  ^^^^^^01f604% 😄   \:smile:    Smiling Face With Open Mouth And Smiling Eyes
  ^^^^^^01f605% 😅   \:sweat_smile:  Smiling Face With Open Mouth And Cold Sweat
  ^^^^^^01f606% 😆   \:laughing: Smiling Face With Open Mouth And Tightly-Closed Eyes
  ^^^^^^01f607% 😇   \:innocent: Smiling Face With Halo
  ^^^^^^01f608% 😈   \:smiling_imp:  Smiling Face With Horns
  ^^^^^^01f609% 😉   \:wink: Winking Face
  ^^^^^^01f60a% 😊   \:blush:    Smiling Face With Smiling Eyes
  ^^^^^^01f60b% 😋   \:yum:  Face Savouring Delicious Food
  ^^^^^^01f60c% 😌   \:relieved: Relieved Face
  ^^^^^^01f60d% 😍   \:heart_eyes:   Smiling Face With Heart-Shaped Eyes
  ^^^^^^01f60e% 😎   \:sunglasses:   Smiling Face With Sunglasses
  ^^^^^^01f60f% 😏   \:smirk:    Smirking Face
  ^^^^^^01f610% 😐   \:neutral_face: Neutral Face
  ^^^^^^01f611% 😑   \:expressionless:   Expressionless Face
  ^^^^^^01f612% 😒   \:unamused: Unamused Face
  ^^^^^^01f613% 😓   \:sweat:    Face With Cold Sweat
  ^^^^^^01f614% 😔   \:pensive:  Pensive Face
  ^^^^^^01f615% 😕   \:confused: Confused Face
  ^^^^^^01f616% 😖   \:confounded:   Confounded Face
  ^^^^^^01f617% 😗   \:kissing:  Kissing Face
  ^^^^^^01f618% 😘   \:kissing_heart:    Face Throwing A Kiss
  ^^^^^^01f619% 😙   \:kissing_smiling_eyes: Kissing Face With Smiling Eyes
  ^^^^^^01f61a% 😚   \:kissing_closed_eyes:  Kissing Face With Closed Eyes
  ^^^^^^01f61b% 😛   \:stuck_out_tongue: Face With Stuck-Out Tongue
  ^^^^^^01f61c% 😜   \:stuck_out_tongue_winking_eye: Face With Stuck-Out Tongue And Winking Eye
  ^^^^^^01f61d% 😝   \:stuck_out_tongue_closed_eyes: Face With Stuck-Out Tongue And Tightly-Closed Eyes
  ^^^^^^01f61e% 😞   \:disappointed: Disappointed Face
  ^^^^^^01f61f% 😟   \:worried:  Worried Face
  ^^^^^^01f620% 😠   \:angry:    Angry Face
  ^^^^^^01f621% 😡   \:rage: Pouting Face
  ^^^^^^01f622% 😢   \:cry:  Crying Face
  ^^^^^^01f623% 😣   \:persevere:    Persevering Face
  ^^^^^^01f624% 😤   \:triumph:  Face With Look Of Triumph
  ^^^^^^01f625% 😥   \:disappointed_relieved:    Disappointed But Relieved Face
  ^^^^^^01f626% 😦   \:frowning: Frowning Face With Open Mouth
  ^^^^^^01f627% 😧   \:anguished:    Anguished Face
  ^^^^^^01f628% 😨   \:fearful:  Fearful Face
  ^^^^^^01f629% 😩   \:weary:    Weary Face
  ^^^^^^01f62a% 😪   \:sleepy:   Sleepy Face
  ^^^^^^01f62b% 😫   \:tired_face:   Tired Face
  ^^^^^^01f62c% 😬   \:grimacing:    Grimacing Face
  ^^^^^^01f62d% 😭   \:sob:  Loudly Crying Face
  ^^^^^^01f62e% 😮   \:open_mouth:   Face With Open Mouth
  ^^^^^^01f62f% 😯   \:hushed:   Hushed Face
  ^^^^^^01f630% 😰   \:cold_sweat:   Face With Open Mouth And Cold Sweat
  ^^^^^^01f631% 😱   \:scream:   Face Screaming In Fear
  ^^^^^^01f632% 😲   \:astonished:   Astonished Face
  ^^^^^^01f633% 😳   \:flushed:  Flushed Face
  ^^^^^^01f634% 😴   \:sleeping: Sleeping Face
  ^^^^^^01f635% 😵   \:dizzy_face:   Dizzy Face
  ^^^^^^01f636% 😶   \:no_mouth: Face Without Mouth
  ^^^^^^01f637% 😷   \:mask: Face With Medical Mask
  ^^^^^^01f638% 😸   \:smile_cat:    Grinning Cat Face With Smiling Eyes
  ^^^^^^01f639% 😹   \:joy_cat:  Cat Face With Tears Of Joy
  ^^^^^^01f63a% 😺   \:smiley_cat:   Smiling Cat Face With Open Mouth
  ^^^^^^01f63b% 😻   \:heart_eyes_cat:   Smiling Cat Face With Heart-Shaped Eyes
  ^^^^^^01f63c% 😼   \:smirk_cat:    Cat Face With Wry Smile
  ^^^^^^01f63d% 😽   \:kissing_cat:  Kissing Cat Face With Closed Eyes
  ^^^^^^01f63e% 😾   \:pouting_cat:  Pouting Cat Face
  ^^^^^^01f63f% 😿   \:crying_cat_face:  Crying Cat Face
  ^^^^^^01f640% 🙀   \:scream_cat:   Weary Cat Face
  ^^^^^^01f645% 🙅   \:no_good:  Face With No Good Gesture
  ^^^^^^01f646% 🙆   \:ok_woman: Face With Ok Gesture
  ^^^^^^01f647% 🙇   \:bow:  Person Bowing Deeply
  ^^^^^^01f648% 🙈   \:see_no_evil:  See-No-Evil Monkey
  ^^^^^^01f649% 🙉   \:hear_no_evil: Hear-No-Evil Monkey
  ^^^^^^01f64a% 🙊   \:speak_no_evil:    Speak-No-Evil Monkey
  ^^^^^^01f64b% 🙋   \:raising_hand: Happy Person Raising One Hand
  ^^^^^^01f64c% 🙌   \:raised_hands: Person Raising Both Hands In Celebration
  ^^^^^^01f64d% 🙍   \:person_frowning:  Person Frowning
  ^^^^^^01f64e% 🙎   \:person_with_pouting_face: Person With Pouting Face
  ^^^^^^01f64f% 🙏   \:pray: Person With Folded Hands
  ^^^^^^01f680% 🚀   \:rocket:   Rocket
  ^^^^^^01f681% 🚁   \:helicopter:   Helicopter
  ^^^^^^01f682% 🚂   \:steam_locomotive: Steam Locomotive
  ^^^^^^01f683% 🚃   \:railway_car:  Railway Car
  ^^^^^^01f684% 🚄   \:bullettrain_side: High-Speed Train
  ^^^^^^01f685% 🚅   \:bullettrain_front:    High-Speed Train With Bullet Nose
  ^^^^^^01f686% 🚆   \:train2:   Train
  ^^^^^^01f687% 🚇   \:metro:    Metro
  ^^^^^^01f688% 🚈   \:light_rail:   Light Rail
  ^^^^^^01f689% 🚉   \:station:  Station
  ^^^^^^01f68a% 🚊   \:tram: Tram
  ^^^^^^01f68b% 🚋   \:train:    Tram Car
  ^^^^^^01f68c% 🚌   \:bus:  Bus
  ^^^^^^01f68d% 🚍   \:oncoming_bus: Oncoming Bus
  ^^^^^^01f68e% 🚎   \:trolleybus:   Trolleybus
  ^^^^^^01f68f% 🚏   \:busstop:  Bus Stop
  ^^^^^^01f690% 🚐   \:minibus:  Minibus
  ^^^^^^01f691% 🚑   \:ambulance:    Ambulance
  ^^^^^^01f692% 🚒   \:fire_engine:  Fire Engine
  ^^^^^^01f693% 🚓   \:police_car:   Police Car
  ^^^^^^01f694% 🚔   \:oncoming_police_car:  Oncoming Police Car
  ^^^^^^01f695% 🚕   \:taxi: Taxi
  ^^^^^^01f696% 🚖   \:oncoming_taxi:    Oncoming Taxi
  ^^^^^^01f697% 🚗   \:car:  Automobile
  ^^^^^^01f698% 🚘   \:oncoming_automobile:  Oncoming Automobile
  ^^^^^^01f699% 🚙   \:blue_car: Recreational Vehicle
  ^^^^^^01f69a% 🚚   \:truck:    Delivery Truck
  ^^^^^^01f69b% 🚛   \:articulated_lorry:    Articulated Lorry
  ^^^^^^01f69c% 🚜   \:tractor:  Tractor
  ^^^^^^01f69d% 🚝   \:monorail: Monorail
  ^^^^^^01f69e% 🚞   \:mountain_railway: Mountain Railway
  ^^^^^^01f69f% 🚟   \:suspension_railway:   Suspension Railway
  ^^^^^^01f6a0% 🚠   \:mountain_cableway:    Mountain Cableway
  ^^^^^^01f6a1% 🚡   \:aerial_tramway:   Aerial Tramway
  ^^^^^^01f6a2% 🚢   \:ship: Ship
  ^^^^^^01f6a3% 🚣   \:rowboat:  Rowboat
  ^^^^^^01f6a4% 🚤   \:speedboat:    Speedboat
  ^^^^^^01f6a5% 🚥   \:traffic_light:    Horizontal Traffic Light
  ^^^^^^01f6a6% 🚦   \:vertical_traffic_light:   Vertical Traffic Light
  ^^^^^^01f6a7% 🚧   \:construction: Construction Sign
  ^^^^^^01f6a8% 🚨   \:rotating_light:   Police Cars Revolving Light
  ^^^^^^01f6a9% 🚩   \:triangular_flag_on_post:  Triangular Flag On Post
  ^^^^^^01f6aa% 🚪   \:door: Door
  ^^^^^^01f6ab% 🚫   \:no_entry_sign:    No Entry Sign
  ^^^^^^01f6ac% 🚬   \:smoking:  Smoking Symbol
  ^^^^^^01f6ad% 🚭   \:no_smoking:   No Smoking Symbol
  ^^^^^^01f6ae% 🚮   \:put_litter_in_its_place:  Put Litter In Its Place Symbol
  ^^^^^^01f6af% 🚯   \:do_not_litter:    Do Not Litter Symbol
  ^^^^^^01f6b0% 🚰   \:potable_water:    Potable Water Symbol
  ^^^^^^01f6b1% 🚱   \:non-potable_water:    Non-Potable Water Symbol
  ^^^^^^01f6b2% 🚲   \:bike: Bicycle
  ^^^^^^01f6b3% 🚳   \:no_bicycles:  No Bicycles
  ^^^^^^01f6b4% 🚴   \:bicyclist:    Bicyclist
  ^^^^^^01f6b5% 🚵   \:mountain_bicyclist:   Mountain Bicyclist
  ^^^^^^01f6b6% 🚶   \:walking:  Pedestrian
  ^^^^^^01f6b7% 🚷   \:no_pedestrians:   No Pedestrians
  ^^^^^^01f6b8% 🚸   \:children_crossing:    Children Crossing
  ^^^^^^01f6b9% 🚹   \:mens: Mens Symbol
  ^^^^^^01f6ba% 🚺   \:womens:   Womens Symbol
  ^^^^^^01f6bb% 🚻   \:restroom: Restroom
  ^^^^^^01f6bc% 🚼   \:baby_symbol:  Baby Symbol
  ^^^^^^01f6bd% 🚽   \:toilet:   Toilet
  ^^^^^^01f6be% 🚾   \:wc:   Water Closet
  ^^^^^^01f6bf% 🚿   \:shower:   Shower
  ^^^^^^01f6c0% 🛀   \:bath: Bath
  ^^^^^^01f6c1% 🛁   \:bathtub:  Bathtub
  ^^^^^^01f6c2% 🛂   \:passport_control: Passport Control
  ^^^^^^01f6c3% 🛃   \:customs:  Customs
  ^^^^^^01f6c4% 🛄   \:baggage_claim:    Baggage Claim
  ^^^^^^01f6c5% 🛅   \:left_luggage: Left Luggage
  ^^00}
\lst@RestoreCatcodes
\makeatother

